SpeechBrain: A General-Purpose Speech Toolkit

SpeechBrain is an open-source and all-in-one speech toolkit. It is designed to facilitate the research and development of neural speech processing technologies by being simple, flexible, user-friendly, and well-documented. This paper describes the core architecture designed to support several tasks of common interest, allowing users to naturally conceive, compare and share novel speech processing pipelines. SpeechBrain achieves competitive or state-of-the-art performance in a wide range of speech benchmarks. It also provides training recipes, pretrained models, and inference scripts for popular speech datasets, as well as tutorials which allow anyone with basic Python proficiency to familiarize themselves with speech technologies.

==> copyofmybib <==
@article{spec_tutorial,
  author    = {Ulrike von Luxburg},
  title     = {A Tutorial on Spectral Clustering},
  journal   = {Statistics and Computing},
  volume    = {17},
  number    = {4},
  year      = {2007},
}


@ARTICLE{bsseval,
  author={Vincent, E. and Gribonval, R. and Fevotte, C.},
  journal={IEEE Transactions on Audio, Speech, and Language Processing}, 
  title={Performance measurement in blind audio source separation}, 
  year={2006},
  volume={14},
  number={4},
  pages={1462-1469},
  doi={10.1109/TSA.2005.858005}}


@misc{landini2020VBX,
      title={Bayesian {HMM} clustering of x-vector sequences ({VBx}) in speaker diarization: theory, implementation and analysis on standard tasks}, 
      author={Federico Landini and Ján Profant and Mireia Diez and Lukáš Burget},
      year={2020},
      eprint={2012.14952},
      archivePrefix={arXiv},
      primaryClass={eess.AS},
      note = {arXiv:2012.14952},
}


@TechReport{Lang+Hinton88,
  author =       "K. J. Lang and G. E. Hinton",
  title =        "The development of the Time-Delay Neural Network
                 architecture for speech recognition",
  number =       "CMU-CS-88-152",
  institution =  "Carnegie-Mellon University",
  year =         "1988",
}

@INPROCEEDINGS{Kenny-plda,
  author={Kenny, Patrick and Stafylakis, Themos and Ouellet, Pierre and Alam, Md. Jahangir and Dumouchel, Pierre},
  booktitle={2013 IEEE International Conference on Acoustics, Speech and Signal Processing}, 
  title={{PLDA} for speaker verification with utterances of arbitrary duration}, 
  year={2013},
  volume={},
  number={},
  pages={7649-7653},
  doi={10.1109/ICASSP.2013.6639151}}


@inproceedings{GarciaRomero2011AnalysisOI,
  title={Analysis of i-vector Length Normalization in Speaker Recognition Systems},
  author={D. Garcia-Romero and C. Espy-Wilson},
  booktitle={INTERSPEECH},
  pages={249-252},
  year={2011}
}

@inproceedings{ami-corpus,
 author = {Carletta, Jean and Ashby, Simone and Bourban, Sebastien and Flynn, Mike and Guillemot, Mael and Hain, Thomas and Kadlec, Jaroslav and Karaiskos, Vasilis and Kraaij, Wessel and Kronenthal, Melissa and Lathoud, Guillaume and Lincoln, Mike and Lisowska, Agnes and McCowan, Iain and Post, Wilfried and Reidsma, Dennis and Wellner, Pierre},
 title = {The {AMI} Meeting Corpus: A Pre-announcement},
 booktitle = {Proc. the Second International Conference on Machine Learning for Multimodal Interaction},
 series = {MLMI'05},
 year = {2006},
 location = {Edinburgh, UK},
 address = {28--39},
 numpages = {12},
 }





@InProceedings{C2,
  author = 	 "Jones, C.D. and Smith, A.B. and Roberts, E.F.",
  title =        "Article Title",
  booktitle =        "Proceedings Title",
  organization = "IEEE",
  year = 	 "2003",
  volume = 	 "II",
  pages = 	 "803-806"
}

@Inproceedings{guerrero16,
  author= {Guerrero, Cristina and Tryfou, Georgina and Omologo, M.},
  title= {{Channel Selection for Distant Speech Recognition Exploiting Cepstral Distance}},
  booktitle = {Proc. of Interspeech 2016}
}

@article{bruttiloc,
  author = {Brutti, Alessio and Omologo, Maurizio and Svaizer, Piergiorgio},
  journal = {EURASIP Journal on Audio, Speech and Music Processing},
  title = {Multiple Source Localization Based on Acoustic Map De-Emphasis.},
  volume = 2010,
  year = 2010,
 pages = {11-17},
}

@inproceedings{Park2019,
  author={Daniel S. Park and William Chan and Yu Zhang and Chung-Cheng Chiu and Barret Zoph and Ekin D. Cubuk and Quoc V. Le},
  title={{SpecAugment: A Simple Data Augmentation Method for Automatic Speech Recognition}},
  year=2019,
  booktitle={Proc. Interspeech},
  pages={2613--2617},}
}

@Inproceedings{acoustic_raw_povey,
author = {P. Ghahremani and V. Manohar and D. Povey and S. Khudanpur},
title = {{Acoustic modelling from the signal domain using CNNs}},
booktitle = {Proc. of Interspeech},
year = {2016} } 

@Inproceedings{verification_raw_ICASSP2018,
author = {J.-W. Jung and  H.-S. Heo and I.-H. Yang and  H.-J. Shim and and H.-J. Yu},
title = {A COMPLETE END-TO-END SPEAKER VERIFICATION SYSTEM USING DEEP NEURAL NETWORKS: FROM RAW SIGNALS TO VERIFICATION RESULT},
booktitle = {Proc. of ICASSP},
year = {2018} } 

@Inproceedings{verification_raw_IS2018,
author = {J.-W. Jung and  H.-S. Heo and  I.-H. Yang and H.-J. Shim, and H.-J. Yu},
title = {{Avoiding Speaker Overfitting in End-to-End DNNs using Raw Waveform
for Text-Independent Speaker Verification}},
booktitle = {Proc. of Interspeech},
year = {2018} } 

@Inproceedings{ravanelli_icassp,
  author= "M. Ravanelli and P. Brakel and M. Omologo and Y. Bengio",
  title= "A network of deep neural networks for distant speech recognition",
  booktitle = "Proc. of ICASSP",
  pages="4880-4884",
  year = "2017"  
}

@ARTICLE{jointraining,
  author={Wang, Zhong-Qiu and Wang, DeLiang},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing}, 
  title={A Joint Training Framework for Robust Automatic Speech Recognition}, 
  year={2016},
  volume={24},
  number={4},
  pages={796-806},
  doi={10.1109/TASLP.2016.2528171}}

@inproceedings{mstyke,
  author = {Sehr, Armin and Hofmann, Christian and Maas, Roland  and Kellermann, Walter },
  booktitle = {Proc. of HSCMA 2011},
  pages = {196-200},
  title = {{Multi-style training of HMMS with stereo data for reverberation-robust speech recognition}}
}

@INPROCEEDINGS{dataaug, 
author={X. Cui and V. Goel and B. Kingsbury}, 
booktitle={Proc. of ICASSP 2014}, 
title={Data Augmentation for deep neural network acoustic modeling}, 
pages={5582-5586}
}

@INPROCEEDINGS{nakatani, 
author={T. Yoshioka and N. Ito and M. Delcroix and A. Ogawa and K. Kinoshita and M. Fujimoto and C. Yu and W. J. Fabian and M. Espi and T. Higuchi and S. Araki and T. Nakatani}, 
booktitle={Proc. ASRU 2015}, 
title={{The NTT CHiME-3 system: Advances in speech enhancement and recognition for mobile multi-microphone devices}}, 
pages={436-443}}


@INPROCEEDINGS{dataaug2, 
author={A. Ragni, K. Knill, S. Rath and M. Gales}, 
booktitle={Proc. of Interspeech 2014}, 
title={Data Augmentation for Low Resource Languages},  
pages={5582-5586}
}

@inproceedings{dataaug3,
  author    = {Tom Ko and
               Vijayaditya Peddinti and
               Daniel Povey and
               Sanjeev Khudanpur},
  title     = {Audio augmentation for speech recognition},
  booktitle = {Proc. of Interspeech 2015},
  pages     = {3586--3589}
}


@inproceedings{cont2,
  author = {Couvreur, Laurent and Couvreur, Christophe and Ris, Christophe},
  booktitle = {Proc. of Interspeech 2000},
  pages = {397-400},
  title = {{A corpus-based approach for robust ASR in reverberant environments.}},
}

@inproceedings{cont3,
  author = {Haderlein, Tino and N{\"o}th, Elmar and Herbordt, Wolfgang and Kellermann, Walter and Niemann, Heinrich},
  pages = {226-233},
  publisher = {Springer},
  series = {Lecture Notes in Computer Science},
  title = {{Using Artificially Reverberated Training Data in Distant-Talking ASR.}},
  volume = 3658,
  year = 2005
}


@article{Davis80-COP,
  author =    {Steven B. Davis and Paul Mermelstein},
  title =     {Comparison of Parametric Representation for Monosyllabic Word Recognition in Continuously Spoken Sentences},
  journal =   {IEEE Transactions on Acoustics, Speech and Signal Processing},
  volume =    {28},
  number =    {4},
  pages =     {357--366},
  year =      {1980}
}

@article{Rabiner89-ATO,
  author =    {Lawrence R. Rabiner},
  title =     {A Tutorial on Hidden {Markov} Models and Selected Applications in Speech Recognition},
  journal =   {Proceedings of the IEEE},
  volume =    {77}, 
  number =    {2},
  pages =     {257--286}, 
  year =      {1989}
}

@book{lideng,
  author =    {D. Yu and L. Deng},
  title =     {Automatic Speech Recognition - A Deep Learning Approach},
  publisher = {Springer},
  year =      {2015}
}




@inproceedings{YourName15-XXX,
  crossref =  {Interspeech15},
  author =    {Firstname1 Lastname1 and Firstname2 Lastname2 and Firstname3 Lastname3},
  title =     {Title of your {Interspeech} 2015 publication},
  pages =     {100--104}
}

@proceedings{Interspeech15,
  key =       {Interspeech},
  title =     {{Interspeech} 2015 -- 16\textsuperscript{th} Annual Conference of the International Speech Communication Association, September 6--10, Dresden, Germany, Proceedings},
  booktitle = {{Interspeech} 2015 -- 16\textsuperscript{th} Annual Conference of the International Speech Communication Association, September 6--10, Dresden, Germany, Proceedings},
  year =      {2015}
}

@InProceedings{P1,
  author = 	 "Jones, C.D. and Roberts, E.F. and Smith, A.B.",
  title = "Paper Title",
  booktitle = "Proc. Conference Name",
  address = "Location",
  year = 	 "Year",
  pages = 	 "1--10"
}


@inproceedings{Nishiura,
  author    = {Takanobu Nishiura and Yoshiki Hirano and Yuki Denda and Masato Nakayama},
  title     = {Investigations into early and late reflections on distant-talking
               speech recognition toward suitable reverberation criteria},
  booktitle = {Proc. of Interspeech},
  year      = {2007},
  pages     = {1082-1085},
}



@Book{B1,
  author = "Roberts, E.F. and Smith, A.B. and Jones, C.D.",
  title = "Book Title",
  publisher = "Publisher",
  year = "Year"
}

% REFS FROM LeMa06



@string{ieeeassp  = "IEEE Trans. Acoust. Speech Signal
                     Processing"}
@string{ieee_m_assp = "{IEEE} {ASSP} Magazine"}
@string{ieeetsa   = "IEEE Transactions on Audio, Speech, and Language Processing"}

@string{ieeetss = "IEEE Transactions on Speech and Audio Processing"}

@string{ieeesp    = "IEEE Transactions on Signal Processing"}

@string{ieeespl    = "IEEE Signal Processing Letters"}

@string{specom    = "Speech Communication"}

@string{jasa    = "Journal of the Acoustical Society of America"}

@string{icassp   = "Proc. International Conference on Acoustics, Speech, and Signal Processing (ICASSP)"}

@string{icslp   = "Proc. International Conference on Spoken Language Processing"}

@string{ieeesamsp="Proc. IEEE Sensor Array and Multichannel Signal Processing Workshop"}

@string{sp="Signal Processing"}

@string{interspeech = "Proc. Interspeech"}

@string{eurospeech = "Proc. Eurospeech"}

@string{eusipco = "Proc. European Signal Processing Conference (EUSIPCO)"}

@string{propor = "Proc. International Conference on Computational Processing of Portuguese Language (PROPOR)"}

@string{fala = "Proc. FALA"}

@string{dsp = "Digital Signal Processing"}

@STRING{IEEE_J_ASSP = {{IEEE} Trans. Acoust., Speech, Signal Process.}}

@Inproceedings{apasci,
  author= "B. Angelini and F. Brugnara and D. Falavigna and D. Giuliani and R. Gretter and M. Omologo",
  title= "Speaker independent continuous speech recognition using an acoustic-phonetic {I}talian corpus",
  booktitle = {ICSLP},
  year = "1994",
  pages= "1391--1394"
}


@Article{BovikMa93,
  author= "A. C. Bovik and P. Maragos and T. F. Quatieri",
  title= "{AM-FM} energy detection and separation in noise using multiband energy operators",
  journal = ieeesp,
  year = "1993",
  volume= "41",
  pages= "3245--3265",
  publisher = "IEEE"
}


@Article{dimitriadis06,
  author= "D. Dimitriadis and P. Maragos",
  title= "Continuous energy demodulation methods and application to speech analysis",
  journal = specom,
  year = "2006",
  volume= "48",
	number= "7",
  pages= "819--837"
}

 @inproceedings{xvector,
 title={X-vectors: Robust DNN Embeddings for Speaker Recognition},
 author={Snyder, D. and Garcia-Romero, D. and Sell, G. and Povey, D. and Khudanpur, S.},
 booktitle={Proc. of ICASSP},
 year={2018},
 }
 
 @article{e2e_spk_id,
 author = {Zhang, C. and Koishida, K. and Hansen, J.},
 title = {Text-Independent Speaker Verification Based on Triplet Convolutional Neural Network Embeddings},
 journal = {IEEE/ACM Trans. Audio, Speech and Lang. Proc.},
 volume = {26},
 number = {9},
 year = {2018},
 pages = {1633--1644},
} 

@INPROCEEDINGS{dnn_spk_rec_class1,
author={G. Heigold and I. Moreno and S. Bengio and N. Shazeer},
booktitle={Proc. of ICASSP},
title={End-to-end text-dependent speaker verification},
year={2016},
pages={5115-5119},
}

@inproceedings{spk_id_mfcc,
  author    = {D. Snyder and
               D. Garcia{-}Romero and
               D. Povey and
               S. Khudanpur},
  title     = {Deep Neural Network Embeddings for Text-Independent Speaker Verification},
  booktitle = {Proc. of Interspeech},
  pages     = {999--1003},
  year      = {2017}
}


@inproceedings{dnn_spk_rec_class3,
  author    = {D. Snyder and
               P. Ghahremani and
               D. Povey and
               D. Romero and
               Y. Carmiel and
               S. Khudanpur},
  title     = {Deep neural network-based speaker embeddings for end-to-end speaker
               verification},
  booktitle = {Proc. of {SLT}},
  pages     = {165--170},
  year      = {2016}
}

@INPROCEEDINGS{kaldi_short,
         author = {Povey, D. and others},
          title = {{The Kaldi Speech Recognition Toolkit}},
      booktitle = {Proc. of ASRU},
           year = {2011}
}

@INPROCEEDINGS{sidekit,
author={A. Larcher and K. A. Lee and S. Meignier},
booktitle={Proc. of ICASSP},
title={An extensible speaker identification sidekit in Python},
year={2016},
pages={5095-5099},
}

@INPROCEEDINGS{dnn_spk_rec_class2,
author={E. Variani and X. Lei and E. McDermott and I. L. Moreno and J. Gonzalez-Dominguez},
booktitle={Proc. of ICASSP},
title={Deep neural networks for small footprint text-dependent speaker verification},
year={2014},
pages={4052-4056},
}

@inproceedings{palaz_raw,
  author = {Palaz, D. and Magimai-Doss, M. and Collobert, R.},
  booktitle = {Proc. of Interspeech},
  title = {{Analysis of CNN-based speech recognition system using raw speech as input}},
  year = 2015
}

@Article{dimitriadis05,
  author= "D. Dimitriadis and P. Maragos and A. Potamianos",
  title= "Robust {AM-FM} features for speech recognition",
  journal = ieeespl,
  year = "2005"
}


@Inproceedings{gridnews,
  author= "D. Dimitriadis and A. Metallinou and I. Konstantinou and G. Goumas and P. Maragos and N. Koziris",
  title= "{GRIDNEWS}: A distributed automatic {G}reek broadcast transcription system",
  booktitle = icassp,
  year = "2009"
}


@Article{gevag06,
  author= "G. Evangelopoulos and P. Maragos",
  title= "Multiband modulation energy tracking for noisy speech detection",
  journal = ieeetsa,
  year = "2006",
  volume= "14",
	number= "6",
  pages= "2024--2038"
}


@Article{DIRHA_D2.2,
  author= {M. Hagm\"{u}ller and others},
  title= "Experimental task definitions",
  journal = "Deliverable D2.2, DIRHA Consortium",
  month = feb,
  year = "2013"
}

@Article{DIRHA_D2.3,
  title= "Simulated acoustic corpora {II}",
  journal = "Deliverable D2.3, DIRHA Consortium",
  year = "2014"
}


@Article{DIRHA_D4.1,
  author= {G.Potamianos and others},
  title= "Robustness of distant--speech recognition and speaker identification-development of baseline system",
  journal = "Deliverable D4.1, DIRHA Consortium",
  month = feb,
  year = "2013"
}

@InProceedings{voxceleb,
  author       = "Nagrani, A. and Chung, J.~S. and Zisserman, A.",
  title        = "VoxCeleb: a large-scale speaker identification dataset",
  booktitle    = "Proc. of Interspech",
  year         = "2017",
}

@article{wang2021voxpopuli,
  title={VoxPopuli: A Large-Scale Multilingual Speech Corpus for Representation Learning, Semi-Supervised Learning and Interpretation},
  author={Wang, Changhan and Rivi{\`e}re, Morgane and Lee, Ann and Wu, Anne and Talnikar, Chaitanya and Haziza, Daniel and Williamson, Mary and Pino, Juan and Dupoux, Emmanuel},
  journal={arXiv preprint arXiv:2101.00390},
  year={2021}
}

@inproceedings{voxceleb2,
  author    = {Joon Son Chung and
               Arsha Nagrani and
               Andrew Zisserman},
  editor    = {B. Yegnanarayana},
  title     = {VoxCeleb2: Deep Speaker Recognition},
  booktitle = {Proc. of Interspeech},
  pages     = {1086--1090},
  publisher = {{ISCA}},
  year      = {2018},
}

@INPROCEEDINGS{FITPUB12224,
   author = "Hossein Zeinali and Shuai Wang and Anna Silnova and Pavel Mat\v{e}jka and Old\v{r}ich Plchot",
   title = "BUT System Description to VoxCeleb Speaker Recognition Challenge 2019",
   pages = "1--4",
   booktitle = "Proceedings of The VoxCeleb Challange Workshop 2019",
   year = 2019,
   location = "Graz, AT",
   language = "english",
   url = "https://www.fit.vut.cz/research/publication/12224"
}

@misc{pal21-meta,
      title={Meta-learning with Latent Space Clustering in Generative Adversarial Network for Speaker Diarization}, 
      author={Monisankha Pal and Manoj Kumar and Raghuveer Peri and Tae Jin Park and So Hyun Kim and Catherine Lord and Somer Bishop and Shrikanth Narayanan},
      year={2020},
      eprint={2007.09635},
      archivePrefix={arXiv},
      primaryClass={eess.AS},
      note = {arXiv:2007.09635}
}

@INPROCEEDINGS{Mccowan05theami,
    author = {I. Mccowan and G. Lathoud and M. Lincoln and A. Lisowska and W. Post and D. Reidsma and P. Wellner},
    title = {The AMI Meeting Corpus},
    booktitle = {In Proc. of the International Conference on Methods and Techniques in Behavioral Research},
    year = {2005}
}

@inproceedings{voxceleb_res,
  author    = {N. Le and
               J.{-}M. Odobez},
  title     = {Robust and Discriminative Speaker Embedding via Intra-Class Distance
               Variance Regularization},
  booktitle = {Proc. of Interspeech},
  pages     = {2257--2261},
  year      = {2018}
}

@Inproceedings{hermansky92,
  author= "H. Hermansky and N. Morgan and A. Bayya and P. Kohn",
  title= "{RASTA-PLP} speech analysis technique",
  booktitle = icassp,
  year = "1992"
}

@article{layer_norm,
  author    = {J. Ba and
               R. Kiros and
               G. E. Hinton},
  title     = {Layer Normalization},
  journal   = {CoRR},
  volume    = {abs/1607.06450},
  year      = {2016}
}

@Inproceedings{ravanelli,
  author= "M. Ravanelli and A. Sosi and P. Svaizer and M. Omologo",
  title= "Impulse response estimation for robust speech recognition in a reverberant environment",
  booktitle = "Proc. of EUSIPCO",
  pages="1668--1672",
  year = "2012"  
}

@inproceedings{GaoDDL15,
  author = {Gao, Tian and Du, Jun and Dai, Li-Rong and Lee, Chin-Hui},
  booktitle = {Proc. of ICASSP},
  title = {Joint training of front-end and back-end deep neural networks for robust speech recognition.},
  year = 2015
}

@inproceedings{hugging,
    title = "Transformers: State-of-the-Art Natural Language Processing",
    author = "Wolf, Thomas  and
      Debut, Lysandre  and
      Sanh, Victor  and
      Chaumond, Julien  and
      Delangue, Clement  and
      Moi, Anthony  and
      Cistac, Pierric  and
      Rault, Tim  and
      Louf, Remi  and
      Funtowicz, Morgan  and
      Davison, Joe  and
      Shleifer, Sam  and
      von Platen, Patrick  and
      Ma, Clara  and
      Jernite, Yacine  and
      Plu, Julien  and
      Xu, Canwen  and
      Le Scao, Teven  and
      Gugger, Sylvain  and
      Drame, Mariama  and
      Lhoest, Quentin  and
      Rush, Alexander",
    booktitle = "Proc of EMNLP",
    year = "2020",
}


@article{rethinking,
  author    = {Tatiana Likhomanenko and
               Qiantong Xu and
               Vineel Pratap and
               Paden Tomasello and
               Jacob Kahn and
               Gilad Avidov and
               Ronan Collobert and
               Gabriel Synnaeve},
  title     = {Rethinking Evaluation in {ASR:} Are Our Models Robust Enough?},
  journal   = {CoRR},
  volume    = {abs/2010.11745},
  year      = {2020},
}

@inproceedings{Chen2015sep,
author = {Chen, Z. and Watanabe, S. and Erdogan, H. and Hershey, J.R.},
title = {Speech Enhancement and Recognition Using Multi-Task Learning of Long Short-Term Memory Recurrent Neural Networks},
booktitle = {Proc. of Interspeech},
year = 2015,
}

@Inproceedings{ravanelli_SLT,
  author= "M. Ravanelli and P. Brakel and M. Omologo and Y. Bengio",
  title= {{Batch-normalized joint training for DNN-based distant speech recognition}},
  booktitle = "Proc. of SLT",
  year = "2016"  
}

@Inproceedings{sincnet_irasl,
  author= "M. Ravanelli and Y.Bengio",
  title= {{Interpretable Convolutional Filters with SincNet}},
  booktitle = "Proc. of NIPS@IRASL",
  year = "2018"  
}

@inproceedings{qrnn,
  author    = {Titouan Parcollet and
               Mirco Ravanelli and
               Mohamed Morchid and
               Georges Linar{\`{e}}s and
               Chiheb Trabelsi and
               Renato De Mori and
               Yoshua Bengio},
  title     = {Quaternion Recurrent Neural Networks},
  booktitle = {Proc. of ICLR},
  year      = {2019},
}

@inproceedings{complex,
  author    = {Chiheb Trabelsi and
               Olexa Bilaniuk and
               Ying Zhang and
               Dmitriy Serdyuk and
               Sandeep Subramanian and
               Jo{\~{a}}o Felipe Santos and
               Soroush Mehri and
               Negar Rostamzadeh and
               Yoshua Bengio and
               Christopher J. Pal},
  title     = {Deep Complex Networks},
  booktitle = {Proc. of ICLR},
  publisher = {OpenReview.net},
  year      = {2018},
}

@Inproceedings{pytorch_kaldi,
  author= "M. Ravanelli and T. Parcollet and Y. Bengio",
  title= {{The PyTorch-Kaldi Speech Recognition Toolkit}},
  booktitle = "Submitted to ICASSP",
  year = "2019"  
}

@Inproceedings{pytorch_kaldi,
  author= "M. Ravanelli and T. Parcollet and Y. Bengio",
  title= {{The PyTorch-Kaldi Speech Recognition Toolkit}},
  booktitle = "Proc. of ICASSP",
  year = "2019"  
}

@Inproceedings{AISV,
  author= "M. Ravanelli and A. Sosi and M. Matassoni and M. Omologo and M. Benetti and G. Pedrotti",
  title= "DISTANT TALKING SPEECH RECOGNITION IN SURGERY ROOM : THE {DOMHOS} PROJECT",
  booktitle = "AISV",
  year = "2013"
}


@article{convtasnet,
  author    = {Yi Luo and
               Nima Mesgarani},
  title     = {Conv-TasNet: Surpassing Ideal Time-Frequency Magnitude Masking for
               Speech Separation},
  journal   = {{IEEE} {ACM} Trans. Audio Speech Lang. Process.},
  volume    = {27},
  number    = {8},
  pages     = {1256--1266},
  year      = {2019},
}


@misc{luo2020dualpath,
      title={Dual-path RNN: efficient long sequence modeling for time-domain single-channel speech separation}, 
      author={Yi Luo and Zhuo Chen and Takuya Yoshioka},
      year={2020},
      eprint={1910.06379},
      archivePrefix={arXiv},
      primaryClass={eess.AS}
}

@inproceedings{transformers,
 author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
 booktitle = {Advances in Neural Information Processing Systems},
 title = {Attention is All you Need},
 volume = {30},
 year = {2017}
}


@inproceedings{convs2s,
  title={Convolutional sequence to sequence learning},
  author={Gehring, Jonas and Auli, Michael and Grangier, David and Yarats, Denis and Dauphin, Yann N},
  booktitle={International Conference on Machine Learning},
  pages={1243--1252},
  year={2017},
  organization={PMLR}
}

@article{pedregosa2011scikit,
  title={Scikit-learn: Machine learning in Python},
  author={Pedregosa, Fabian and Varoquaux, Ga{\"e}l and Gramfort, Alexandre and Michel, Vincent and Thirion, Bertrand and Grisel, Olivier and Blondel, Mathieu and Prettenhofer, Peter and Weiss, Ron and Dubourg, Vincent and others},
  journal={the Journal of machine Learning research},
  volume={12},
  pages={2825--2830},
  year={2011},
  publisher={JMLR. org}
}

@article{howard2020fastai,
  title={Fastai: A layered API for deep learning},
  author={Howard, Jeremy and Gugger, Sylvain},
  journal={Information},
  volume={11},
  number={2},
  pages={108},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@misc{sepformer,
      title={Attention is All You Need in Speech Separation}, 
      author={Cem Subakan and Mirco Ravanelli and Samuele Cornell and Mirko Bronzi and Jianyuan Zhong},
      year={2021},
      booktitle = "Proc. of ICASSP",
}

@misc{ecapa_diarization,
      title={{ECAPA-TDNN} Embeddings for Speaker Diarization},
      author={Nauman Dawalatabad and Mirco Ravanelli and Francois Grondin and Jenthe Thienpondt and Brecht Desplanques and Hwidong Na},
        year={2021},
      eprint={2104.01466},
      archivePrefix={arXiv},
      primaryClass={eess.AS},
      note={arXiv:2104.01466}
}

@inproceedings{deepclustering,
title = {Deep clustering: Discriminative embeddings for segmentation and separation},
author = "Hershey, {John R.} and Zhuo Chen and {Le Roux}, Jonathan and Shinji Watanabe",
year = "2016",
booktitle = "Proc. of ICASSP",
}


@article{timers-and-such,
  author    = {Loren Lugosch and
               Piyush Papreja and
               Mirco Ravanelli and
               Abdelwahab Heba and
               Titouan Parcollet},
  title     = {Timers and Such: {A} Practical Benchmark for Spoken Language Understanding
               with Numbers},
  journal   = {CoRR},
  volume    = {abs/2104.01604},
  year      = {2021},
}

@inproceedings{slurp,
    author = {Emanuele Bastianelli and Andrea Vanzo and Pawel Swietojanski and Verena Rieser},
    title={{SLURP: A Spoken Language Understanding Resource Package}},
    booktitle={{Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)}},
    year={2020}
}

@article{Serdyuk2018,
author = {Serdyuk, Dmitriy and Wang, Yongqiang and Fuegen, Christian and Kumar, Anuj and Liu, Baiyang and Bengio, Yoshua},
eprint = {1802.08395},
journal = {ICASSP},
title = {{Towards end-to-end spoken language understanding}},
year = {2018}
}

@article{Haghani2018,
author = {Haghani, Parisa and Narayanan, Arun and Bacchiani, Michiel and Chuang, Galen and Gaur, Neeraj and Moreno, Pedro and Prabhavalkar, Rohit and Qu, Zhongdi and Waters, Austin},
title = {{From Audio to Semantics: Approaches to end-to-end spoken language understanding}},
journal = {IEEE Spoken Language Technology Workshop (SLT)},
year = {2018}
}

@misc{k2,
  author = {Povey, Daniel and others},
  title = {k2},
  year = {2020},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {\url{https://github.com/k2-fsa/k2}}
}


@article{seo2021integration,
  title={Integration of Pre-trained Networks with Continuous Token Interface for End-to-End Spoken Language Understanding},
  author={Seo, Seunghyun and Kwak, Donghyun and Lee, Bowon},
  journal={arXiv preprint arXiv:2104.07253},
  year={2021}
}

@article{hannun2017sequence,
  author = {Hannun, Awni},
  title = {Sequence Modeling with {CTC}},
  journal = {Distill},
  year = {2017},
  note = {https://distill.pub/2017/ctc},
  doi = {10.23915/distill.00008}
}

@inproceedings{fluent,
      title={Speech Model Pre-training for End-to-End Spoken Language Understanding}, 
      author={Loren Lugosch and Mirco Ravanelli and Patrick Ignoto and Vikrant Singh Tomar and Yoshua Bengio},
      year={2019},
      booktitle = "Proc. of InterSpeech",
      
}

@article{gsc,
   author = { {Warden}, P.},
    title = "{Speech Commands: A Dataset for Limited-Vocabulary Speech Recognition}",
  journal = {ArXiv e-prints},
  archivePrefix = "arXiv",
  eprint = {1804.03209},
  primaryClass = "cs.CL",
  keywords = {Computer Science - Computation and Language, Computer Science - Human-Computer Interaction},
    year = 2018,
    month = apr,
    url = {https://arxiv.org/abs/1804.03209},
}

@Inproceedings{hscma1,
  author= "M. Omologo and P. Svaizer and A. Brutti and L. Cristoforetti",
  title= "Speaker localization in {CHIL} lectures: Evaluation criteria and results",
  booktitle = "Machine Learning for Multimodal Interaction, pp. 47-487",
  year = "Springer, 2006"
}

@article {chil_corpus,
	title = {{The CHIL Audiovisual Corpus for Lecture and Meeting Analysis inside Smart Rooms}},
	journal = {Language resources and evaluation},
	volume = {41},
	number = {3},
	year = {2007},
	month = {01/2008},
	pages = {389--407},
	author = {Mostefa, D. and Moreau, N. and Choukri, K. and Potamianos, G. and Chu, S. and Tyagi, A. and Casas, J. and Turmo, J. and Cristoforetti, L. and Tobia, F. and Pnevmatikakis, A. and Mylonakis, V. and Talantzis, F. and Burger, S. and Stiefelhagen, R. and Bernardin, K. and Rochet, C.}
}

@Inproceedings{hscma2,
  author= "A. Temko and R. Malkin and C. Zieger and D. Mascho and C. Nadeu and M. Omologo",
  title= "Clear evaluation of acoustic event detection and classification systems",
  booktitle = "Proceedings of the 1st International Evaluation Conference on Classification of Events, Activities and Relationships",
  year = "2007, CLEAR 06, Springer-Verlag"
}


@Inproceedings{hscma,
  author= "A. Brutti and M. Ravanelli and P. Svaizer and M. Omologo",
  title= "A SPEECH EVENT DETECTION/LOCALIZATION TASK FOR MULTIROOM ENVIRONMENTS",
  booktitle = "Proc. of HSCMA 2014",
  pages="157--161 "
}


@Inproceedings{aura,
  author= "M. Vorlander",
  title= "Auralization",
  booktitle = "Springer",
  year = "2007"
}


@Book{kutt,
  author = "H. Kuttruff",
  title = "Room acoustic",
  edition   = 5,
  publisher = "Spon Press",
  year = "2009"
}








@INPROCEEDINGS{farina,
    author = {Angelo Farina},
    title = {Simultaneous Measurement of Impulse Response and Distortion With a Swept-Sine Technique},
    booktitle = {Proc. of the 108th AES Convention},
    year = {2000},
    pages = {18--22}
}


@article{matassoni,
  author = {Matassoni, Marco and Omologo, Maurizio and Giuliani, Diego and Svaizer, Piergiorgio},
  journal = {{Computer Speech \& Language}},
  number = 2,
  pages = {205-223},
  title = {{Hidden Markov model training with contaminated speech material for distant-talking speech recognition.}},
  volume = 16,
  year = 2002
}

@incollection{yann,
  title={Efficient backprop},
  author={LeCun, Y. and Bottou, L. and Orr, G. and M{\"u}ller, K.},
  booktitle={Neural networks: Tricks of the trade},
  pages={9--50},
  year={1998},
  publisher={Springer Berlin Heidelberg}
}

@Inproceedings{lrec,
  author= "L. Cristoforetti and M. Ravanelli and M. Omologo and A. Sosi and A. Abad and M. Hagmueller and P. Maragos",
  title= "The {DIRHA} simulated corpus",
  booktitle = "Proc. of LREC 2014",
  pages={2629-2634}
}


@Inproceedings{brutti,
  author= "A. Brutti and M. Matassoni",
  title= "{On the use of Early-to-Late Reverberation Ratio for ASR in reverberant environments}",
  booktitle = "Proc. of ICASSP 2014",
  year = "2014",
  pages={4670-4675}
}





@Incollection{kaiser83,
  author= "J. F. Kaiser",
  title= "Some observations on vocal tract operation from a fluid flow point of view",
  booktitle = "Vocal Fold Physiology: Biomechanics, Acoustics, and Phonatory Control",
  editor = "I. R. Titze and R. C. Scherer",
  year = "1983",
  pages= "358--386",
  publisher = "Denver Center for Performing Arts",
  address = "Denver, CO"
}


@Inproceedings{lee+1993,
  author= "C. H. Lee and J. L. Gauvain",
  title= "Speaker adaptation based on {MAP} estimation of {HMM} parameters",
  booktitle = icassp,
  year = "1993",
  volume= "2",
  pages= "558--561"
}


@Article{leggetter+1995,
  author= "C. J. Leggetter and P. C. Woodland",
  title= "Maximum likelihood linear regression for speaker adaptation of continuous density hidden {M}arkov models",
  journal = "Computer Speech \& Language",
  year = "1995",
  volume= "9",
	number= "2",
  pages= "171--185"
}

@Article{maragos93,
  author= "P. Maragos and J. F. Kaiser and T. F. Quatieri",
  title= "Energy separation in signal modulations with application to speech analysis",
  journal = ieeesp,
  year = "1993",
  volume= "41",
	number= "10",
  pages= "3024--3051"
}

@inproceedings{google_rawmulti,
title	= {Speech Acoustic Modeling from Raw Multichannel Waveforms},
author	= {Y. Hoshen and R. Weiss and K. W. Wilson},
year	= {2015},
booktitle	= {Proc. of ICASSP}
}

@article{spoofing_raw,
  title={{End-to-end spoofing detection with raw waveform CLDNNS}},
  author={H. Dinkel and N. Chen and Y. Qian and K. Yu},
  journal={Proc. of ICASSP},
  year={2017},
}



@inproceedings{attention_asr,
  author    = {D. Bahdanau and
               J. Chorowski and
               D. Serdyuk and
               P. Brakel and
               Y. Bengio},
  title     = {End-to-end attention-based large vocabulary speech recognition},
  booktitle = {Proc. of ICASSP},
  pages     = {4945--4949},
  year      = {2016},
}

@article{bahdanau2014neural,
  title={Neural machine translation by jointly learning to align and translate},
  author={Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
  journal={ICLR},
  year={2015}
}

@inproceedings{tuske,
  title={{Acoustic modeling with deep neural networks using raw time signal for LVCSR}},
  author={Z. T{\"u}ske and P. Golik and R. Schl{\"u}ter and H. Ney},
  booktitle={Proc. of Interspeech},
  year={2014}
}

@inproceedings{wavenet,
title	= {WaveNet: A Generative Model for Raw Audio},
author	= {A. van den Oord and S. Dieleman and H. Zen and K. Simonyan and O. Vinyals and A. Graves and N. Kalchbrenner and A. Senior and K. Kavukcuoglu},
year	= {2016},
URL	= {https://arxiv.org/abs/1609.03499},
booktitle	= {Arxiv}
}

@article{sample_rnn,
  author    = {S. Mehri and
               K. Kumar and
               I. Gulrajani and
               R. Kumar and
               S. Jain and
               J. Sotelo and
               A. C. Courville and
               Y. Bengio},
  title     = {SampleRNN: An Unconditional End-to-End Neural Audio Generation Model},
  journal   = {CoRR},
  volume    = {abs/1612.07837},
  year      = {2016}
}




@inproceedings{dnn_speech_sep,
  author    = {P. Huang and
               M. Kim and
               M. Johnson and
               P. Smaragdis},
  title     = {Deep learning for monaural speech separation},
  booktitle = {Proc. of {ICASSP}},
  pages     = {1562--1566},
  year      = {2014}
}




@Article{DIRHA_D1.2,
  author= "M. Matassoni and others",
  title= "Definition of the evaluation plan",
  journal = "Deliverable D1.2, DIRHA Consortium",
  month = aug,
  year = "2012"
}


@Inproceedings{bdpublico,
  author= "J. P. Neto and C. A. Martins and H. Meinedo and L. B. Almeida",
  title= "The design of a large vocabulary speech corpus for {P}ortuguese",
  booktitle = eurospeech,
  year = "1997",
  pages= "1707--1710"
}

@Inproceedings{potamianos94,
  author= "A. Potamianos and P. Maragos",
  title= "Speech processing applications using {AM-FM} models and energy operators",
  booktitle = eusipco,
  year = "1994",
  volume= "3",
  pages= "1669--1672"
}

@Book{rabiner11,
  author= "L. R. Rabiner and R. W. Schafer",
  title= "Theory and Applications of Digital Speech Processing",
  publisher = "Prentice Hall, NJ",
  year = "2011"
}


@Book{BrandWard,
  author= "M. Brandstein and D. Ward",
  title= "Microphone arrays",
  publisher = "Springer, Berlin",
  year = "2000"
}


@Book{adverse,
  author= "E. H{\"a}nsler and G. Schmidt ",
  title= "Speech and Audio Processing in Adverse Environments",
  publisher = "Springer",
  year = "2008"
}



    



@Inproceedings{cmutools,
  author= "R. Rosenfield and P. Clarkson",
  title= "Statistical language modeling using the {CMU}-{C}ambridge toolkit",
  booktitle = eurospeech,
  year = "1997"
}

@misc{BAScorpus,
  author        = "F. Schiel and A. Baumann",
  title         = "{PhonDat1} Corpus Documentation",
  url          = "http://www.phonetik.uni-muenchen.de/Bas/BasPD1README"
}

@Inproceedings{srilm,
  author= "A. Stolcke",
  title= "{SRILM} - An extensible language modeling toolkit",
  booktitle = icslp,
  year = "2002"
}




@Inproceedings{Szoke2005,
  author= {I. Sz\"{o}ke and P. Schwarz and P. Mat\v{e}jka and L. Burget and M. Karafi\'{a}t and M. Fap\v{s}o and J. \v{C}ernock\'{y}},
  title= "Comparison of keyword spotting approaches for informal continuous speech",
  booktitle = interspeech,
  year = "2005",
  pages= "633--636"
}


@Inproceedings{woodland:94,
  author= "P. C. Woodland and J. J. Odell and V. Valtchev and S. J. Young",
  title= "Large vocabulary continuous speech recognition using {HTK}",
  booktitle = icassp,
  year = "1994",
  volume= "2",
  pages= "125--128"
}

@Manual{htkbook,
  author = "S. Young and others",
  title = "{HTK} -- Hidden {M}arkov Model Toolkit", 
  howpublished = "Manual",
  url = "http://htk.eng.cam.ac.uk/",
  year = "2006"
}

@Inproceedings{nzlat12,
  author= "A. Zlatintsi and P. Maragos",							
  title= "{AM-FM} modulation features for music instrument signal analysis and recognition",
  booktitle = eusipco,
  year = "2012"
}

@misc{sampa,
  author        = "S. Young and others",
  title         = "{SAMPA} - Computer Readable Phonetic Alphabet",
  url = "http://www.phon.ucl.ac.uk/home/sampa/"
}


@Inproceedings{Abad2008,
  author= "A. Abad and J. Paulo da Silva Neto",							
  title= "Automatic classification and transcription of telephone speech in radio {B}roadcast data",
  booktitle= propor,
  year = "2008"
}


@Inproceedings{Abad2009,
  author= "A. Abad and I. Trancoso and N. Neto and M. do C\'{e}u Guerreiro Viana Ribeiro",							
  title= "Porting an {E}uropean {P}ortuguese {B}roadcast News Recognition System to {B}razilian {P}ortuguese",
  booktitle= interspeech,
  year = "2009"
}


@Article{Abad2012a,
  author= "A. Abad and A. Pompili and A. Costa and I. Trancoso and J. Fonseca and G. Leal and L. Farrajota and I.P. Martins",							
  title= "Automatic word naming recognition for an on-line aphasia treatment system",
  journal= "Computer Speech \& Language",
  year = "2012"
}


@inproceedings{ecapa,
  author    = {Brecht Desplanques and
               Jenthe Thienpondt and
               Kris Demuynck},
  editor    = {Helen Meng and
               Bo Xu and
               Thomas Fang Zheng},
  title     = {{ECAPA-TDNN:} Emphasized Channel Attention, Propagation and Aggregation
               in {TDNN} Based Speaker Verification},
  booktitle = {Proc. of InterSpeech},
  year      = {2020},
}

@Inproceedings{Abad2012b,
  author= "A. Abad and H. Meinedo and I. Trancoso and J. Paulo da Silva Neto",							
  title= "Transcription of Multi-Variety {P}ortuguese Media Contents",
  booktitle= propor,
  year = "2012"
}


@Inproceedings{Adami2010,
  author= "A. G. Adami",							
  title= "Automatic speech recognition: from the beginning to {P}ortuguese language",
  booktitle = propor,
  year = "2010"
}


%%%% ISIDOROS


@Inproceedings{Koller2010,
	author= {O. Koller and A. Abadand and I. Trancoso and M. do Ceu Guerreiro Viana Ribeiro}, 
	title= "Exploiting Variety-Dependent Phones in {P}ortuguese Variety Identification Applied to Broadcast News Transcription",
    booktitle = interspeech,
    year= "2010"      
}
          
@Inproceedings{Lopes2012,
	author="J. Lopes and M. Eskenazi and I. Trancoso",
	title= "Incorporating {ASR} information in Spoken Dialog System confidence score",
	booktitle= propor,
	year=2012
}


@Inproceedings{Meinedo2003,
	author="H. Meinedo and D. Ant\'{o}nio Caseiro and J. Paulo da Silva Neto and I. Trancoso", 
	title="{AUDIMUS}.media: a Broadcast News speech recognition system for the {E}uropean {P}ortuguese language",
	booktitle=propor,
	year="2003"
}	

@Inproceedings{Meinedo2008,
	author="H. Meinedo and A. Abad and T. Pellegrini and I. Trancoso and J. Paulo da Silva Neto", 
	title="The {L2F} Broadcast News Speech Recognition System", 
	booktitle=fala,
	month = nov,
	year=2010,
	address = "Vigo, Spain"
}

@Inproceedings{Neves2008,
	author="Luis Miguel Leitao Neves and Ciro Alexandre Domingues Martins and Hugo Meinedo and Joao Paulo da Silva Neto", 
	title="Domain adaptation of a Broadcast News Transcription System
			for the {P}ortuguese Parliament",
	booktitle=propor,
	year=2008
}


@Inproceedings{Trancoso2006,
	author="Isabel Trancoso and Ricardo Jorge Francisco Nunes and Luis Miguel Leitao Neves and Maria do C\'{e}u Guerreiro Viana Ribeiro and Helena Moniz and Diamantino Antonio Caseiro and Ana Isabel Mata da Silva",
	title="Recognition of Classroom Lectures in {E}uropean {P}ortuguese",
	booktitle= interspeech,
	pages="281--284",
	year="2006"
}
	 
@Inproceedings{word,
	author={L. Ferrer and E. Shriberg and S. Kajarekar and A. Stolcke and K. S\"{o}nmez and A. Venkataraman and H. Bratt},
	title="The contribution of cepstral and stylistic features to {SRI}'s 2005 {NIST} speaker recognition evaluation system",
	booktitle=icassp,
	year=2006,
	volume=1,
	pages="101--104"
}


@Inproceedings{duration,
	author={Ferrer, L. and Bratt, H. and Gadde, V. R. R. and Kajarekar, S. and Shriberg, E. and S\"{o}nmez, K. and Stolcke, A. and Venkataraman, A.},
	title="Modeling duration patterns for speaker recognition",
	booktitle=eurospeech,
	year=2003,
	pages="2017--2020",
	address="Geneva",
}

@Article{prosodic,
	author="Shriberg, E. and Ferrer, L. and Kajarekar, S. S. and Venkataraman, A. and Stolcke, A.",
	title="Modeling Prosodic Feature Sequences for Speaker Recognition",
	journal=specom,
	volume= 46,
	number = "3--4",
	pages= "455--472",
	year=2005
}

@Article{rasta,
	author="Hermansky, H. and Morgan, N.",
	title="{RASTA} processing of speech",
	journal=ieeetss,
	volume=2,
	number = "4",
	pages="578--589",
	month = oct,
	year=1994
}

%%
@Inproceedings{warping,
	author="Pelecanos, J. and Sridharan, S.",
	title="Feature warping for robust speaker verification",
	booktitle="Proc. of Odyssey Speaker and Language Recognition Workshop",
	year=2001,
        pages = "213--218"
}

@Inproceedings{gretter,
  author= "R. Gretter",
  title= "Euronews: a multilingual speech corpus for {ASR}",
  booktitle = "Proc. of LREC 2014",
  year=2014,
}

@Inproceedings{apasci1,
  author= "B. Angelini and F. Brugnara and D. Falavigna and D. Giuliani and R. Gretter and M. Omologo",
  title= "Speaker independent continuous speech recognition using an acoustic-phonetic {I}talian corpus",
  booktitle = "Proc. of ICSLP",
  year = "1994",
  pages= "1391--1394"
}

@Article{score,
	author="Auckenthaler, R. and Carey, M. J. and Lloyd-Thomas, H.",
	title="Score Normalization for Text-Independent Speaker Verification Systems",
	journal=dsp,
	volume=10,
	pages="42--54",
        number="1--3",
	year=2000
}
%
@Inproceedings{mllr,
	author="Stolcke, A. and Ferrer, L. and Kajarekar, S. and Shriberg, E. and Venkataraman, A.",
	title="{MLLR} transforms as features in speaker recognition",
	booktitle=eurospeech,
	pages="2425--2428",
	year=2005
}


@Inproceedings{image,
	author="J.B. Allen and D.A. Berkley",
	title="Image method for efficiently simulating small‐room acoustics",
	booktitle="J. Acoust. Soc. Am",
    pages="2425--2428",
	year=1979
}

    
@Inproceedings{mearev,
	author="M.R Schroeder",
	title="New Method of Measuring Reverberation Time",
	booktitle="J. Acoust. Soc. Am",
    pages="",
	year=1965
}


@Inproceedings{mls,
	author="M.R Schroeder",
	title={{Diffuse sound reflection by maximum-length
sequences}},
	booktitle="J. Acoust. Soc. Am",
    volume="57(1)",
    pages="149-150",
	year=1975
}
    
     
    
@Inproceedings{tnsvm,
	author="Abad, A. and Trancoso, I.",
	title="Speaker Recognition Experiments using Connectionist Transformation Network Features",
	booktitle=interspeech,
	year=2010,
	pages="378--381"
}
%%
@Article{gmm_ubm,
	author="Reynolds, D. A. and Quatieri, T. F. and Dunn, R. B.",
	title="Speaker verification using adapted {G}aussian mixture models",
	journal=dsp,
	volume=10,
        number="1--3",
	pages="19--41",
	year="2000"
}	

@Article{gsv,
	author="Campbell, W. M. and Sturim, D. E. and Reynolds, D. A.",
	title="Support vector machines using {GMM} supervectors for speaker verification",
	journal=ieeespl,
	volume=13,
	number=5,
	pages="308--311",
	year=2006
}	

@Inproceedings{ivector2,
	author="Dehak, N. and Dehak, R. and Kenny, P. and {Br\"{u}mmer}, N. and Ouellet, P. and Dumouchel, P.",
	title="Support vector machines versus fast scoring in the low-dimensional total variability space for speaker verification",
	booktitle=interspeech,
	year=2009,
	pages="1559--1562"
}

@ARTICLE{ivector,
author={N. Dehak and P. J. Kenny and R. Dehak and P. Dumouchel and P. Ouellet},
journal={IEEE Transactions on Audio, Speech, and Language Processing},
title={Front-End Factor Analysis for Speaker Verification},
year={2011},
volume={19},
number={4},
pages={788-798}}

@Inproceedings{LVP11,
  author = "Lecouteux, B. and Vacher, M. and Portet, F.",
  title = "Distant speech recognition in a smart home: {C}omparison of several multisource {ASR}s in realistic conditions",
  booktitle = interspeech,
  year = 2011,
  pages = "2273-2276"
}


@Article{jfa,
	author="Kenny, P. and Boulianne,  G. and Ouellet, P. and Dumouchel, P.",
	title="Joint factor analysis versus eigenchannels in speaker recognition",
	journal=ieeetsa,
	volume=15,
	number=4, 
	pages="1435--1447",
	year="2007"
}

@Inproceedings{dicit2008,
	author="M. Omologo",
	title="Front-end processing of a distant-talking speech interface for control of an interactive {TV} system",
	booktitle="Proc. of  Acoustics",
	year=2008,
	pages="1425--1429"
}

@Book{Goodfellow-et-al-2016-Book,
  author= "I. Goodfellow and Y. Bengio and A. Courville",
  title= "Deep Learning",
  publisher = "MIT Press",
  year = 2016
}

@article{gan,
title = {Generative Adversarial Nets},
author = {Goodfellow, I. and Pouget-Abadie, J. and Mirza, M. and Xu, B. and Warde-Farley, D. and Ozair, S. and Courville, A. and Bengio, Y.},
journal = {Proc. of NIPS},
pages = {2672--2680},
year = {2014},
}

@article{ganin,
 author = {Ganin, Y. and Ustinova, E. and Ajakan, H. and Germain, P. and Larochelle, H. and Laviolette, F. and Marchand, M. and Lempitsky, V.},
 title = {Domain-adversarial Training of Neural Networks},
 journal = {J. Mach. Learn. Res.},
 volume = {17},
 number = {1},
 month = jan,
 year = {2016},
 issn = {1532-4435},
 pages = {2096--2030},
} 



@ARTICLE{dima_invariant,
    author = {Serdyuk, D. and Brakel, P. and Ramabhadran, B. and Thomas, S. and Bengio, Y. and Audhkhasi, K.},
     title = {Invariant Representations for Noisy Speech Recognition},
   journal = {arXiv e-prints},
    volume = {abs/1612.01928},
      year = {2016},
}

@ARTICLE{philemon,
    author = {Brakel, P. and Bengio, Y.},
     title = {Learning Independent Features with Adversarial Nets for Non-linear ICA},
   journal = {arXiv e-prints},
    volume = {1710.05050},
      year = {2017},
}


@article{cpc_deepmind,
  author    = {A. van den Oord and
               Y. Li and
               O. Vinyals},
  title     = {Representation Learning with Contrastive Predictive Coding},
  journal   = {CoRR},
  volume    = {abs/1807.03748},
  year      = {2018}
}


@ARTICLE{devon_infomax,
    author = {Hjelm, R. D. and Fedorov, A. and Lavoie-Marchildon, S. and Grewal, K. and Trischler, A. and Bengio, Y.},
     title = {Learning deep representations by mutual information estimation and maximization},
   journal = {arXiv e-prints},
    volume = {1808.06670},
      year = {2018},
}


@InProceedings{mine,
  title = 	 {Mutual Information Neural Estimation},
  author = 	 {Belghazi, M. I. and Baratin, A. and Rajeshwar, S. and Ozair, S. and Bengio, Y. and Courville, A. and Hjelm, R. D.},
  booktitle = 	 {Proc. of ICML},
  pages = 	 {531--540},
  year = 	 {2018},
}

@INPROCEEDINGS{ami,
author={S. Renals and T. Hain and H. Bourlard},
booktitle={Proc. of HSCMA},
title={{Interpretation of Multiparty Meetings the AMI and Amida Projects}},
year={2008},
pages={115-118}
}

@INPROCEEDINGS{aspire,
author={M. Harper},
booktitle={Proc. of ASRU},
title={The Automatic Speech recogition In Reverberant Environments (ASpIRE) challenge},
year={2015},
pages={547-554}
}

@article {mi_ref,
	author = {Kinney, J. B. and Atwal, G. S.},
	title = {Equitability, mutual information, and the maximal information coefficient},
	volume = {111},
	number = {9},
	pages = {3354--3359},
	year = {2014},
	journal = {Proceedings of the National Academy of Sciences}
}


@article{mi_comp,
 author = {Paninski, L.},
 title = {Estimation of Entropy and Mutual Information},
 journal = {Neural Comput.},
 volume = {15},
 number = {6},
 month = jun,
 year = {2003},
 pages = {1191--1253},
} 


@book{applebaum_book, 
edition={2}, 
title={Probability and Information: An Integrated Approach}, 
publisher={Cambridge University Press}, 
author={Applebaum, D.}, 
year={2008}
}

@Inproceedings{fakotakis97,
	author="Chatzi, I. and Fakotakis, N. and Kokkinakis, G.",
	title="Greek speech database for creation of voice driven teleservices",
	booktitle=eurospeech,
	year=1997
}	 

@Inproceedings{fakotakis09,
	author="Mporas, I. and Ganchev, T. and Kostoulas, T. and Kermanidis, K. and Fakotakis, N.",
	title="Automatic Speech Recognition System for Home Appliances Control",
	booktitle="Proc. 13th Panhellenic Conference on Informatics (PCI)",
	year=2009,
	pages="114--117",
}	
%
@Inproceedings{oikonomidis03,
	author="Oikonomidis, D. and Digalakis, V.",
	title="Stem-based Maximum Entropy Language Models for Inflectional Languages",
	booktitle=eurospeech,
	year=2003
}	

@Article{digalakis66,
	author="Digalakis, V. and Monaco, P. and Murveit, H.",
	title="Genones: Generalized Mixture Tying in Continuous Hidden {M}arkov Model-Based Speech Recognizers",
	 journal=ieeetss,
	 pages="281--289",
	 month=jul,
	 year=1996
}


@Article{chsel,
	author="M. Wolf and C. Nadeu",
	title="Channel selection measures for multi-microphone speech recognition",
	 journal="Speech Communication",
	 pages="170--180",
     volume= "57",
	 year=2014
}

@Inproceedings{Meinedo2010,
	author="H. Meinedo and A. Abad and T. Pellegrini and I. Trancoso and J. Neto",
	title="The {L2F} {B}roadcast news speech recognition system",
	booktitle="Proc. FALA",
	year=2010
}	

@Book{JurafskyMartin09,
  author= "D. Jurafsky and Martin, J. H.",
  title= "Speech and Language Processing. An Introduction to Natural Language Processing, Computational Linguistics, and Speech Recognition",
  publisher = "Pearson",
  year = 2009
}


@inproceedings{graves_ctc,
 author = {Graves, A. and Jaitly, N.},
 title = {Towards End-to-end Speech Recognition with Recurrent Neural Networks},
 booktitle = {Proc. of ICML},
 year = {2014},
 pages = {1764--1772},
}

@inproceedings{CTC,
  title={Connectionist temporal classification: labelling unsegmented sequence data with recurrent neural networks},
  author={Graves, Alex and Fern{\'a}ndez, Santiago and Gomez, Faustino and Schmidhuber, J{\"u}rgen},
  booktitle={Proceedings of the 23rd international conference on Machine learning},
  pages={369--376},
  year={2006}
}

@article{lingvo,
  title={Lingvo: a modular and scalable framework for sequence-to-sequence modeling},
  author={Shen, Jonathan and Nguyen, Patrick and Wu, Yonghui and Chen, Zhifeng and Chen, Mia X and Jia, Ye and Kannan, Anjuli and Sainath, Tara and Cao, Yuan and Chiu, Chung-Cheng and others},
  journal={arXiv preprint arXiv:1902.08295},
  year={2019}
}

@inproceedings{wav2vect,
 author = {Baevski, Alexei and Zhou, Yuhao and Mohamed, Abdelrahman and Auli, Michael},
 booktitle = {Proc. of NeurIPS},
 title = {wav2vec 2.0: A Framework for Self-Supervised Learning of Speech Representations},
 year = {2020}
}

@inproceedings{sentencepiece,
    title = "{S}entence{P}iece: A simple and language independent subword tokenizer and detokenizer for Neural Text Processing",
    author = "Kudo, Taku  and
      Richardson, John",
    booktitle = "Proceedings of EMNLP",
    year = "2018",
}

@ARTICLE{hybrid_ctc_att,
  author={Watanabe, Shinji and Hori, Takaaki and Kim, Suyoun and Hershey, John R. and Hayashi, Tomoki},
  journal={IEEE Journal of Selected Topics in Signal Processing}, 
  title={Hybrid CTC/Attention Architecture for End-to-End Speech Recognition}, 
  year={2017},
  volume={11},
  number={8},
  pages={1240-1253}
  }
  
@article{graves_transducer,
  author    = {Alex Graves},
  title     = {Sequence Transduction with Recurrent Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1211.3711},
  year      = {2012},
}


@inproceedings{espnet_se,
  author    = {Chenda Li and
               Jing Shi and
               Wangyou Zhang and
               Aswin Shanmugam Subramanian and
               Xuankai Chang and
               Naoyuki Kamo and
               Moto Hira and
               Tomoki Hayashi and
               Christoph B{\"{o}}ddeker and
               Zhuo Chen and
               Shinji Watanabe},
  title     = {ESPnet-SE: End-To-End Speech Enhancement and Separation Toolkit Designed
               for {ASR} Integration},
  booktitle = {Proc. of the IEEE Spoken Language Technology Workshop},
  pages     = {785--792},
  year      = {2021},
}


@article{fst,
author = {Mohri, Mehryar and Pereira, Fernando and Riley, Michael},
title = {Weighted Finite-State Transducers in Speech Recognition},
year = {2002},
issue_date = {January 2002},
publisher = {Academic Press Ltd.},
volume = {16},
number = {1},
issn = {0885-2308},
journal = {Computer Speech and Language},
month = jan,
pages = {69–88},
numpages = {20}
}

@inproceedings{tedlium,
  author    = {Fran{\c{c}}ois Hernandez and
               Vincent Nguyen and
               Sahar Ghannay and
               Natalia A. Tomashenko and
               Yannick Est{\`{e}}ve},
  editor    = {Alexey Karpov and
               Oliver Jokisch and
               Rodmonga Potapova},
  title     = {{TED-LIUM} 3: Twice as Much Data and Corpus Repartition for Experiments
               on Speaker Adaptation},
  booktitle = {Proc. of SPECOM},
  year      = {2018},
}

@Book{ravanelli_thesis,
  author= "M. Ravanelli",
  title= "Deep learning for Distant Speech Recognition",
  publisher = "PhD Thesis, Unitn",
  year = 2017
}

@inproceedings{adversarial,
title	= {Explaining and Harnessing Adversarial Examples},
author	= {I. Goodfellow and J. Shlens and C. Szegedy},
year	= {2015},
booktitle	= {Proc.of ICLR}
}


@INPROCEEDINGS{dnn_emotion,
author={G. Trigeorgis and F. Ringeval and R. Brueckner and E. Marchi and M. A. Nicolaou and B. Schuller and S. Zafeiriou},
booktitle={Proc. of ICASSP},
title={Adieu features? End-to-end speech emotion recognition using a deep convolutional recurrent network},
year={2016},
volume={},
number={},
pages={5200-5204}}


@Book{BenestySondhi08,
  editor= "J. 
  and Sondhi, M. M. and Y. Huang",
  title= "Springer Handbook of Speech Processing",
  publisher = "Springer",
  year = 2008
}

@Book{dsrbook,
  author = "W{\"o}lfel, M. and McDonough, J.",
  title = "Distant Speech Recognition",
  publisher = "Wiley",
  year = 2009
  
}



@Book{RabinerJuang93,
  author= "Rabiner, L. R. and Huang, B.-H.",
  title= "Fundamentals of Speech Recognition",
  publisher = "Prentice-Hall",
  year = 1993
}

@inproceedings{Falavigna2012,
    Author = {Daniele Falavigna and Roberto Gretter},
    Title = {Focusing Language Models For Automatic Speech Recognition},
    Booktitle = {Proc. International Workshop on Spoken Language Translation (IWSLT)},
    Pages = {171--178},
    Year = {2012}
}

@article{Bertoldi2002,
    Author = {N. Bertoldi and F. Brugnara and M. Cettolo and M. Federico and D. Giuliani},
    Title = {Cross-Task Portability of a Broadcast News Speech Recognition System},
    Journal = {Speech Communication},
    Pages = {335-347},
    Volume = {38},
    Number = {3-4},
    Year = {2002}
}


@article{stolckeCN,
    Author = {L. Mangu and E. Brill and A. Stolcke},
    Title = {Finding consensus in speech recognition: word error minimization and other applications of confusion networks Recognition System},
    Journal = {{Computer Speech \& Language}},
    Pages = {373-400},
    Volume = {14},
    Number = {4},
    Year = {2000}
}




@inproceedings{Bertoldi2001,
    Author = {N. Bertoldi and F. Brugnara and M. Cettolo and M. Federico and D. Giuliani},
    Title = {From {B}roadcast News to Spontaneous Dialogue Transcription: {P}ortability Issues},
    Booktitle = {Proc. International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
    Year = {2001}
}

@inproceedings{Girardi2011,
  author    = {Christian Girardi and
               Roberto Gretter and
               Daniele Falavigna and
               Fabio Brugnara and
               Diego Giuliani and
               Marcello Federico},
  title     = {{NeMo}: A Platform for Multilingual News Monitoring},
  booktitle = {Proc. Interspeech},
  year      = {2011},
  pages     = {2261--2264}
}

@inproceedings{Falavigna2010,
 author = {Falavigna, Daniele and Gerosa, Matteo and Giuliani, Diego and Gretter, Roberto},
 title = {An automatic transcription system of hearings in {I}talian courtrooms},
 booktitle = {Proc. ACM Workshop on Multimedia in Forensics, Security and Intelligence (MiFor)},
 year = {2010},
 pages = {99--104},
} 

@inproceedings{Falavigna2011,
  author    = {Daniele Falavigna and Roberto Gretter},
  title     = {Cheap Bootstrap of Multi-Lingual Hidden {M}arkov Models},
  booktitle = {Proc. Interspeech},
  year      = {2011},
  pages     = {2325-2328}
}

@article{Gerosa2009,
author = "Matteo Gerosa and Diego Giuliani and Fabio Brugnara",
title = "Towards age-independent acoustic modeling",
journal = "Speech Communication",
volume = "51",
number = "6",
pages = "499 - 509",
year = "2009",
}

@INPROCEEDINGS{Federico2008,
AUTHOR = "Marcello Federico and Nicola Bertoldi and Mauro Cettolo",
TITLE = "{IRSTLM}: an open source toolkit for handling large scale language models",
BOOKTITLE = "Proc. Interspeech",
PAGES = {1618--1621},
YEAR = {2008} 
}

@INPROCEEDINGS{rav_is16,
AUTHOR = "M. Ravanelli and P. Svaizer and M. Omologo",
TITLE = "Realistic multi-microphone data simulation for distant speech recognition",
BOOKTITLE = "Proc. of Interspeech",
YEAR = {2016} 
}



@INPROCEEDINGS{dicit2009,
author={Marquardt, L. and Svaizer, P. and Mabande, E. and Brutti, A. and Zieger, C. and Omologo, M. and Kellermann, W.},
title={A natural acoustic front-end for Interactive {TV} in the {EU}-{P}roject {DICIT}},
booktitle={Proc. Pacific Rim Conference on Communications, Computers and Signal Processing}, 
year={2009},
pages={894--899}
}

@article{Brutti2010,
  author    = {Alessio Brutti and
               Luca Cristoforetti and
               Walter Kellermann and
               Lutz Marquardt and
               Maurizio Omologo},
  title     = {{WOZ} acoustic data collection for interactive {TV}},
  journal   = {Language Resources and Evaluation},
  volume    = {44},
  number    = {3},
  year      = {2010},
  pages     = {205--219}

}

@INPROCEEDINGS{bocchieri13,
author	= {Bocchieri, Enrico and Dimitriadis, Dimitrios},
title	= {INVESTIGATING DEEP NEURAL NETWORK BASED TRANSFORMS OF ROBUST AUDIO FEATURES FOR {LVCSR}},
booktitle	= icassp,
year	= {2013}
}

@INPROCEEDINGS{fiscus97,
author = {J. G. Fiscus},
title = {A post-processing system to yield reduced word error rates: Recognizer output voting error reduction ({ROVER})},
booktitle= {Proc. Automatic Speech Recognition and Understanding Workshop}, 
pages = {347--352},
year = {1997}
}

@INPROCEEDINGS{stolcke97,
  title={Explicit word error minimization in n-best list rescoring.},
  author={Stolcke, Andreas and Konig, Yochai and Weintraub, Mitchel},
  booktitle=eurospeech,
  volume={97},
  pages={163--166},
  year={1997}
}

@INPROCEEDINGS{xu10,
  title={An improved consensus-like method for minimum bayes risk decoding and lattice combination},
  author={Xu, Haihua and Povey, Daniel and Mangu, Lidia and Zhu, Jie},
  booktitle=icassp,
  pages={4938--4941},
  year={2010}
}

@INPROCEEDINGS{irodoma13b,
  title={Advances In Large Vocabulary Continuous Speech Recognition In {G}reek: {M}odeling And Nonlinear Features},
  author={Isidoros Rodomagoulakis and Gerasimos Potamianos and Petros Maragos},
  booktitle=eusipco,
  year={2013}
}

@INPROCEEDINGS{nkatsam14,
title={ROBUST FAR-FIELD SPOKEN COMMAND RECOGNITION FOR HOME AUTOMATION COMBINING ADAPTATION AND MULTICHANNEL PROCESSING},
author={Athanasios Katsamanis and Isidoros Rodomagoulakis and Gerasimos Potamianos and Petros Maragos and Antigoni Tsiami},
booktitle={(TO APPEAR in {ICASSP} 2014)}
}

@inproceedings{neti00,
  title={Audio-visual speech recognition},
  author={Neti, Chalapathy and Potamianos, Gerasimos and Luettin, Juergen and Matthews, Iain and Glotin, Herve and Vergyri, Dimitra and Sison, June and Mashari, Azad and Zhou, Jie},
  booktitle={Final Workshop 2000 Report},
  volume={764},
  year={2000}
}


% This file was created with JabRef 2.9.2.
% Encoding: MacRoman

@ARTICLE{Barker13,
  author = {Barker, J. and Vincent, E. and Ma, N. and Christensen, H. and Green,
	P.},
  title = {The {PASCAL} {CHiME} speech separation and recognition challenge},
  journal = {Computer Speech \& Language},
  year = {2013},
  volume = {27},
  pages = {621-633},
  number = {3}
}

@BOOK{Benesty08,
  title = {Microphone Array Signal Processing},
  publisher = {Springer},
  year = {2008},
  author = {Benesty, J. and Chen, J. and Huang, Y.},
  volume = {1}
}

@ARTICLE{Chan08,
  author = {Chan, M. and Estève, D. and Escriba, C. and Campo, E.},
  title = {A review of smart homes - {P}resent state and future challenges},
  journal = {Computer Methods and Programs in Biomedicine},
  year = {2008},
  volume = {91},
  pages = {55-81},
  number = {1}
}

@INPROCEEDINGS{Chen13,
  author = {Chen, I.-F. and Lee, C.-H},
  title = {A Resource-Dependent Approach to Word Modeling for Keyword Spotting},
  booktitle = interspeech,
  year = {2013}
}

@INCOLLECTION{CMP06,
  author = {Chu, S.M. and Marcheret, E. and Potamianos, G.},
  title = {Automatic Speech Recognition and Speech Activity Detection in the
	{CHIL} Smart Room},
  booktitle = {Machine Learning for Multimodal Interaction},
  publisher = {Springer Berlin Heidelberg},
  year = {2006},
  editor = {Renals, S. and Bengio, S.},
  owner = {nassos},
  timestamp = {2013.11.04}
}

@INPROCEEDINGS{logotypographia,
  author = {Digalakis, V. and Oikonomidis, D. and Pratsolis, D. and Tsourakis,
	N. and Vosnidis, C. and Chatzichrisafis, N. and Diakoloukas, V.},
  title = {Large vocabulary continuous speech recognition in {G}reek: {C}orpus
	and an automatic dictation system},
  booktitle = interspeech,
  year = {2003}
}

@ARTICLE{Keshet09,
  author = {Keshet, J. and Grangier, D. and Bengio, S.},
  title = {Discriminative keyword spotting},
  journal = {Speech Communication},
  year = {2009},
  volume = {51},
  pages = {317-329},
  number = {4}
}

@ARTICLE{Kumatani12,
  author = {Kumatani, K. and McDonough, J. and Raj, B.},
  title = {Microphone Array Processing for Distant Speech Recognition: {F}rom
	Close-Talking Microphones to Far-Field Sensors},
  journal = IEEE_M_SP,
  year = {2012},
  volume = {29},
  pages = {127-140},
  number = {6}
}



@ARTICLE{Lefkimmiatis07,
  author = {Lefkimmiatis, S. and Maragos, P.},
  title = {A generalized estimation approach for linear and nonlinear microphone
	array post-filters},
  journal = {Speech Communication},
  year = {2007},
  volume = {49},
  pages = {657-666},
  number = {7-8}
}

@INPROCEEDINGS{Mandal13,
  author = {Mandal, A. and Hout, J. and Tam, Y.-C. and Mitra, V. and Lei, Y.
	and Zheng, J. and Vergyri, D. and Ferrer, L. and Graciarena, M. and
	Kathol, A. and Horacio, F.},
  title = {Strategies for High Accuracy Keyword Detection in Noisy Channels},
  booktitle = interspeech,
  year = {2013}
}

@ARTICLE{Mat+02,
  author = {Matassoni, M. and Omologo, M. and Giuliani, D. and Svaizer, P.},
  title = {Hidden {M}arkov model training with contaminated speech material
	for distant-talking speech recognition },
  journal = J_CSL,
  year = {2002},
  volume = {16},
  pages = {205-223},
  number = {2},
  doi = {http://dx.doi.org/10.1006/csla.2002.0191},
  issn = {0885-2308},
  url = {http://www.sciencedirect.com/science/article/pii/S0885230802901919}
}

@INPROCEEDINGS{Mporas09,
  author = {Mporas, I. and Ganchev, T. and Kostoulas, T. and Kermanidis, K. and
	Fakotakis, N.},
  title = {Automatic Speech Recognition System for Home Appliances Control},
  booktitle = {13th Panhellenic Conference on Informatics},
  year = {2009},
  pages = {114-117}
}

@ARTICLE{Omologo97,
  author = {Omologo, M. and Svaizer, P.},
  title = {Use of the crosspower-spectrum phase in acoustic event location},
  journal = IEEE_J_SAP,
  year = {1997},
  volume = {5},
  pages = {288-292}
}

@INPROCEEDINGS{Ost+91,
  author = {Ostendorf, M. and Kannan, A. and Austin, S. and Kimball, O. and Schwartz,
	R. M. and Rohlicek, J. R.},
  title = {Integration of Diverse Recognition Methodologies Through Reevaluation
	of {N}-{B}est Sentence Hypotheses.},
  booktitle = C_HLT,
  year = {1991},
  pages = {83-87},
  url = {http://acl.ldc.upenn.edu/H/H91/H91-1013.pdf},
  urldate = {2013-09-06}
}

@INPROCEEDINGS{Pri+13,
  author = {Principi, Emanuele and Squartini, Stefano and Piazza, Francesco and
	Fuselli, Danilo and Bonifazi, Maurizio},
  title = {A Distributed System for Recognizing Home Automation Commands and
	Distress Calls in the {I}talian Language},
  booktitle = interspeech,
  year = {2013},
  owner = {nassos},
  timestamp = {2013.10.10}
}

@INPROCEEDINGS{Rav+12,
  author = {Ravanelli, M. and Sosi, A. and Svaizer, P. and Omologo, M.},
  title = {Impulse response estimation for robust speech recognition in a reverberant
	environment},
  booktitle = EURASIP_C_EUSIPCO,
  year = {2012},
  pages = {1668-1672}
}

@INPROCEEDINGS{RSGMP13,
  author = {Rodomagoulakis, I. and Giannoulis, P. and Skordilis, Z.-I. and Maragos,
	P. and Potamianos, G.},
  title = {Experiments on Far-field Multichannel Speech Processing in Smart
	Homes},
  booktitle = {Proc. 18th Int. Conf. Digital Signal Processing},
  year = {2013},
  owner = {nassos},
  timestamp = {2013.11.04}
}

@INPROCEEDINGS{RPM13,
  author = {Rodomagoulakis, I. and Potamianos, G. and Maragos, P.},
  title = {Advances In Large Vocabulary Continuous Speech Recognition In {G}reek:
	{M}odeling And Nonlinear Features},
  booktitle = eusipco,
  year = {2013}
}

@INCOLLECTION{SeKe08,
  author = {Sehr, A. and Kellermann, W.},
  title = {Towards Robust Distant-Talking Automatic Speech Recognition in Reverberant
	Environments},
  booktitle = {Speech and Audio Processing in Adverse Environments},
  publisher = {Springer Berlin Heidelberg},
  year = {2008},
  editor = {H\"{a}nsler, E. and Schmidt, G.},
  pages = {679-728},
  owner = {nassos},
  timestamp = {2013.11.04}
}

@ARTICLE{Smith87,
  author = {Smith, J.O. and Abel, J.S.},
  title = {Closed-form least-squares source location estimation from range-difference
	measurements},
  journal = {Acoustics, Speech and Signal Processing, IEEE Transactions on},
  year = {1987},
  volume = {35},
  pages = {1661-1669},
  number = {12}
}

@INPROCEEDINGS{Vac+13,
  author = {Vacher, M. and Lecouteux, B. and Istrate, D. and Joubert, T. and
	Portet, F. and Sehili, M. and Chahuara, P.},
  title = {Evaluation of a Real-Time Voice Order Recognition System from Multiple
	Audio Channels in a Home},
  booktitle = interspeech,
  year = {2013}
}


@INPROCEEDINGS{kellerman1,
  author = {A. Sehr and E.A.P. Habets and R. Maas and W. Kellermann},
  title = {Towards a better understanding of the effect of reverberation on speech recognition performance},
  booktitle =  {Proc. of the International Workshop on Acoustic Echo and Noise Control (IWAENC)},
  year = {2010}
}

@INPROCEEDINGS{revch,
author={Kinoshita at all, K.},
booktitle={Proc. of WASPAA 2013},
title={{The reverb challenge: A Common Evaluation Framework for Dereverberation and Recognition of Reverberant Speech}},
pages={1-4}
}

@INPROCEEDINGS{revch_full,
author={Kinoshita, K. and Delcroix, M. and Yoshioka, T. and Nakatani, T. and Habets, E. and Haeb-Umbach, R. and Leutnant, V. and Sehr, A. and Kellermann, W. and Maas, R. and Gannot, S. and Raj, B.},
booktitle={Proc. of WASPAA 2013},
title={{The reverb challenge: A Common Evaluation Framework for Dereverberation and Recognition of Reverberant Speech}},
pages={1-4}
}


@INPROCEEDINGS{VKF05,
  author = {Vovos, A. and Kladis, B. and Fakotakis, N.},
  title = {Speech Operated Smart-Home Control System for Users with Special
	Needs},
  booktitle = interspeech,
  year = {2005}
}

@INPROCEEDINGS{WFIM06,
  author = {W\"{o}lfel, M. and F\"{u}gen, C. and Ikbal, S. and McDonough, J.
	W.},
  title = {Multi-Source Far-Distance Microphone Selection and Combination
	
	for Automatic Transcription of Lectures},
  booktitle = interspeech,
  year = {2006},
  pages = {361-364},
  owner = {nassos},
  timestamp = {2013.11.04}
}

@ARTICLE{Wil+90,
  author = {Wilpon, J. and Rabiner, L. R. and Lee, C.-H. and Goldman, E. R.},
  title = {Automatic recognition of keywords in unconstrained speech using hidden
	{M}arkov models},
  journal = IEEE_J_ASSP,
  year = {1990},
  volume = {38},
  pages = {1870-1878},
  number = {11}
}

@INPROCEEDINGS{WoNa13,
  author = {Wolf, M. and Nadeu, C.},
  title = {Channel Selection Using {N}-{B}est Hypothesis for Multi-Microphone
	{ASR}},
  booktitle = interspeech,
  year = {2013}
}

@INPROCEEDINGS{WoNa10,
  author = {Wolf, M. and Nadeu, C.},
  title = {On the potential of channel selection for
	
	recognition of reverberated speech with multiple microphones},
  booktitle = interspeech,
  year = {2010},
  pages = {80 - 83},
  owner = {nassos},
  timestamp = {2013.11.04}
}



@INPROCEEDINGS{Woo01,
  author = {Woodland, P. C.},
  title = {Speaker adaptation for continuous density {HMM}s: {A} review},
  booktitle = {ISCA Tutorial and Research Workshop on Adaptation Methods for Speech
	Recognition},
  year = {2001}
}

@BOOK{Young02,
  title = {The {HTK} Book},
  publisher = {Entropic Cambridge Research Laboratory, Cambridge, United Kingdom},
  year = {2002},
  author = {Young, S. and Evermann, G. and Hain, T. and Kershaw, D. and Moore,
	G. and Odell, J. and Ollason, D. and Povey, D. and Valtchev, V. and
	Woodland, P.}
}

@MISC{dirhaproj,
  title = {{DIRHA}: {D}istant-speech {I}nteraction for {R}obust {H}ome {A}pplications},
  note = {[Online] Available: \url{http://dirha.fbk.eu/}}
}




@Article{Matassoni-02,
  author = 	 "M. Matassoni and M. Omologo and D. Giuliani and P. Svaizer",
  title = 	 "{HMM Training with Contaminated Speech Material for Distant-Talking Speech Recognition}",
  journal =  "Computer Speech and Language",
  year =         "2002",
  publisher = "Elsevier",
}

@Article{Schroeder-65,
  author = 	 "M. R. Schroeder",
  title = 	 "A new method of measuring reverberation time",
  journal =  "Journal of the Acoustical Society of America",
  pages =    "409--412",
  volume =   "37",
  year =     "1965",
}

 @Inproceedings{Schuppler-14,
  author = 	 "B. Schuppler and M. Hagm{\"u}ller and J. A. Morales Cordovilla and H. Pessentheiner",
  title = 	 "{GRASS: the Graz corpus of Read And Spontaneous Speech}",
  booktitle = "Proceedings of LREC 2014",
  year = 	 "2014",
}

 @Inproceedings{Farina-00,
  author = 	 "A. Farina",
  title = 	 "{Simultaneous Measurement of Impulse Response and Distortion with a Swept-Sine Technique}",
  booktitle = "Proceedings of 108th AES Convention",
  year = 	 "2000",
}

 @Inproceedings{Ravanelli-12,
  author = 	 "M. Ravanelli and A. Sosi and P. Svaizer and M. Omologo",
  title = 	 "Impulse response estimation for robust speech recognition in a reverberant environment",
  booktitle = "Proc. of EUSIPCO 2012"
}

 @Inproceedings{asilomar-10,
  author = 	 "M. Omologo",
  title = 	 "{A prototype of distant-talking interface for control of interactive TV}",
  booktitle = "Proceedings of Asilomar Conference on Signals, Systems and Computers",
  year = 	 "2010",
}

 @Inproceedings{interspeech-08,
  author = 	 "J. Huang and M. Epstein and M. Matassoni",
  title = 	 "{Effective Acoustic Adaptation for A Distant-talking Interactive TV System}",
  booktitle = "Proceedings of Interspeech 2008",
  year = 	 "2008",
}


@Techreport{Ravanelli-14,
  author =       "M. Ravanelli and M. Omologo",
  title =        "{Deliverable D2.1\_D2.3\_D2.4: DIRHA-simcorpora I and II}",
  institution =  "DIRHA Consortium",
  year =         "2014",
  timestamp =    "2014.02.24"
}

@Incollection{chil-06,
  author = 		"M. Omologo and P. Svaizer and A. Brutti and L. Cristoforetti",
  title = 		"Speaker localization in {CHIL} lectures: Evaluation criteria and results",
  booktitle = 	"Machine Learning for Multimodal Interaction",
  pages = 		"476--487",
  year = 		"2006",
  editor =      "S. Renals and S. Bengio",
  publisher =   "Springer Verlag"
}

@inproceedings{gru2,
    author = {Chung, J. and G{\"{u}}l{\c c}ehre, {\c C}. and Cho, K. and Bengio, Y.},
     title = {Empirical Evaluation of Gated Recurrent Neural Networks on Sequence Modeling},
 booktitle = {Proc. of NIPS},
      year = {2014},
}

@inproceedings{SincNet,
  author    = {M. Ravanelli and
               Y. Bengio},
  title     = {{Speaker Recognition from raw waveform with SincNet}},
  booktitle = {Proc. of SLT},
  year = {2018},
}

@Inproceedings{ravanelli_is17,
  author= "M. Ravanelli and P. Brakel and M. Omologo and Y. Bengio",
  title= "Improving speech recognition by revising gated recurrent units",
  booktitle = "Proc. of Interspeech",
  year = "2017"  
}


@Inproceedings{ravanelli_twin,
  author= "M. Ravanelli and  D. Serdyuk and Y. Bengio",
  title= "Twin Regularization for online speech recognition",
  booktitle = "Proc. of Interspeech",
  year = "2018"  
}

@ARTICLE{li_gru,
author={M. Ravanelli and P. Brakel and M. Omologo and Y. Bengio},
journal={IEEE Transactions on Emerging Topics in Computational Intelligence},
title={Light Gated Recurrent Units for Speech Recognition},
year={2018},
volume={2},
number={2},
pages={92-102},
month={April},}

@article{triplet_loss_spk_rec,
  author    = {C. Li and
               X. Ma and
               B. Jiang and
               X. Li and
               X. Zhang and
               X. Liu and
               Y. Cao and
               A. Kannan and
               Z. Zhu},
  title     = {Deep Speaker: an End-to-End Neural Speaker Embedding System},
  journal   = {CoRR},
  volume    = {abs/1705.02304},
  year      = {2017},
}

@article{triplet_loss,
  added-at = {2018-08-13T00:00:00.000+0200},
  author = {Schroff, F. and Kalenichenko, D. and Philbin, J.},
  journal = {CoRR},
  title = {FaceNet: A Unified Embedding for Face Recognition and Clustering.},
  volume = {abs/1503.03832},
  year = 2015
}

@article{unsup_spk_id,
  author    = {A. Jati and
               P. G. Georgiou},
  title     = {Neural Predictive Coding using Convolutional Neural Networks towards Unsupervised Learning of Speaker Characteristics},
  journal   = {CoRR},
  volume    = {abs/1802.07860},
  year      = {2018},
}

@Inproceedings{hscma,
  author= "A. Brutti and M. Ravanelli and P. Svaizer and M. Omologo",
  title= "A SPEECH EVENT DETECTION/LOCALIZATION TASK FOR MULTIROOM ENVIRONMENTS",
  booktitle = "Proceedings of HSCMA 2014",
  year = "2014"
}

@INPROCEEDINGS{dirha_asru, 
author={M. Ravanelli and L. Cristoforetti and R. Gretter and M. Pellin and A. Sosi and M. Omologo},
booktitle={Proc. of ASRU 2015}, 
title={{The DIRHA-ENGLISH corpus and related tasks for distant-speech recognition in domestic environments}},  
pages={275-282}
}

@INPROCEEDINGS{dirha_icassp, 
author={E. Zwyssig and M. Ravanelli and P. Svaizer and M. Omologo}, 
booktitle={Proc. of ICASSP 2015}, 
title={A multi-channel corpus for distant-speech interaction in presence of known interferences}, 
pages={4480-4484}, 
}



@incollection{kellerman,
year={2008},
booktitle={Speech and Audio Processing in Adverse Environments},
title={Towards Robust Distant-Talking Automatic Speech Recognition in Reverberant Environments},
publisher={Springer Berlin Heidelberg},
author={Sehr, Armin and Kellermann, Walter},
pages={679-728},
language={English}
}



 @Inproceedings{Martin-90,
  author = 	 "Martin, L.E.",
  title = 	 "Knowledge Extraction",
  booktitle = "Proceedings of the Twelfth Annual Conference of the Cognitive Science Society",
  year = 	 "1990",
  month = 	 "",
  date =     "",
  pages = 	 "252--262",
  address =  "Hillsdale, NJ",
  editor = 	 "",
  publisher = "Lawrence Erlbaum Associates",
  isbn = "",
}


@misc{librimix,
      title={LibriMix: An Open-Source Dataset for Generalizable Speech Separation}, 
      author={Joris Cosentino and Manuel Pariente and Samuele Cornell and Antoine Deleforge and Emmanuel Vincent},
      year={2020},
      eprint={2005.11262},
      archivePrefix={arXiv},
      primaryClass={eess.AS}
}


@inproceedings{whamr,
  author    = {Matthew Maciejewski and
               Gordon Wichern and
               Emmett McQuinn and
               Jonathan Le Roux},
  title     = {WHAMR!: Noisy and Reverberant Single-Channel Speech Separation},
  booktitle = {Proc. of ICASSP},
  pages     = {696--700},
  year      = {2020},
}
@inproceedings{wham,
  author={Gordon Wichern and Joe Antognini and Michael Flynn and Licheng Richard Zhu and Emmett McQuinn and Dwight Crow and Ethan Manilow and Jonathan Le Roux},
  title={{WHAM!: extending speech separation to noisy environments}},
  year=2019,
  booktitle={Proc. Interspeech},
  pages={1368--1372},
  doi={10.21437/Interspeech.2019-2821},
  url={http://dx.doi.org/10.21437/Interspeech.2019-2821}
}

@InProceedings{dns_challenge,
author = {Reddy, Chandan K. A. and Gopal, Vishak and Cutler, Ross and Beyrami, Ebrahim and Cheng, Roger and Dubey, Harishchandra and Matusevych, Sergiy and Aichner, Robert and Aazami, Ashkan and Braun, Sebastian and Rana, Puneet and Srinivasan, Sriram and Gehrke, Johannes},
title = {The INTERSPEECH 2020 Deep Noise Suppression Challenge: Datasets, Subjective Testing Framework, and Challenge Results},
booktitle = {Proc. of Interspeech},
year = {2020},
}

@inproceedings{aishell_2017,
  title={AIShell-1: An Open-Source Mandarin Speech Corpus and A Speech Recognition Baseline},
  author={Hui Bu, Jiayu Du, Xingyu Na, Bengu Wu, Hao Zheng},
  booktitle={Oriental COCOSDA 2017},
  pages={Submitted},
  year={2017}
}

@INPROCEEDINGS{pesq,
  author={Rix, A.W. and Beerends, J.G. and Hollier, M.P. and Hekstra, A.P.},
  booktitle={2001 IEEE International Conference on Acoustics, Speech, and Signal Processing. Proceedings (Cat. No.01CH37221)}, 
  title={Perceptual evaluation of speech quality (PESQ)-a new method for speech quality assessment of telephone networks and codecs}, 
  year={2001},
  volume={2},
  number={},
  pages={749-752 vol.2},
  doi={10.1109/ICASSP.2001.941023}}
  
@Inproceedings{apasci,
  author= "B. Angelini and F. Brugnara and D. Falavigna and D. Giuliani and R. Gretter and M. Omologo",
  title= "{S}peaker independent continuous speech recognition using an acoustic-phonetic {I}talian corpus",
  booktitle = "Proceedings of ICSLP 1994",
  year = "1994",
}

@inproceedings{contextnet,
title	= {ContextNet: Improving Convolutional Neural Networks for Automatic Speech Recognition with Global Context},
author	= {Wei Han and Zhengdong Zhang and Yu Zhang and Jiahui Yu and Chung-Cheng Chiu and James Qin and Anmol Gulati and Ruoming Pang and Yonghui Wu},
year	= {2020},
URL	= {https://arxiv.org/abs/2005.03191}
}



@misc{timit,
  author = "Garofolo, J. S. and Lamel, L. F. and Fisher, W. M. and Fiscus, J. G. and Pallett, D. S. and Dahlgren, N. L.",
  publisher = "NIST",
  title = "{DARPA TIMIT Acoustic Phonetic Continuous Speech Corpus CDROM}",
  year = "1993"
}

@inproceedings{demand,
  TITLE = {{The Diverse Environments Multi-channel Acoustic Noise Database (DEMAND): A database of multichannel environmental noise recordings}},
  AUTHOR = {Thiemann, Joachim and Ito, Nobutaka and Vincent, Emmanuel},
  BOOKTITLE = {{21st International Congress on Acoustics}},
  YEAR = {2013},
}

@INPROCEEDINGS{voicebank,
  author={Veaux, Christophe and Yamagishi, Junichi and King, Simon},
  booktitle={2013 International Conference Oriental COCOSDA held jointly with 2013 Conference on Asian Spoken Language Research and Evaluation (O-COCOSDA/CASLRE)}, 
  title={The voice bank corpus: Design, collection and data analysis of a large regional accent speech database}, 
  year={2013},}
  
@article{librilight,
  author    = {Jacob Kahn and
               Morgane Rivi{\`{e}}re and
               Weiyi Zheng and
               Evgeny Kharitonov and
               Qiantong Xu and
               Pierre{-}Emmanuel Mazar{\'{e}} and
               Julien Karadayi and
               Vitaliy Liptchinsky and
               Ronan Collobert and
               Christian Fuegen and
               Tatiana Likhomanenko and
               Gabriel Synnaeve and
               Armand Joulin and
               Abdelrahman Mohamed and
               Emmanuel Dupoux},
  title     = {Libri-Light: {A} Benchmark for {ASR} with Limited or No Supervision},
  journal   = {CoRR},
  volume    = {abs/1912.07875},
  year      = {2019},
}

@Book{Chercheur-94,
  title =        "Case-Based Reasoning",
  author =       "J.L. Chercheur",
  publisher =    "Morgan Kaufman Publishers",
  year =         "1994",
  edition =      "2nd",
  address =      "San Mateo, CA",
}


@Book{speechde,
  title =        "Speech Dereverberation",
  author =       "P. A. Naylor and N. D. Gaubitch",
  publisher =    "Springer",
  year =         "2010",

}



@Article{CastorPollux-92,
  author =       "A. Castor and L. E. Pollux",
  title =        "The use of user modelling to guide inference and learning",
  journal =      "Applied Intelligence",
  volume =       "2(1)",
  pages =        "37--53",
  year =         "1992",
}

@Phdthesis{Zavatta-92,
  author =       "A. Zavatta",
  year =         "1992",
  title =        "Un G�n�rateur d'Insultes s'int�grant dans un Syst�me de Dialogue Humain-Machine.",
  school =       "Universit� Paris-sud, Centre d'Orsay",
  type =         "Th�se de Doctorat en Informatique",
}

@Inbook{Grandchercheur-83,
  author =       "L. B. Grandchercheur",
  title =        "Vers une mod�lisation cognitive de l'�tre et du n�ant",
  booktitle =    "Fondement des Sciences Cognitives",
  editor =       "S. G. Paris and G. M. Olson anf H. W. Stevenson",
  publisher =    "Lawrence Erlbaum Associates",
  year =         "1983",
  pages =        "6--38",
  address =      "Hillsdale, N.J."
}

%fictitious reference
@Book{Superman-Batman-Catwoman-Spiderman-00,
  author =       "S. Superman and B. Batman and C. Catwoman and S. Spiderman",
  title =        "Superheroes experiences with books",
  journal =      "Journal journal journal",
  year =         "2000",
  publisher =    "The Phantom Editors Associates",
  edition =      "20th",
  address =      "Gotham City",
}



%% @COMMENT{Other examples taken from the document describing BS 5605}
@Book{chicago-82,
  title =        "The {C}hicago Manual of Style",
  author =       "`Chicago'",
  year =         "1982",
  publisher =    "University of Chicago Press",
  edition =      "13th",
}

@Article{howells-66-pop,
  author =       "W. W. Howells",
  title =        "Population Distances: Biological, Linguistic,
                 Geographical and Environmental",
  journal =      "Current Anthropology",
  volume =       "7",
  pages =        "531--540",
  year =         "1966",
}

@Manual{anon-67,
  author =       "Anon.",
  title =        "Title title title title title title title title title
                 title",
  organization = "Organization organization organization",
  year =         "1967",
}

@INPROCEEDINGS{librispeech,
author={V. Panayotov and G. Chen and D. Povey and S. Khudanpur},
booktitle={Proc. of ICASSP},
title={{Librispeech: An ASR corpus based on public domain audio books}},
year={2015},
volume={},
number={},
pages={5206-5210}
}


@INPROCEEDINGS{transformers_asr,
  author={Karita, Shigeki and Chen, Nanxin and Hayashi, Tomoki and Hori, Takaaki and Inaguma, Hirofumi and Jiang, Ziyan and Someki, Masao and Soplin, Nelson Enrique Yalta and Yamamoto, Ryuichi and Wang, Xiaofei and Watanabe, Shinji and Yoshimura, Takenori and Zhang, Wangyou},
  booktitle={Proc. of ASRU}, 
  title={A Comparative Study on Transformer vs RNN in Speech Applications}, 
  year={2019}
  }
  
@inproceedings{szymanski-etal-2020-wer,
    title = "{WER} we are and {WER} we think we are",
    author = "Szyma{\'n}ski, Piotr  and
      {\.Z}elasko, Piotr  and
      Morzy, Mikolaj  and
      Szymczak, Adrian  and
      {\.Z}y{\l}a-Hoppe, Marzena  and
      Banaszczak, Joanna  and
      Augustyniak, Lukasz  and
      Mizgajski, Jan  and
      Carmiel, Yishay",
    booktitle = "Proc. of EMNLP",
    year = "2020",
}

@inproceedings{commonvoice:2020,
  author = {Ardila, R. and Branson, M. and Davis, K. and Henretty, M. and Kohler, M. and Meyer, J. and Morais, R. and Saunders, L. and Tyers, F. M. and Weber, G.},
  title = {Common Voice: A Massively-Multilingual Speech Corpus},
  booktitle = {Proceedings of the 12th Conference on Language Resources and Evaluation (LREC 2020)},
  pages = {4211--4215},
  year = 2020
}
  
@INPROCEEDINGS{leaky_relu,
    author = {A. L. Maas and A. Y. Hannun and A. Y. Ng},
    title = {Rectifier nonlinearities improve neural network acoustic models},
    booktitle = {Proc. of ICML},
    year = {2013}
}

@Incollection{hanson-67,
  author =       "C. W. Hanson",
  title =        "Subject inquiries and literature searching",
  booktitle =    "Handbook of special librarianship and information
                 work",
  editor =       "W. Ashworth",
  year =         "1967",
  edition =      "3rd",
  pages =        "414--452",
}

@Inbook{wright-63,
  author =       "R. C. Wright",
  title =        "Report Literature",
  booktitle =    "Special Materials in the Library",
  editor =       "J. Burkett and T. S. Morgan",
  year =         "1963",
  pages =        "46--59",
}

%% @COMMENT{Some examples taken from document describing BS 1629}

@Book{hoel-71-whole,
  author =       "Paul Gerhard Hoel",
  title =        "Elementary Statistics",
  publisher =    "Wiley",
  year =         "1971",
  series =       "Wiley series in probability and mathematical
                 statistics",
  address =      "New York, Chichester",
  edition =      "3rd",
  note =         "ISBN 0~471~40300",
}


@book{WaibelStiefelhagen2009,
  author = "A. Waibel and R. Stiefelhagen",
  isbn = "978-1-84882-053-1",
  publisher = "Springer",
  title = "Computers in the Human Interaction Loop",
  year = "2009",
}

@Inbook{hoel-71-portion,
  author =       "Paul Gerhard Hoel",
  title =        "Elementary Statistics",
  publisher =    "Wiley",
  year =         "1971",
  series =       "Wiley series in probability and mathematical
                 statistics",
  address =      "New York, Chichester",
  edition =      "3rd",
  note =         "ISBN 0~471~40300",
  pages =        "19--33",
}

@Book{singer-whole,
  year =         "1954--58",
  editor =       "Charles Joseph Singer and E. J. Holmyard and A. R.
                 Hall",
  title =        "A history of technology",
  address =      "London",
  publisher =    "Oxford University Press",
  note =         "5 vol.",
}

@Incollection{singer-portion-chapter,
  title =        "The late nineteenth century",
  year =         "1954--58",
  editor =       "Charles Joseph Singer and E. J. Holmyard and A. R.
                 Hall",
  booktitle =    "A history of technology",
  address =      "London",
  publisher =    "Oxford University Press",
  type =         "Vol.",
  chapter =      "5",
}

@Inproceedings{chomsky-73,
  author =       "N. Chomsky",
  year =         "1973",
  title =        "Conditions on Transformations",
  booktitle =    "A festschrift for {Morris Halle}",
  editor =       "S. R. Anderson and P. Kiparsky",
  publisher =    "Holt, Rinehart \& Winston",
  address =      "New York",
}


@INPROCEEDINGS{stahl,
author={Stahl, V. and Fischer, A. and Bippus, R.},
booktitle={IEEE International Conference on Acoustics, Speech, and Signal Processing (ICASSP 2001)},
title={Acoustic synthesis of training data for speech recognition in living room environments},
year={2001},
month={},
volume={1},
pages={21-24},
}


@Manual{bs-2570-manual,
  author =       "BSI",
  title =        "Natural Fibre Twines",
  organization = "British Standards Institution",
  address =      "London",
  edition =      "3rd",
  year =         "1973",
  note =         "BS 2570",
}

@Techreport{bs-2570-techreport,
  author =       "BSI",
  title =        "Natural Fibre Twines",
  institution =  "British Standards Institution",
  address =      "London",
  year =         "1973",
  type =         "BS",
  number =       "2570",
  note =         "3rd. edn.",
}


@Techreport{winget-67,
  author =       "{Winget Ltd.}",
  title =        "Detachable Bulldozer Attachment for Dumper Vehicles",
  year =         "1967",
  type =         "GB Patent Specification",
  number =       "1060631",
  month =        "8~" # mar,
}

@InProceedings{P1,
  author = 	 "Jones, C.D. and Roberts, E.F. and Smith, A.B.",
  title = "Paper Title",
  booktitle = "Proc. Conference Name",
  address = "Location",
  year = 	 "Year",
  pages = 	 "1--10"
}

@Book{B1,
  author = "Roberts, E.F. and Smith, A.B. and Jones, C.D.",
  title = "Book Title",
  publisher = "Publisher",
  year = "Year"
}

% REFS FROM LeMa06



@string{ieeeassp  = "IEEE Trans. Acoust. Speech Signal
                     Processing"}
@string{ieee_m_assp = "{IEEE} {ASSP} Magazine"}
@string{ieeetsa   = "IEEE Transactions on Audio, Speech, and Language Processing"}

@string{ieeetss = "IEEE Transactions on Speech and Audio Processing"}

@string{ieeesp    = "IEEE Transactions on Signal Processing"}

@string{ieeespl    = "IEEE Signal Processing Letters"}

@string{specom    = "Speech Communication"}

@string{jasa    = "Journal of the Acoustical Society of America"}

@string{icassp   = "Proc. International Conference on Acoustics, Speech, and Signal Processing (ICASSP)"}

@string{icslp   = "Proc. International Conference on Spoken Language Processing (ICSLP)"}

@string{ieeesamsp="Proc. IEEE Sensor Array and Multichannel Signal Processing Workshop"}

@string{sp="Signal Processing"}

@string{interspeech = "Proc. Interspeech"}

@string{eurospeech = "Proc. Eurospeech"}

@string{eusipco = "Proc. European Signal Processing Conference (EUSIPCO)"}

@string{propor = "Proc. International Conference on Computational Processing of Portuguese Language (PROPOR)"}

@string{fala = "Proc. FALA"}

@string{dsp = "Digital Signal Processing"}

@STRING{IEEE_J_ASSP = {{IEEE} Trans. Acoust., Speech, Signal Process.}}

@Inproceedings{apasci,
  author= "B. Angelini and F. Brugnara and D. Falavigna and D. Giuliani and R. Gretter and M. Omologo",
  title= "Speaker independent continuous speech recognition using an acoustic-phonetic {I}talian corpus",
  booktitle = icslp,
  year = "1994",
  pages= "1391--1394"
}


@Article{BovikMa93,
  author= "A. C. Bovik and P. Maragos and T. F. Quatieri",
  title= "{AM-FM} energy detection and separation in noise using multiband energy operators",
  journal = ieeesp,
  year = "1993",
  volume= "41",
  pages= "3245--3265",
  publisher = "IEEE"
}


@Article{dimitriadis06,
  author= "D. Dimitriadis and P. Maragos",
  title= "Continuous energy demodulation methods and application to speech analysis",
  journal = specom,
  year = "2006",
  volume= "48",
	number= "7",
  pages= "819--837"
}

@Article{dimitriadis05,
  author= "D. Dimitriadis and P. Maragos and A. Potamianos",
  title= "Robust {AM-FM} features for speech recognition",
  journal = ieeespl,
  year = "2005"
}


@Inproceedings{gridnews,
  author= "D. Dimitriadis and A. Metallinou and I. Konstantinou and G. Goumas and P. Maragos and N. Koziris",
  title= "{GRIDNEWS}: A distributed automatic {G}reek broadcast transcription system",
  booktitle = icassp,
  year = "2009"
}


@Article{gevag06,
  author= "G. Evangelopoulos and P. Maragos",
  title= "Multiband modulation energy tracking for noisy speech detection",
  journal = ieeetsa,
  year = "2006",
  volume= "14",
	number= "6",
  pages= "2024--2038"
}


@Article{DIRHA_D2.2,
  author= {M. Hagm\"{u}ller and others},
  title= "Experimental task definitions",
  journal = "Deliverable D2.2, DIRHA Consortium",
  month = feb,
  year = "2013"
}

@Article{DIRHA_D2.3,
  title= "Simulated acoustic corpora {II}",
  journal = "Deliverable D2.3, DIRHA Consortium",
  year = "2014"
}

@Article{DIRHA_D4.1,
  author= {G.Potamianos and others},
  title= "Robustness of distant--speech recognition and speaker identification-development of baseline system",
  journal = "Deliverable D4.1, DIRHA Consortium",
  month = feb,
  year = "2013"
}



@inproceedings{hermansky92,
  author= "H. Hermansky and N. Morgan and A. Bayya and P. Kohn",
  title= "{RASTA-PLP} speech analysis technique",
  booktitle = icassp,
  year = "1992"
}

@INPROCEEDINGS{MMI, 
author={L. {Bahl} and P. {Brown} and P. {de Souza} and R. {Mercer}}, 
booktitle={Proc. of ICASSP}, 
title={Maximum mutual information estimation of hidden Markov model parameters for speech recognition}, 
year={1986}, 
volume={11}, 
number={}, 
pages={49-52},
}

@Inproceedings{ravanelli,
  author= "M. Ravanelli and A. Sosi and P. Svaizer and M. Omologo",
  title= "Impulse response estimation for robust speech recognition in a reverberant environment",
  booktitle = "EUSIPCO 2012"
}


@INPROCEEDINGS{acw1,
author={Guoguo Chen and Parada, C. and Heigold, G.},
booktitle={ICASSP 2014},
title={Small-footprint keyword spotting using deep neural networks},
year={2014},
pages={4087-4091}
}

@Inproceedings{AISV,
  author= "M. Ravanelli and A. Sosi and M. Matassoni and M. Omologo and M. Benetti and G. Pedrotti",
  title= "DISTANT TALKING SPEECH RECOGNITION IN SURGERY ROOM : THE {DOMHOS} PROJECT",
  booktitle = "AISV",
  year = "2013"
}






@Inproceedings{aura,
  author= "M. Vorlander",
  title= "Auralization",
  booktitle = "Springer",
  year = "2007"
}



@Inproceedings{kutt,
  author= "H. Kuttruff",
  title= "Room acoustic",
  edition =      "5nd",
  booktitle = "Spon Press",
  year = "2009"
}









@Inproceedings{farina,
  author= "A. Farina",
  title= "Simultaneous Measurement of Impulse Response and Distortion with a Swept-Sine Technique",
  booktitle = "110th AES Convention",
  year = "February 2000"
}

@Inproceedings{matassoni,
  author= "M. Matassoni and M. Omologo and D. Giuliani and P. Svaizer",
  title= "{HMM} Training with Contaminated Speech Material for Distant-Talking Speech Recognition",
  booktitle = "COMPUTER SPEECH AND LANGUAGE",
  year = "2002"
}

@Inproceedings{lrec,
  author= "L. Cristoforetti and M. Ravanelli and M. Omologo and A. Sosi and A. Abad and M. Hagmueller and P. Maragos",
  title= "The {DIRHA} simulated corpus",
  booktitle = "LREC 2014",
  pages="2629--2634"
}



@Incollection{kaiser83,
  author= "J. F. Kaiser",
  title= "Some observations on vocal tract operation from a fluid flow point of view",
  booktitle = "Vocal Fold Physiology: Biomechanics, Acoustics, and Phonatory Control",
  editor = "I. R. Titze and R. C. Scherer",
  year = "1983",
  pages= "358--386",
  publisher = "Denver Center for Performing Arts",
  address = "Denver, CO"
}


@Inproceedings{lee+1993,
  author= "C. H. Lee and J. L. Gauvain",
  title= "Speaker adaptation based on {MAP} estimation of {HMM} parameters",
  booktitle = icassp,
  year = "1993",
  volume= "2",
  pages= "558--561"
}


@Article{leggetter+1995,
  author= "C. J. Leggetter and P. C. Woodland",
  title= "Maximum likelihood linear regression for speaker adaptation of continuous density hidden {M}arkov models",
  journal = "Computer Speech and Language",
  year = "1995",
  volume= "9",
	number= "2",
  pages= "171--185"
}

@Article{maragos93,
  author= "P. Maragos and J. F. Kaiser and T. F. Quatieri",
  title= "Energy separation in signal modulations with application to speech analysis",
  journal = ieeesp,
  year = "1993",
  volume= "41",
	number= "10",
  pages= "3024--3051"
}


@Article{DIRHA_D1.2,
  author= "M. Matassoni and others",
  title= "Definition of the evaluation plan",
  journal = "Deliverable D1.2, DIRHA Consortium",
  month = aug,
  year = "2012"
}


@Inproceedings{bdpublico,
  author= "J. P. Neto and C. A. Martins and H. Meinedo and L. B. Almeida",
  title= "The design of a large vocabulary speech corpus for {P}ortuguese",
  booktitle = eurospeech,
  year = "1997",
  pages= "1707--1710"
}

@Inproceedings{potamianos94,
  author= "A. Potamianos and P. Maragos",
  title= "Speech processing applications using {AM-FM} models and energy operators",
  booktitle = eusipco,
  year = "1994",
  volume= "3",
  pages= "1669--1672"
}

@Book{rabiner11,
  author= "L. R. Rabiner and R. W. Schafer",
  title= "Theory and Applications of Digital Speech Processing",
  publisher = "Prentice Hall, NJ",
  year = "2011"
}


@Book{bss,
  author= "Makino, S. and Lee, T. and Sawada, H.",
  title= "Blind Speech Separation",
  publisher = "Springer",
  year = "2010"
}


@Book{asr1,
  author= "De Mori, R.",
  title= "Spoken Dialogue With Computers.",
  publisher = "Academic Press",
  year = "1998"
}


@Book{rabiner_dsp,
  author= "L. R. Rabiner, B. Gold",
  title= "Spoken Dialogue With Computers.",
  publisher = "Prentice-Hall",
  year = "1975"
}



@Book{derev,
  author= "Naylor, P. A. and Gaubitch, N. D.",
  title= "Speech Dereverberation.",
  publisher = "Springer",
  year = "2010"
}


@Book{asr2,
  author= "Rabiner, L. and Juang, B. H.",
  title= "Fundamentals of speech recognition",
  publisher = "Prentice-Hall",
  year = "1993"
}



@INPROCEEDINGS{revch,
author={K. Kinoshita et al.},
booktitle={Proc. of WASPAA},
title={{The REVERB challenge: A Common Evaluation Framework for Dereverberation and Recognition of Reverberant Speech}},
year={2013},
pages={1-4}
}



@inproceedings{mikolov,
  title={Recurrent neural network based language model.},
  author={Mikolov, T. and Karafi{\'a}t, M. and Burget, L. and Cernock{\`y}, J. and Khudanpur, S.},
  booktitle={Proc. of Interspeech 2010},
  pages={1045--1048},
  year={2010}
}


@inproceedings{dirha_grid,
  title={{The DIRHA-GRID corpus: baseline and tools for multi-room distant speech recognition using distributed microphones}},
  author={Matassoni, M. and Astudillo, R. and Katsamanis, A. and Ravanelli, M.},
  booktitle={Proc. of Interspeech 2014},
  pages={1616--1617}
}

@inproceedings{hscma,
  title={A speech event detection and localization task for multiroom environments},
  author={Brutti, A. and Ravanelli, M. and  Svaizer, P. and  Omologo, M.},
  booktitle={Proc. of HSCMA 2014},
  pages={157-161},
  year={2014}
}


@inproceedings{evalita,
  title={{SASLODOM: Speech Activity detection and Speaker LOcalization in DOMestic environments}},
  author={Brutti, A. and Ravanelli, M. and  Omologo, M.},
  booktitle={EVALITA 2014},
  year={2014}
}


@INPROCEEDINGS{Povey,
         author = {Povey et al., D.},
          title = {{The Kaldi Speech Recognition Toolkit}},
      booktitle = {Proc. of ASRU},
      year = {2011}
}

@inproceedings{Watanabe2018,
  author={Shinji Watanabe and Takaaki Hori and Shigeki Karita and Tomoki Hayashi and Jiro Nishitoba and Yuya Unno and Nelson {Enrique Yalta Soplin} and Jahn Heymann and Matthew Wiesner and Nanxin Chen and Adithya Renduchintala and Tsubasa Ochiai},
  title={ESPnet: End-to-End Speech Processing Toolkit},
  year=2018,
  booktitle={Proc. Interspeech 2018},
  pages={2207--2211},
  doi={10.21437/Interspeech.2018-1456},
  url={http://dx.doi.org/10.21437/Interspeech.2018-1456}
}


@Inproceedings{ravanelli15,
  author= {Ravanelli, M. and Omologo, M.},
  title= {{Contaminated speech training methods for robust DNN-HMM distant speech recognition}},
  booktitle = {Proc. of Interspeech 2015},
  pages = {756--760}
}


@inproceedings{cnn_lecun,
 author = {LeCun, Y. and Haffner, P. and Bottou, L. and Bengio, Y.},
 title = {Object Recognition with Gradient-Based Learning},
 booktitle = {Shape, Contour and Grouping in Computer Vision},
 year = {1999},
 publisher = {Springer-Verlag},
 address = {London, UK, UK},
} 



@Inproceedings{rav_in14,
  author= {M. Ravanelli and M. Omologo},
  title= {{On the selection of the impulse responses for distant-speech recognition based on contaminated speech training}},
  booktitle = {Proc. of Interspeech 2014},
  pages = {1028--1032}
}





@inproceedings{IRs_paper,
  title={Impulse response estimation for robust speech recognition in a reverberant environment},
  author={Ravanelli, M. and Sosi, A. and Svaizer, P. and Omologo, M.},
  booktitle={Proc. of EUSIPCO 2012},
  pages={1668--1672}
}


@inproceedings{tb,
  author        = "Ravanelli, M. and Do, V.H. and Janin, A.",
  title         = "{TANDEM-Bottleneck Feature Combination using Hierarchical Deep Neural Networks}",
  booktitle     = "Proc. of ISCSLP 2014",
  pages={113-117},
   year = "2014"
}


@inproceedings{rover,
  title={{A post-processing system to yield reduced word error rates: Recognizer  output voting error reduction (ROVER)}},
  author={Fiscus, J. G.},
  booktitle={Proc. of ASRU 1997},
  pages={347--354},
  year={1997}
}

@inproceedings{ravanelli_eusipco,
 	author = {Ravanelli, M. and Elizalde, B. and Ni, K. and Friedland, G.},
 	title = {Audio Concept Classification with hierarchical deep neural networks},
 	booktitle = {European Signal Processing Conference},
 	year = {2014}
}

@article{stolke,
title = "Finding consensus in speech recognition: word error minimization and other applications of confusion networks ",
journal = "Computer Speech and Language ",
volume = "14",
number = "4",
pages = "373 - 400",
year = "2000",
author = "Mangu, L. and Brill, E. and Stolcke, A."
}

@inproceedings{cm,
author={Wessel, F. and Schluter, R. and Macherey, K. and Ney, H.},
journal={ IEEE Transactions on Speech and Audio Processing},
title={Confidence measures for large vocabulary continuous speech recognition},
year={2001},
month={March},
volume={9},
number={3},
pages={288-298}
}


@article{limabeam,
author={Seltzer, M.L. and Raj B. and Stern, R.M.},
journal={In IEEE Transactions on Speech and Audio Processing},
title={Likelihood-maximizing beamforming for robust hands-free speech recognition},
year={2004},
volume={12},
number={3},
month={September},
pages={489-498}
}


@Book{nn_1,
  author= "Bishop, C.M.",
  title= "Neural Networks for Pattern Recognition",
  publisher = "Oxford University Press",
  year = "1995"
}

@book{Beigi,
 author = {Beigi, H.},
 title = {Fundamentals of Speaker Recognition},
 year = {2011},
 publisher = {Springer},
} 


@book{book_interp,
 author = {C. Molnar},
 title = {Interpretable Machine Learning: A Guide for Making Black Box Models Explainable},
 year = {2018},
 publisher = {Leanpub},
} 


@inproceedings{lime,
 author = {Ribeiro, M. T. and Singh, S. and Guestrin, C.},
 title = {"Why Should I Trust You?": Explaining the Predictions of Any Classifier},
 booktitle = {Proc. of ACM SIGKDD},
 year = {2016},
 pages = {1135--1144},
} 

@INPROCEEDINGS{int_summary,
author={S. Chakraborty and others},
booktitle={Proc. of SmartWorld},
title={Interpretability of deep learning models: A survey of results},
year={2017},
}

@Article{int_visual,
author="Zhang, Q.-S.
and Zhu, S.-C.",
title="Visual interpretability for deep learning: a survey",
journal="Frontiers of Information Technology {\&} Electronic Engineering",
year="2018",
month="Jan",
volume="19",
number="1",
pages="27--39",
}

@incollection{capsule,
title = {Dynamic Routing Between Capsules},
author = {Sabour, S. and Frosst, N. and Hinton, G. E},
booktitle = {Proc. of NIPS},
pages = {3856--3866},
year = {2017},
}

@article{rbm1,
author={Hinton, G.E. and Osindero S. and Teh Y.},
journal={Neural Computation},
title={A fast learning algorithm for deep belief nets},
year={2006},
volume={18},
number={1},
pages={1527--1554,}
}


@InProceedings{understand_cnn,
author="Zeiler, M. D.
and Fergus, R.",
title="Visualizing and Understanding Convolutional Networks",
booktitle="Proc. of ECCV",
year="2014",
}

@ARTICLE{dnn_4,
author={Krizhevsky, A. and Sutskever, I. and Hinton, G. E.},
journal={Neural Computation},
title={ImageNet Classification with Deep Convolutional Neural Networks},
year={2012}
}


@inproceedings{exp_graph,
  author = {Zhang, Q. and Cao, R. and Shi, F. and Wu, Y. N. and Zhu, S.-C.},
  booktitle = {Proc. of AAAI},
  title = {Interpreting CNN Knowledge via an Explanatory Graph.},
  year = 2018
}


@article{int_audio,
  author    = {S. Becker and
               M. Ackermann and
               S. Lapuschkin and
               K.{-}R. M{\"{u}}ller and
               W. Samek},
  title     = {Interpreting and Explaining Deep Neural Networks for Classification
               of Audio Signals},
  journal   = {CoRR},
  volume    = {abs/1807.03418},
  year      = {2018}
}

@INPROCEEDINGS{ney,
author={Kneser, R. and Ney, H.},
booktitle={International Conference on Acoustics, Speech, and Signal Processing, ICASSP-95},
title={Improved backing-off for M-gram language modeling},
year={1995},
pages={181-184 vol.1}
}

@inproceedings{i-vect_short,
  author = {Sarkar, A. K. and Matrouf, D, and Bousquet, P.M. and Bonastre, J.F.},
  booktitle = {Proc. of Interspeech},
  pages = {2662-2665},
  title = {Study of the Effect of I-vector Modeling on Short and Mismatch Utterance Duration for Speaker Verification},
  year = 2012
}

@inproceedings{i-vect_short2,
	title = {Modified-prior i-{Vector} {Estimation} for {Language} {Identification} of {Short} {Duration} {Utterances}},
	booktitle = {Proc. of Interspeech},
	author = {Travadi, R. and Van Segbroeck, M., and Narayanan, S.,},
	year = {2014},
	pages = {3037--3041}
}

@inproceedings{i-vect_short3,
  author    = {A. Kanagasundaram and
               R. Vogt and
               D. Dean and
               S. Sridharan and
               M. Mason},
  title     = {i-vector Based Speaker Recognition on Short Utterances},
  booktitle = {Proc. of Interspeech},
  pages     = {2341--2344},
  year      = {2011},
}

@Inproceedings{dnn_5},
  author= {Salakhutdinov, R. R. and Hinton, G. E.},
  title= {Semantic Hashing},
  booktitle = {{In Proceedings of the SIGIR Workshop on Information Retrieval and Applications of Graphical Models}},
  year = {2007}
}

@inproceedings{dnn_speaker_rec_plp,
  author    = {F. Richardson and
               D. A. Reynolds and
               N. Dehak},
  title     = {A unified deep neural network for speaker and language recognition},
  booktitle = {Proc. of Interspeech},
  pages     = {1146--1150},
  year      = {2015}
}

@Inproceedings{dnn_6},
  author= "Collobert, R. and Weston, J.",
  title= "A Unified Architecture for Natural Language Processing: Deep Neural Networks with Multitask Learning",
  booktitle = "In Proceedings of the 25th International Conference on Machine Learnin",
  year = "2008"
}




@article{plp,
  author = {Hermansky H.},
  journal = {Journal of Acoustic Society of America (JASA)},
  number = 3,
  pages = {621-633},
  title = {{Perceptual linear predictive (PLP) analysis of speech}},
  volume = 28,
  year = 1990
}


@article{mllr,
  author = {Gales, M.J.F.},
  journal = {Computer Speech and Language},
  title = {{Maximum Likelihood Linear Transformations for HMM-Based Speech Recognition}},
  volume = 12,
  number = 4,
  pages = {75-98},
  year = 1998
}


@article{contamination,
  author = {Matassoni, M. and Omologo, M. and Giuliani, D. and Svaizer, P.},
  journal = {Computer Speech and Language},
  title = {{HMM Training with Contaminated Speech Material for Distant-Talking Speech Recognition}},
  volume = "16",
  number = "2",
   pages = "205 - 223",
  year = 2002
}


@article{rabiner,
    author = {Rabiner, L.},
    journal = {Proceedings of the IEEE},
    month = feb,
    number = {2},
    pages = {257--286},
    title = {{A tutorial on hidden Markov models and selected applications in speech recognition}},
    volume = {77},
    year = {1989}
}

@INPROCEEDINGS{pawel,
author={Renals, S. and Swietojanski, P.},
booktitle={Proc. of HSCMA 2014},
title={Neural networks for distant speech recognition},
pages={172-176},
year={2014}
}

@inproceedings{pawel2,
  author = {Swietojanski, P. and Ghoshal, A. and Renals, S.},
  title = {HYBRID ACOUSTIC MODELS FOR DISTANT AND MULTICHANNEL LARGE VOCABULARY SPEECH RECOGNITION},
  pages = {285--290},
  booktitle = {Proc. of ASRU 2013}
}

@INPROCEEDINGS{hain,
author={Y. Liu and P. Zhang and Hain, T.},
booktitle={Proc. of ICASSP 2014},
title={Using neural network front-ends on far field multiple microphones based speech recognition},
pages={5542-5546}
}

@inproceedings{droppo,
author = {J. Droppo and A. Acero},
booktitle={Proc. of ICASSP},
title = {Joint Discriminative Front End and Back End Training for Improved Speech Recognition Accuracy},
pages={281-284},
year = {2006},
}

@article{dnn_se1,
  title={An experimental study on speech enhancement based on deep neural networks},
  author={Xu, Y. and Du, J. and Dai, L. and Lee, C.},
  journal={IEEE Signal Processing Letters},
  volume={21},
  number={1},
  pages={65--68},
  year={2014},
}

@article{joint1,
  author    = {Z.Q. Wang and
               D. Wang},
  title     = {A Joint Training Framework for Robust Automatic Speech Recognition},
  journal   = {{IEEE/ACM} Trans. Audio, Speech {\&} Language Processing},
  volume    = {24},
  number    = {4},
  pages     = {796--806},
  year      = {2016}
}

@inproceedings{joint2,
  title={Joint noise adaptive training for robust automatic speech recognition},
  author={Narayanan, A. and Wang, D.},
  booktitle={Proc. of ICASSP},
  pages     = {4380--4384},
  year={2014},
}

@INPROCEEDINGS{joint3,
author={T. Gao and J. Du and L. R. Dai and C. H. Lee},
booktitle={Proc. of ICASSP},
title={Joint training of front-end and back-end deep neural networks for robust speech recognition},
year={2015},
pages={4375-4379}}

@inproceedings{joint6,
  author    = {Z. Chen and
               S. Watanabe and
               H. Erdogan and
               J. Hershey},
  title     = {Speech enhancement and recognition using multi-task learning of long short-term memory recurrent neural networks},
  booktitle = {Proc. of Interspeech},
  pages     = {3274--3278},
  year      = {2015},
}

@article{lstm,
 author = {Hochreiter, S. and Schmidhuber, J.},
 title = {Long Short-Term Memory},
 journal = {Neural Computation},
 volume = {9},
 number = {8},
 month = nov,
 year = {1997},
 pages = {1735--1780}
} 

@inproceedings{joint7,
  author    = {T. N. Sainath and R. J. Weiss and K. W. Wilson and A. Narayanan and M. Bacchiani, and A. Senior},
  title     = {Speaker Localization and Microphone Spacing Invariant Acoustic Modeling from Raw Multichannel Waveforms},
  booktitle = {Proc. of ASRU},
  year      = {2015},
}


@inproceedings{joint4,
  title={Joint Optimization of Denoising Autoencoder and DNN Acoustic Model Based on Multi-Target Learning for Noisy Speech Recognition},
  author={M. Mimura and S. Sakai and T. Kawahara},
  booktitle={Proc. of Interspeech},
  year={2016},
}

@inproceedings{joint5,
  title={Optimization of Speech Enhancement Front-End with Speech Recognition-Level Criterion},
  author={T. Higuchi and T. Yoshioka and T. Nakatani},
  booktitle={Proc. of Interspeech},
  year={2016},
}


@INPROCEEDINGS{ndnn1,
author={H. Erdogan and J. R. Hershey and S. Watanabe and J. Le Roux},
booktitle={Proc. of ICASSP},
title={Phase-sensitive and recognition-boosted speech separation using deep recurrent neural networks},
year={2015},
pages={708-712}
}


@inproceedings{batchnorm,
   title="Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift",
   Author={Ioffe, S. and Szegedy, C.},
   year="2015",
   Booktitle="Proc. of ICML",
   pages="448-456"
   } 

@ARTICLE{dnn_se2,
author={Y. Xu and J. Du and L. R. Dai and C. H. Lee},
journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
title={A Regression Approach to Speech Enhancement Based on Deep Neural Networks},
year={2015},
volume={23},
number={1},
pages={7-19},
month={Jan}}

@article{dropout,
  author  = {N. Srivastava and G. Hinton and A. Krizhevsky and I. Sutskever and R. Salakhutdinov},
  title   = {Dropout: A Simple Way to Prevent Neural Networks from Overfitting},
  journal = {Journal of Machine Learning Research},
  year    = {2014},
  volume  = {15},
  pages   = {1929-1958},
}


@inproceedings{Romero-et-al-ICLR2015-small,
       author = {Romero, A. and Ballas, N. and Ebrahimi K., Samira and Chassang, A. and Gatta, C. and Bengio, Y.},
        title = {FitNets: Hints for Thin Deep Nets},
         year = {2015},
  booktitle = {Proc. of ICLR},
}

@article{initbn,
  title={Recurrent Batch Normalization},
  author={Cooijmans, T. and Ballas, N. and Laurent, C. and G{\"u}l{\c{c}}ehre, {\c{C}}. and Courville, A.},
  journal={arXiv preprint arXiv:1603.09025},
  year={2016}
}

@article{know_matter,
  author  = {\c{C}. G\"{u}l\c{c}ehre and Y. Bengio},
  title   = {Knowledge Matters: Importance of Prior Information for Optimization},
  journal = {Journal of Machine Learning Research},
  year    = {2016},
  volume  = {17},
  number  = {8},
  pages   = {1-32}
}

@inproceedings{dnn_se3,
  author    = {F. Weninger and
               H. Erdogan and
               S. Watanabe and
               E. Vincent and
               J. Le Roux and
               J. R. Hershey and
               B. W. Schuller},
  title     = {Speech Enhancement with {LSTM} Recurrent Neural Networks and its Application to Noise-Robust {ASR}},
  booktitle = {Proc. of LVA/ICA},
  pages     = {91--99},
  year      = {2015}
}


@INPROCEEDINGS{dnn3,
author={A. Schwarz and C. Huemmer and R. Maas and W. Kellermann},
booktitle={Proc. of ICASSP 2015},
pages     = {4380--4384},
title={{Spatial Diffuseness Features for DNN-Based Speech Recognition in Noisy and Reverberant Environments}}
}




@article{IEEEexample:intro1,
  author	= "Dahl, G. and Yu, D. and Deng, L. and Acero, A.",    
  title =        "Context-Dependent Pre-trained Deep Neural Networks for Large Vocabulary Speech Recognition",
  journal = 	 "IEEE Transactions on Audio, Speech, and Language Processing",
  volume    = {20},
  number    = {1},
  year      = {2012},
  pages     = {30-42}
}


@inproceedings{dnn_rev,
 author = {Weninger, F. and Watanabe, S. and {Le Roux}, J. and Hershey, J.R. and Tachioka, Y. and Geiger, J. and Schuller, B. and Rigoll, G.},
    title = {{The MERL/MELCO/TUM System for the REVERB Challenge Using Deep Recurrent Neural Network Feature Enhancement}},
    booktitle = {IEEE REVERB Workshop},
    year = 2014,
    }
    
    
 @inproceedings{dnn_rev2,
 author = {M. Mimura, S. Sakai, and T. Kawahara},
    title = {REVERBERANT SPEECH RECOGNITION COMBINING DEEP NEURAL NETWORKS AND DEEP AUTOENCODERS},
    booktitle = {IEEE REVERB Workshop},
    year = 2014,
    }
    
    
    @inproceedings{online2,
  author = {Lei, Xin and Senior, Andrew and Gruenstein, Alexander and Sorensen, Jeffrey},
  booktitle = {in Proc. of Interspeech 2013},
  pages = {662-665},
  title = {Accurate and compact large vocabulary speech recognition on mobile devices.},
  year = 2013
}



@inproceedings{IEEEexample:intro2,
  author        = "H. Hermansky and S. Sharma",
  title         = "{TRAPS-Classifiers of temporal patterns}",
  intype        = "",
  booktitle     = "ICSLP",
  pages = {1003-1006},
  year          = "1998"
}

@incollection{bengio,
  author = {Bengio, Y. and Lamblin, P. and Popovici, D. and Larochelle, H.},
  booktitle = {Advances in Neural Information Processing Systems},
  pages = {153--160},
  publisher = {MIT Press},
  title = {Greedy layer-wise training of deep networks},
  year = 2007
}





@inproceedings{IEEEexample:intro3,
  author        = "B.Y. Chen",
  title         = "{Learning discriminant narrow-band temporal patters for automatic recognition of conversational telephone speech}",
  intype        = "",
  booktitle     = "Ph.D. dissertation, Univ. of California, Berkeley",
  year          = "2005"
}


@inproceedings{eusipco,
  author        = "M. Ravanelli and B. Elizalde and K. Ni and G. Friedland",
  title         = "{Audio Concept Classification with Hierarchical Deep Neural Networks}",
  intype        = "",
  booktitle     = "Proc. of EUSIPCO",
  year = 2014
}


@inproceedings{wsj_corpus,
 author = {P., Douglas and Baker, J. M.},
 title = {The Design for the Wall Street Journal-based CSR Corpus},
 booktitle = {Proceedings of the Workshop on Speech and Natural Language},
 series = {Proc. of HLT},
 year = {1992},
 pages = {357--362},
} 
    

@Article{IEEEexample:intro4,
  author	= "N. Morgan",    
  title =        "Deep and Wide: Multiple Layers in Automatic Speech Recognition",
  journal = 	 "IEEE Transactions on Audio, Speech, and Language Processing",
  volume    = {20},
  number    = {1},
  year      = {2012},
  pages     = {7-13}
}



@inproceedings{IEEEexample:intro5,
  author        = "A. Mohamed and G. Dahl and G. E. Hinton",
  title         = "{Deep Belief Networks for phone recognition}",
  intype        = "",
  booktitle     = "NIPS",
  year          = "2009"
}


@inproceedings{IEEEexample:intro6,
  author        = "C.M Bishop",
  title         = "{Neural Networks for Pattern Recognition}",
  intype        = "",
  booktitle     = "Oxford University Press",
  year          = "1995"
}



@Article{IEEEexample:intro7,
  author	= "H. Bourlard and N. Morgan",    
  title =        "Continuous speech recognition by connectionist statistical methods",
  journal = 	 "IEEE Transactions on Neural Networks",
  volume    = {4},
  number    = {6},
  year      = {1993},
  pages     = {893-909}
}



@inproceedings{IEEEexample:intro8,
  author        = "O. Vinyals and S.V. Ravuri",
  title         = "{Comparing Multilayer Perceptron to Deep Belief Network Tandem Features for robust ASR}",
  intype        = "",
  booktitle     = "ICASSP",
  pages     = {4596-4599 },
  year          = "2011"
}



@Article{IEEEexample:gab1,
  author	= "M. Kleinschmidt",    
  title =        "Methods for capturing spectro-temporal modulations in automatic speech recognition",
  journal = 	 "Acta Acustica united with Acustica",
  volume    = {88},
  number    = {3},
  year      = {2002},
  pages     = {416-422}
}


@inproceedings{IEEEexample:gab2,
  author        = "B.T. Meyer and B. Kollmeier",
  title         = "{Optimization and Evaluation of Gabor feature sets for ASR}",
  intype        = "",
  booktitle     = "Interspeech",
  pages = {906-909},
  year          = "2008"
}


@inproceedings{IEEEexample:gab3,
  author        = "B.T. Meyer and S. Ravuri and M.R. Schadler and N. Morgan",
  title         = "{Comparing Different Flavors of Spectro-Temporal Features for ASR}",
  intype        = "",
  booktitle     = "Interspeech",
  pages = {1269-1272},
  year          = "2011"
}



@Article{IEEEexample:gab4,
  author	= "M.R. Schadler and B.T. Meyer and B. Kollmeier",    
  title =        "Spectro-temporal Modulation Subspace-Spanning Filter Bank Features for Robust Automatic Speech Recognition",
  journal = 	 "Journal of the Acoustical Society of America",
  volume    = {131},
  number    = {5},
  year      = {2012},
  pages     = {4134-4152}
}



  @inproceedings{IEEEexample:gab6,
  author        = "M. Kleinschmidt",
  title         = "{Spectro-temporal Gabor features as a front end for automatic speech recognition}",
  intype        = "",
  booktitle     = "Forum Acusticum",
  year          = "2002"
}

@inproceedings{IEEEexample:tandem1,
  author        = "H. Hermansky and D. Ellis and S. Sharma",
  title         = "{Tandem connectionist feature extraction for conventional HMM systems}",
  intype        = "",
  booktitle     = "ICASSP 2000",
  pages     = {1635-1638},
  year          = "2000"
}


@inproceedings{IEEEexample:tandem2,
  author        = "H. Hermansky and P. Fousek",
  title         = "{Multi-resolution RASTA filtering for TANDEM-based ASR}",
  intype        = "",
  booktitle     = "Interspeech",
  pages = {361-364},
  year          = "2005"
}

  @inproceedings{IEEEexample:tandem3,
  author        = "M. Kleinschmidt and D. Gelbart",
  title         = "{Improving word accuracy with Gabor feature extraction}",
  intype        = "",
  booktitle     = "ICSLP",
  pages = {25-28},
  year          = "2002"
}

  @inproceedings{IEEEexample:tandem4,
  author        = "D. Ellis and R. Singh and S. Sivadas",
  title         = "TANDEM ACOUSTIC MODELING IN LARGE-VOCABULARY RECOGNITION",
  intype        = "",
  booktitle     = "ICASSP",
  pages = {517-520}, 
  year          = "2002"
}

  @inproceedings{IEEEexample:bn1,
  author        = "F. Gr\'ezl and M. Karafi\'at  and S. Kont\'ar and J. \v{C}ernock\'y",
  title         = "Probabilistic and bottle-neck features",
  intype        = "",
  booktitle     = "ICASSP 2007",
  pages = {757-760}, 
  year          = "2007"
}


  @inproceedings{IEEEexample:bn2,
  author        = "F. Gr\'ezl and P. Fousek",
  title         = "{Optimizing bottle-neck features for LVCSR}",
  intype        = "",
  booktitle     = "ICASSP",
  pages = {4729-4732}, 
  year          = "2008"
}


  @inproceedings{IEEEexample:bn3,
  author        = "F. Gr\'ezl and M. Karafi\'at and L. Burget",
  title         = "Investigation into bottle-neck features for meeting speech recognition",
  intype        = "",
  booktitle     = "Interspeech",
  pages = {2947-2950}, 
  year          = "2009"
}



  @inproceedings{IEEEexample:bn4,
  author        = "F. Valente and M.M. Doss and W. Wang",
  title         = "{Analysis and comparison of recent MLP features for LVCSR systems}",
  intype        = "",
  booktitle     = "Interspeech",
  pages = {1245-1248}, 
  year          = "2011"
}



  @inproceedings{IEEEexample:bn6,
  author        = "C. Plahl and R. Schluter and H. Ney",
  title         = "{Hierarchical Bottle-Neck Features for LVCSR}",
  intype        = "",
  booktitle     = "Interspeech",
  year          = "2010"
}



@inproceedings{IEEEexample:rbm1,
  author	= "G.E. Hinton and S. Osindero and Y. Teh",    
  title =        "A fast learning algorithm for deep belief nets",
  journal = 	 "Neural Computation",
  volume    = {18},
  year      = {2006},
  pages     = {1527-1554}
}


  @inproceedings{IEEEexample:rbm2,
  author        = "D. Yu and Michael L. Seltzer",
  title         = "{Improved Bottleneck Features Using Pretrained Deep Neural Networks}",
  intype        = "",
  booktitle     = "Interspeech",
  pages     = {237-240},
  year          = "2011"
}


 @inproceedings{IEEEexample:rbm3,
  author        = "O. Vinyals and S. V. Ravuri",
  title         = "{Comparing Multilayer Perceptron to Deep Belief Network Tandem Features for Robust ASR}",
  intype        = "",
  booktitle     = "ICASSP",
  pages     = {4596-4599},
  year          = "2011"
}
 

 @inproceedings{IEEEexample:rbm4,
  author        = "Y. Bengio and P. Lamblin and D. Popovici and H. Larochelle",
  title         = "{Greedy Layer-Wise Training of Deep Networks}",
  intype        = "",
  booktitle     = "NIPS",
  year          = "2006"
}

 @inproceedings{IEEEexample:rbm5,
  author        = "F. Seide and G. Li and X. Chen and D. Yu",
  title         = "{Feature Engineering in Context-Dependent Deep Neural Networks for Conversational Speech Transcription}",
  intype        = "",
  booktitle     = "ASRU",
  year          = "2011"
}

@inproceedings{IEEEexample:hbn1,
  author        = "F. Valente and J. Vepa and C. Plahl and C. Gollan and H. Hermansky, and R. Schluter",
  title         = "Hierarchical neural networks feature extraction for LVCSR system",
  intype        = "",
  booktitle     = "Interspeech",
  pages     = {42-45},
  year          = "2007"
}


  @inproceedings{IEEEexample:hbn2,
  author        = "F. Gr\'ezl and M. Karafi\'at",
  title         = "{Hierarchical Neural Net Architectures for Feature Extraction in ASR}",
  intype        = "",
  booktitle     = "Interspeech",
  pages = {1201-1204},
  year          = "2010"
}

  @inproceedings{IEEEexample:hbn3,
  author        = "F. Gr\'ezl and M. Karafi\'at and L. Brurget",
  title         = "{Investigation into Bottle-Neck Features for Meeting Speech Recognition}",
  intype        = "",
  booktitle     = "Interspeech",
  pages = {2947-2950},
  year          = "2009"
}

  @inproceedings{IEEEexample:msdnn,
  author        = "P. Zhou and L. Dai and Q. Liu and H. Jiang",
  title         = "{Combining Information from Multi-Stream Features Using Deep Neural Network in Speech Recognition}",
  intype        = "",
  booktitle     = "ICSP",
  pages = {557-561},
  year          = "2012"
}

@article{petar,
  author    = {P. Velickovic and
               W. Fedus and
               W. L. Hamilton and
               P. Li{\`{o}} and
               Y. Bengio and
               R. D. Hjelm},
  title     = {Deep Graph Infomax},
  journal   = {CoRR},
  volume    = {abs/1809.10341},
  year      = {2018}
}

@article{var_auto,
  author = {Kingma, D. P. and Welling, M.},
  title = {{Auto-Encoding Variational Bayes}},
  journal = {CoRR},
  volume = {abs/1312.6114},
  year = 2013,
}



  @inproceedings{IEEEexample:feacomb,
  author        = "C. Plahl and M. Kozielski and R. Schluter and H. Ney",
  title         = "{Feature Combination and Stacking of Recurrent and Non-Recurrent Neural Network for LVCSR}",
  intype        = "",
  booktitle     = "ICASSP",
  year          = "2013"
}



  @inproceedings{IEEEexample:na1,
  author        = "K. Riedhammer and V.H. Do and J. Hieronymus",
  title         = "{A Study on LVCSR and Keyword Search for Tagalog}",
  intype        = "",
  booktitle     = "Interspeech",
  year          = "2013"
}

  @inproceedings{IEEEexample:tnet1,
  author        = "K. Vesel\'y and L. Burget and F. Gr\'ezl",
  title         = "{Parallel Training of Neural Networks for Speech Recognition}",
  intype        = "",
  booktitle     = "Interspeech",
  pages = {439-446},
  year          = "2010"
}


  @inproceedings{IEEEexample:other1,
  author        = "J. Fiscus",
  title         = "{A Post-Processing System To Yield Reduced Word Error Rates: Recognizer Output Voting Error Reduction (ROVER)}",
  intype        = "",
  booktitle     = "ASRU",
  year          = "1997"
}

  @inproceedings{IEEEexample:other2,
  author        = "V.H. Do and X. Xiao and E. Chng",
  title         = "{Comparison and Combination of Multilayer Perceptrons and Deep Belief Networks in Hybrid Automatic Speech Recognition Systems}",
  intype        = "",
  booktitle     = "APSIPA",
  year          = "2011"
}

  @inproceedings{IEEEexample:other3,
  author        = "S. Young and D. Kershaw and J. Odell and D. Ollason and V. Valtchev and P. Woodland",
  title         = "{The HTK Book Version 3.0}",
  intype        = "",
  booktitle     = "Cambridge",
  year          = "2000"
}

  @inproceedings{IEEEexample:pitch1,
  author        = "B. Lee and D. Ellis",
  title         = "{Noise robust pitch tracking using subband autocorrelation classification (SAcC)}",
  intype        = "",
  booktitle     = "Interspeech",
  year          = "2012"
}

  @inproceedings{IEEEexample:pitch2,
  author        = "P. Bagshaw, S. Hiller, and M. Jack",
  title         = "{Enhanced pitch tracking and the processing of F0 contours for computer aided intonation teaching}",
  intype        = "",
  booktitle     = "EUROSPEECH",
  year          = "1993"
}

  @inproceedings{IEEEexample:lm1,
  author        = "R. Kneser and H. Ney",
  title         = "{Improved backing-off for m-gram language modeling}",
  intype        = "",
  booktitle     = "ICASSP 1995",
  pages = {181-184},
  year          = "1995"
}


article{rabiner,
  author = {Rabiner, L.},
  journal = {IEEE Transactions on Acoustics, Speech, and Signal Processing},
  number = 3,
  pages = {621-633},
  title = {{A tutorial on hidden Markov models and selected applications in speech recognition.},
  volume = 77,
  pages = {257-286},
  number = 2,
  year = 1989
}


@article{mfcc,
  author = {Davis, S. Mermelstein, P.},
  journal = {IEEE Transactions on Acoustics, Speech, and Signal Processing},
  number = 3,
  pages = {621-633},
  title = {{Comparison of Parametric Representations for Monosyllabic Word Recognition in Continuously Spoken Sentences.}},
  volume = 28,
  year = 1980
}


@article{chime,
  author = {J. Barker and E. Vincent and N. Ma and H. Christensen and P. Green},
  journal = {Computer Speech and Language},
  number = 3,
  pages = {621-633},
  title = {{The PASCAL CHiME speech separation and recognition challenge.}},
  volume = 27,
  year = 2013
}







@inproceedings{aec,
  title={{Comparison between Subband and fullband {NLMS} for in-Car audio compensation and handsfree speech recognition}},
  author={M. Omologo and C. Zieger},
  booktitle={Proc. of IWAENC 2005},
  pages={189--192},
  year={2005}
}


@inproceedings{chime3,
  title={{The third CHiME Speech Separation and Recognition Challenge: Dataset, task and baselines}},
  author={J. Barker and R. Marxer and E. Vincent and S. Watanabe },
  pages={504--511},
  year={2015},
  booktitle={Proc. of ASRU}
}





@article{ss,
  title={{Speech Enhancement Using a Minimum Mean-Square Error Short-Time Spectral Amplitude Estimator}},
  author={Ephraim, Y. and Malah, D.},
  journal={IEEE Transactions on Audio, Speech, and Language Processing},
  volume={32},
  number={6},
  pages={1109--1121},
  year={1984},
}


@article{nesta,
  title={{Batch-online semi-blind source separation applied to multi-channel acoustic echo cancellation}},
  author={F. Nesta and T. Wada and B. Juang},
  journal={IEEE Transactions on Audio, Speech, and Language Processing},
  volume={19},
  number={3},
  pages={583--599},
  year={2011},
  publisher={IEEE}
}


@article{aec2,
  title={{Frequency-domain and multirate adaptive filtering}},
  author={J. Shynk},
  journal={IEEE Signal Processing Magazine},
  volume={9},
  number={1},
  pages={14--37},
  year={1992}
}


@Inproceedings{cmutools,
  author= "R. Rosenfield and P. Clarkson",
  title= "Statistical language modeling using the {CMU}-{C}ambridge toolkit",
  booktitle = eurospeech,
  year = "1997"
}

@misc{BAScorpus,
  author        = "F. Schiel and A. Baumann",
  title         = "{PhonDat1} Corpus Documentation",
  url          = "http://www.phonetik.uni-muenchen.de/Bas/BasPD1README"
}

@Inproceedings{srilm,
  author= "A. Stolcke",
  title= "{SRILM} - An extensible language modeling toolkit",
  booktitle = icslp,
  year = "2002"
}




@Inproceedings{woodland:94,
  author= "P. C. Woodland and J. J. Odell and V. Valtchev and S. J. Young",
  title= "Large vocabulary continuous speech recognition using {HTK}",
  booktitle = icassp,
  year = "1994",
  volume= "2",
  pages= "125--128"
}

@Manual{htkbook,
  author = "S. Young and others",
  title = "{HTK} -- Hidden {M}arkov Model Toolkit", 
  howpublished = "Manual",
  url = "http://htk.eng.cam.ac.uk/",
  year = "2006"
}

@Inproceedings{nzlat12,
  author= "A. Zlatintsi and P. Maragos",							
  title= "{AM-FM} modulation features for music instrument signal analysis and recognition",
  booktitle = eusipco,
  year = "2012"
}

@misc{sampa,
  author        = "S. Young and others",
  title         = "{SAMPA} - Computer Readable Phonetic Alphabet",
  url = "http://www.phon.ucl.ac.uk/home/sampa/"
}


@Inproceedings{Abad2008,
  author= "A. Abad and J. Paulo da Silva Neto",							
  title= "Automatic classification and transcription of telephone speech in radio {B}roadcast data",
  booktitle= propor,
  year = "2008"
}


@Inproceedings{Abad2009,
  author= "A. Abad and I. Trancoso and N. Neto and M. do C\'{e}u Guerreiro Viana Ribeiro",							
  title= "Porting an {E}uropean {P}ortuguese {B}roadcast News Recognition System to {B}razilian {P}ortuguese",
  booktitle= interspeech,
  year = "2009"
}


@Article{Abad2012a,
  author= "A. Abad and A. Pompili and A. Costa and I. Trancoso and J. Fonseca and G. Leal and L. Farrajota and I.P. Martins",							
  title= "Automatic word naming recognition for an on-line aphasia treatment system",
  journal= "Computer Speech and Language",
  year = "2012"
}

@Inproceedings{Abad2012b,
  author= "A. Abad and H. Meinedo and I. Trancoso and J. Paulo da Silva Neto",							
  title= "Transcription of Multi-Variety {P}ortuguese Media Contents",
  booktitle= propor,
  year = "2012"
}


@Inproceedings{Adami2010,
  author= "A. G. Adami",							
  title= "Automatic speech recognition: from the beginning to {P}ortuguese language",
  booktitle = propor,
  year = "2010"
}


%%%% ISIDOROS


@Inproceedings{Koller2010,
	author= {O. Koller and A. Abadand and I. Trancoso and M. do Ceu Guerreiro Viana Ribeiro}, 
	title= "Exploiting Variety-Dependent Phones in {P}ortuguese Variety Identification Applied to Broadcast News Transcription",
    booktitle = interspeech,
    year= "2010"      
}
          
@Inproceedings{Lopes2012,
	author="J. Lopes and M. Eskenazi and I. Trancoso",
	title= "Incorporating {ASR} information in Spoken Dialog System confidence score",
	booktitle= propor,
	year=2012
}


@Inproceedings{Meinedo2003,
	author="H. Meinedo and D. Ant\'{o}nio Caseiro and J. Paulo da Silva Neto and I. Trancoso", 
	title="{AUDIMUS}.media: a Broadcast News speech recognition system for the {E}uropean {P}ortuguese language",
	booktitle=propor,
	year="2003"
}	

@Inproceedings{Meinedo2008,
	author="H. Meinedo and A. Abad and T. Pellegrini and I. Trancoso and J. Paulo da Silva Neto", 
	title="The {L2F} Broadcast News Speech Recognition System", 
	booktitle=fala,
	month = nov,
	year=2010,
	address = "Vigo, Spain"
}

@Inproceedings{Neves2008,
	author="Luis Miguel Leitao Neves and Ciro Alexandre Domingues Martins and Hugo Meinedo and Joao Paulo da Silva Neto", 
	title="Domain adaptation of a Broadcast News Transcription System
			for the {P}ortuguese Parliament",
	booktitle=propor,
	year=2008
}


@Inproceedings{Trancoso2006,
	author="Isabel Trancoso and Ricardo Jorge Francisco Nunes and Luis Miguel Leitao Neves and Maria do C\'{e}u Guerreiro Viana Ribeiro and Helena Moniz and Diamantino Antonio Caseiro and Ana Isabel Mata da Silva",
	title="Recognition of Classroom Lectures in {E}uropean {P}ortuguese",
	booktitle= interspeech,
	pages="281--284",
	year="2006"
}
	 
@Inproceedings{word,
	author={L. Ferrer and E. Shriberg and S. Kajarekar and A. Stolcke and K. S\"{o}nmez and A. Venkataraman and H. Bratt},
	title="The contribution of cepstral and stylistic features to {SRI}'s 2005 {NIST} speaker recognition evaluation system",
	booktitle=icassp,
	year=2006,
	volume=1,
	pages="101--104"
}


@Inproceedings{duration,
	author={Ferrer, L. and Bratt, H. and Gadde, V. R. R. and Kajarekar, S. and Shriberg, E. and S\"{o}nmez, K. and Stolcke, A. and Venkataraman, A.},
	title="Modeling duration patterns for speaker recognition",
	booktitle=eurospeech,
	year=2003,
	pages="2017--2020",
	address="Geneva",
}

@Article{prosodic,
	author="Shriberg, E. and Ferrer, L. and Kajarekar, S. S. and Venkataraman, A. and Stolcke, A.",
	title="Modeling Prosodic Feature Sequences for Speaker Recognition",
	journal=specom,
	volume= 46,
	number = "3--4",
	pages= "455--472",
	year=2005
}

@Article{rasta,
	author="Hermansky, H. and Morgan, N.",
	title="{RASTA} processing of speech",
	journal=ieeetss,
	volume=2,
	number = "4",
	pages="578--589",
	month = oct,
	year=1994
}

%%
@Inproceedings{warping,
	author="Pelecanos, J. and Sridharan, S.",
	title="Feature warping for robust speaker verification",
	booktitle="Proc. of Odyssey Speaker and Language Recognition Workshop",
	year=2001,
        pages = "213--218"
}


@INPROCEEDINGS{gmm-free,
AUTHOR = "Andrew W. Senior and Georg Heigold and Michiel Bacchiani and Hank Liao",
TITLE = "{{GMM-free DNN acoustic model training}}",
BOOKTITLE = "ICASSP 20014",
PAGES = {5602-5606},
YEAR = {2014}, 
}

@INPROCEEDINGS{kaldi,
         author = {Povey, D. and Ghoshal, A. and Boulianne, G. and Burget, L. and Glembek, O. and Goel, N. and Hannemann, M. and Motlicek, P. and Qian, Y. and Schwarz, P. and Silovsky, J. and Stemmer, G. and Vesely, K.},
          title = {{The Kaldi Speech Recognition Toolkit}},
      booktitle = {Proc. of ASRU},
           year = {2011}
}

@ARTICLE{theano,
   author = {{Theano Development Team}},
    title = "{Theano: A {Python} framework for fast computation of mathematical expressions}",
  journal = {arXiv e-prints},
   volume = {abs/1605.02688},
     year = 2016,
    month = may
}

@misc{WinNT,
  title = {{MS Windows NT} Kernel Description},
  howpublished = {\url{http://web.archive.org/web/20080207010024/http://www.808multimedia.com/winnt/kernel.htm}},
  note = {Accessed: 2010-09-30}
}


@INPROCEEDINGS{xavier,
    author = {X. Glorot and Y. Bengio},
    title = {Understanding the difficulty of training deep feedforward neural networks},
    booktitle = {Proc.  of AISTATS},
    year = {2010},
    pages={249-256}
}

@INPROCEEDINGS{kpitch,
author={Ghahremani, P. and BabaAli, B. and Povey, D. and Riedhammer, K. and Trmal, J. and Khudanpur, S.},
booktitle={Proc. of ICASSP 2014 },
title={A pitch extraction algorithm tuned for automatic speech recognition},
year={2014},
pages={2494-2498}
}

@Inproceedings{gretter,
  author= "R. Gretter",
  title= "Euronews: a multilingual speech corpus for {ASR}",
  booktitle = "LREC 2014",
  pages = {2635--2638},
  year={2014}
}

@Inproceedings{apasci1,
  author= "B. Angelini and F. Brugnara and D. Falavigna and D. Giuliani and R. Gretter and M. Omologo",
  title= "Speaker independent continuous speech recognition using an acoustic-phonetic {I}talian corpus",
  booktitle = "icslp",
  year = "1994",
  pages= "1391--1394"
}

@Article{score,
	author="Auckenthaler, R. and Carey, M. J. and Lloyd-Thomas, H.",
	title="Score Normalization for Text-Independent Speaker Verification Systems",
	journal=dsp,
	volume=10,
	pages="42--54",
        number="1--3",
	year=2000
}
%



@Inproceedings{image,
	author="J.B. Allen and D.A. Berkley",
	title="Image method for efficiently simulating small‐room acoustics",
	booktitle="J. Acoust. Soc. Am",
    pages="2425--2428",
	year=1979
}

    
@Inproceedings{mearev,
	author="M.R Schroeder",
	title="New Method of Measuring Reverberation Time",
	booktitle="J. Acoust. Soc. Am",
    pages="",
	year=1965
}

    
    
     
    
@Inproceedings{tnsvm,
	author="Abad, A. and Trancoso, I.",
	title="Speaker Recognition Experiments using Connectionist Transformation Network Features",
	booktitle=interspeech,
	year=2010,
	pages="378--381"
}
%%
@Article{gmm_ubm,
	author="Reynolds, D. A. and Quatieri, T. F. and Dunn, R. B.",
	title="Speaker verification using adapted {G}aussian mixture models",
	journal="Digital Signal Processing",
	volume=10,
        number="1--3",
	pages="19--41",
	year="2000"
}	

@Article{gsv,
	author="Campbell, W. M. and Sturim, D. E. and Reynolds, D. A.",
	title="Support vector machines using {GMM} supervectors for speaker verification",
	journal=ieeespl,
	volume=13,
	number=5,
	pages="308--311",
	year=2006
}	

@Inproceedings{ivector,
	author="Dehak, N. and Dehak, R. and Kenny, P. and {Br\"{u}mmer}, N. and Ouellet, P. and Dumouchel, P.",
	title="Support vector machines versus fast scoring in the low-dimensional total variability space for speaker verification",
	booktitle=interspeech,
	year=2009,
	pages="1559--1562"
}
%%
@Article{jfa,
	author="Kenny, P. and Boulianne,  G. and Ouellet, P. and Dumouchel, P.",
	title="Joint factor analysis versus eigenchannels in speaker recognition",
	journal=ieeetsa,
	volume=15,
	number=4, 
	pages="1435--1447",
	year="2007"
}

@Inproceedings{dicit2008,
	author="M. Omologo",
	title="Front-end processing of a distant-talking speech interface for control of an interactive {TV} system",
	booktitle="Proc. of  Acoustics",
	year=2008,
	pages="1425--1429"
}

@Inproceedings{fakotakis97,
	author="Chatzi, I. and Fakotakis, N. and Kokkinakis, G.",
	title="Greek speech database for creation of voice driven teleservices",
	booktitle=eurospeech,
	year=1997
}	 

@Inproceedings{fakotakis09,
	author="Mporas, I. and Ganchev, T. and Kostoulas, T. and Kermanidis, K. and Fakotakis, N.",
	title="Automatic Speech Recognition System for Home Appliances Control",
	booktitle="Proc. 13th Panhellenic Conference on Informatics (PCI)",
	year=2009,
	pages="114--117",
}	
%
@Inproceedings{oikonomidis03,
	author="Oikonomidis, D. and Digalakis, V.",
	title="Stem-based Maximum Entropy Language Models for Inflectional Languages",
	booktitle=eurospeech,
	year=2003
}	

@Article{digalakis66,
	author="Digalakis, V. and Monaco, P. and Murveit, H.",
	title="Genones: Generalized Mixture Tying in Continuous Hidden {M}arkov Model-Based Speech Recognizers",
	 journal=ieeetss,
	 pages="281--289",
	 month=jul,
	 year=1996
}	 
%%


@Inproceedings{Meinedo2010,
	author="H. Meinedo and A. Abad and T. Pellegrini and I. Trancoso and J. Neto",
	title="The {L2F} {B}roadcast news speech recognition system",
	booktitle="Proc. FALA",
	year=2010
}	

@Book{JurafskyMartin09,
  author= "D. Jurafsky and Martin, J. H.",
  title= "Speech and Language Processing. An Introduction to Natural Language Processing, Computational Linguistics, and Speech Recognition",
  publisher = "Pearson",
  year = 2009
}

@Book{BenestySondhi08,
  editor= "J. Benesty and Sondhi, M. M. and Y. Huang",
  title= "Springer Handbook of Speech Processing",
  publisher = "Springer",
  year = 2008
}

@Book{RabinerJuang93,
  author= "Rabiner, L. R. and Huang, B.-H.",
  title= "Fundamentals of Speech Recognition",
  publisher = "Prentice-Hall",
  year = 1993
}

@inproceedings{Falavigna2012,
    Author = {Daniele Falavigna and Roberto Gretter},
    Title = {Focusing Language Models For Automatic Speech Recognition},
    Booktitle = {Proc. International Workshop on Spoken Language Translation (IWSLT)},
    Pages = {171--178},
    Year = {2012}
}

@inproceedings{gcf,
  title={Acoustic event localization using a crosspower-spectrum phase based technique},
  author={Omologo, M. and Svaizer, P.},
  booktitle={Proc. of ICASSP},
  pages={273--276},
  year={1994},
}

@article{Bertoldi2002,
    Author = {N. Bertoldi and F. Brugnara and M. Cettolo and M. Federico and D. Giuliani},
    Title = {Cross-Task Portability of a Broadcast News Speech Recognition System},
    Journal = {Speech Communication},
    Pages = {335-347},
    Volume = {38},
    Number = {3-4},
    Year = {2002}
}

@inproceedings{Bertoldi2001,
    Author = {N. Bertoldi and F. Brugnara and M. Cettolo and M. Federico and D. Giuliani},
    Title = {From {B}roadcast News to Spontaneous Dialogue Transcription: {P}ortability Issues},
    Booktitle = {Proc. International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
    Year = {2001}
}

@inproceedings{Girardi2011,
  author    = {Christian Girardi and
               Roberto Gretter and
               Daniele Falavigna and
               Fabio Brugnara and
               Diego Giuliani and
               Marcello Federico},
  title     = {{NeMo}: A Platform for Multilingual News Monitoring},
  booktitle = {Proc. Interspeech},
  year      = {2011},
  pages     = {2261--2264}
}

@inproceedings{Falavigna2010,
 author = {Falavigna, Daniele and Gerosa, Matteo and Giuliani, Diego and Gretter, Roberto},
 title = {An automatic transcription system of hearings in {I}talian courtrooms},
 booktitle = {Proc. ACM Workshop on Multimedia in Forensics, Security and Intelligence (MiFor)},
 year = {2010},
 pages = {99--104},
} 

@inproceedings{Falavigna2011,
  author    = {Daniele Falavigna and Roberto Gretter},
  title     = {Cheap Bootstrap of Multi-Lingual Hidden {M}arkov Models},
  booktitle = {Proc. Interspeech},
  year      = {2011},
  pages     = {2325-2328}
}

@article{Gerosa2009,
author = "Matteo Gerosa and Diego Giuliani and Fabio Brugnara",
title = "Towards age-independent acoustic modeling",
journal = "Speech Communication",
volume = "51",
number = "6",
pages = "499 - 509",
year = "2009",
}

@INPROCEEDINGS{Federico2008,
AUTHOR = "Marcello Federico and Nicola Bertoldi and Mauro Cettolo",
TITLE = "{IRSTLM}: an open source toolkit for handling large scale language models",
BOOKTITLE = "Proc. Interspeech",
PAGES = {1618--1621},
YEAR = {2008} 
}

@INPROCEEDINGS{dicit2009,
author={Marquardt, L. and Svaizer, P. and Mabande, E. and 
, A. and Zieger, C. and Omologo, M. and Kellermann, W.},
title={A natural acoustic front-end for Interactive {TV} in the {EU}-{P}roject {DICIT}},
booktitle={Proc. Pacific Rim Conference on Communications, Computers and Signal Processing}, 
year={2009},
pages={894--899}
}

@article{Brutti2010,
  author    = {Alessio Brutti and
               Luca Cristoforetti and
               Walter Kellermann and
               Lutz Marquardt and
               Maurizio Omologo},
  title     = {{WOZ} acoustic data collection for interactive {TV}},
  journal   = {Language Resources and Evaluation},
  volume    = {44},
  number    = {3},
  year      = {2010},
  pages     = {205--219}

}

@INPROCEEDINGS{bocchieri13,
author	= {Bocchieri, Enrico and Dimitriadis, Dimitrios},
title	= {INVESTIGATING DEEP NEURAL NETWORK BASED TRANSFORMS OF ROBUST AUDIO FEATURES FOR {LVCSR}},
booktitle	= icassp,
year	= {2013}
}

@INPROCEEDINGS{fiscus97,
author = {J. G. Fiscus},
title = {A post-processing system to yield reduced word error rates: Recognizer output voting error reduction ({ROVER})},
booktitle= {Proc. Automatic Speech Recognition and Understanding Workshop}, 
pages = {347--352},
year = {1997}
}

@INPROCEEDINGS{stolcke97,
  title={Explicit word error minimization in n-best list rescoring.},
  author={Stolcke, Andreas and Konig, Yochai and Weintraub, Mitchel},
  booktitle=eurospeech,
  volume={97},
  pages={163--166},
  year={1997}
}

@INPROCEEDINGS{xu10,
  title={An improved consensus-like method for minimum bayes risk decoding and lattice combination},
  author={Xu, Haihua and Povey, Daniel and Mangu, Lidia and Zhu, Jie},
  booktitle=icassp,
  pages={4938--4941},
  year={2010}
}

@INPROCEEDINGS{irodoma13b,
  title={Advances In Large Vocabulary Continuous Speech Recognition In {G}reek: {M}odeling And Nonlinear Features},
  author={Isidoros Rodomagoulakis and Gerasimos Potamianos and Petros Maragos},
  booktitle=eusipco,
  year={2013}
}

@INPROCEEDINGS{nkatsam14,
title={ROBUST FAR-FIELD SPOKEN COMMAND RECOGNITION FOR HOME AUTOMATION COMBINING ADAPTATION AND MULTICHANNEL PROCESSING},
author={Athanasios Katsamanis and Isidoros Rodomagoulakis and Gerasimos Potamianos and Petros Maragos and Antigoni Tsiami},
booktitle={(TO APPEAR in {ICASSP} 2014)}
}

@inproceedings{neti00,
  title={Audio-visual speech recognition},
  author={Neti, Chalapathy and Potamianos, Gerasimos and Luettin, Juergen and Matthews, Iain and Glotin, Herve and Vergyri, Dimitra and Sison, June and Mashari, Azad and Zhou, Jie},
  booktitle={Final Workshop 2000 Report},
  volume={764},
  year={2000}
}


% This file was created with JabRef 2.9.2.
% Encoding: MacRoman

@ARTICLE{Barker13,
  author = {Barker, J. and Vincent, E. and Ma, N. and Christensen, H. and Green,
	P.},
  title = {The {PASCAL} {CHiME} speech separation and recognition challenge},
  journal = J_CSL,
  year = {2013},
  volume = {27},
  pages = {621-633},
  number = {3}
}

@BOOK{Benesty08,
  title = {Microphone Array Signal Processing},
  publisher = {Springer},
  year = {2008},
  author = {Benesty, J. and Chen, J. and Huang, Y.},
  volume = {1}
}

@ARTICLE{Chan08,
  author = {Chan, M. and Estève, D. and Escriba, C. and Campo, E.},
  title = {A review of smart homes - {P}resent state and future challenges},
  journal = {Computer Methods and Programs in Biomedicine},
  year = {2008},
  volume = {91},
  pages = {55-81},
  number = {1}
}


@inproceedings{bottleneck_spk_rec,
  author    = {S. Yaman and
               J. W. Pelecanos and
               R. Sarikaya},
  title     = {Bottleneck features for speaker recognition},
  booktitle = {Proc. of Speaker Odyssey},
  pages     = {105--108},
  year      = {2012}
}


@inproceedings{classify_ivect,
  author    = {T. Stafylakis and
               P. Kenny and
               M. Senoussaoui and
               P. Dumouchel},
  title     = {Preliminary investigation of Boltzmann machine classifiers for speaker
               recognition},
  booktitle = {Speaker Odyssey},
  pages     = {109--116},
  year      = {2012}
}


@inproceedings{tara_raw,
  author    = {T. N. Sainath and
               R. J. Weiss and
               A. W. Senior and
               K. W. Wilson and
               O. Vinyals},
  title     = {{Learning the speech front-end with raw waveform CLDNNs}},
  booktitle = {Proc. of Interspeech},
  year      = {2015},
}


@inproceedings{raw_speaker_id,
  author    = {Muckenhirn, H. and Magimai-Doss, M. and Marcel,  S.},
  title     = {{Towards directly modeling raw speech signal for speaker  verification using CNNs}},
  booktitle = {Proc. of ICASSP},
  year      = {2018}
}

@inproceedings{spk_rec_time_freq,
  author    = {G. Bhattacharya and
               J. Alam and
               P. Kenny},
  title     = {Deep Speaker Embeddings for Short-Duration Speaker Verification},
  booktitle = {Proc. of {Interspeech}},
  pages     = {1517--1521},
  year      = {2017}
}

@ARTICLE{dnn_speaker_rec2,
author={F. Richardson and D. Reynolds and N. Dehak},
journal={IEEE Signal Processing Letters},
title={Deep Neural Network Approaches to Speaker and Language Recognition},
year={2015},
volume={22},
number={10},
pages={1671-1675},
}

@INPROCEEDINGS{Chen13,
  author = {Chen, I.-F. and Lee, C.-H},
  title = {A Resource-Dependent Approach to Word Modeling for Keyword Spotting},
  booktitle = interspeech,
  year = {2013}
}


@INPROCEEDINGS{speaker_rec_dnn,
author={M. McLaren and Y. Lei and L. Ferrer},
booktitle={Proc. of ICASSP},
title={Advances in deep neural network approaches to speaker recognition},
year={2015},
volume={},
number={},
pages={4814-4818},
}


@INPROCEEDINGS{Kenny_deepneural,
    author = {P. Kenny and V. Gupta and T. Stafylakis and P. Ouellet and J. Alam},
    title = {Deep Neural Networks for extracting Baum-Welch statistics for Speaker Recognition},
    booktitle = {Proc. of Speaker Odyssey},
    year = {2014}
}


@INCOLLECTION{CMP06,
  author = {Chu, S.M. and Marcheret, E. and Potamianos, G.},
  title = {Automatic Speech Recognition and Speech Activity Detection in the
	{CHIL} Smart Room},
  booktitle = {Machine Learning for Multimodal Interaction},
  publisher = {Springer Berlin Heidelberg},
  year = {2006},
  editor = {Renals, S. and Bengio, S.},
  owner = {nassos},
  timestamp = {2013.11.04}
}

@INPROCEEDINGS{logotypographia,
  author = {Digalakis, V. and Oikonomidis, D. and Pratsolis, D. and Tsourakis,
	N. and Vosnidis, C. and Chatzichrisafis, N. and Diakoloukas, V.},
  title = {Large vocabulary continuous speech recognition in {G}reek: {C}orpus
	and an automatic dictation system},
  booktitle = interspeech,
  year = {2003}
}

@ARTICLE{Keshet09,
  author = {Keshet, J. and Grangier, D. and Bengio, S.},
  title = {Discriminative keyword spotting},
  journal = {Speech Communication},
  year = {2009},
  volume = {51},
  pages = {317-329},
  number = {4}
}

@ARTICLE{Kumatani12,
  author = {Kumatani, K. and McDonough, J. and Raj, B.},
  title = {Microphone Array Processing for Distant Speech Recognition: {F}rom
	Close-Talking Microphones to Far-Field Sensors},
  journal = IEEE_M_SP,
  year = {2012},
  volume = {29},
  pages = {127-140},
  number = {6}
}

@INPROCEEDINGS{LVP11,
  author = {Lecouteux, B. and Vacher, M. and Portet, F.},
  title = {Distant speech recognition in a smart home: {C}omparison of several
	multisource {ASR}s in realistic conditions},
  booktitle = interspeech,
  year = {2011},
  pages = {2273-2276}
}

@ARTICLE{Lefkimmiatis07,
  author = {Lefkimmiatis, S. and Maragos, P.},
  title = {A generalized estimation approach for linear and nonlinear microphone
	array post-filters},
  journal = {Speech Communication},
  year = {2007},
  volume = {49},
  pages = {657-666},
  number = {7-8}
}

@INPROCEEDINGS{Mandal13,
  author = {Mandal, A. and Hout, J. and Tam, Y.-C. and Mitra, V. and Lei, Y.
	and Zheng, J. and Vergyri, D. and Ferrer, L. and Graciarena, M. and
	Kathol, A. and Horacio, F.},
  title = {Strategies for High Accuracy Keyword Detection in Noisy Channels},
  booktitle = interspeech,
  year = {2013}
}

@book{mitra,
 author = {Mitra, S. K.},
 title = {Digital Signal Processing},
 year = {2005},
 publisher = {McGraw-Hill},
} 

@INPROCEEDINGS{tara_asru2013,
author={T. N. Sainath and B. Kingsbury and A. R. Mohamed and B. Ramabhadran},
booktitle={Proc. of ASRU},
title={Learning filter banks within a deep neural network framework},
year={2013},
pages={297-302},
}


@ARTICLE{learn_fbank_const,
author={H. Yu and Z. H. Tan and Y. Zhang and Z. Ma and J. Guo},
journal={IEEE Access},
title={{DNN Filter Bank Cepstral Coefficients for Spoofing Detection}},
year={2017},
volume={5},
number={},
pages={4779-4787},
}

@INPROCEEDINGS{fbank_par,
author={H. Seki and K. Yamamoto and S. Nakagawa},
booktitle={Proc. of ICASSP},
title={A deep neural network integrated with filterbank learning for speech recognition},
year={2017},
pages={5480-5484},
}


@ARTICLE{Mat+02,
  author = {Matassoni, M. and Omologo, M. and Giuliani, D. and Svaizer, P.},
  title = {Hidden {M}arkov model training with contaminated speech material
	for distant-talking speech recognition },
  journal = J_CSL,
  year = {2002},
  volume = {16},
  pages = {205-223},
  number = {2},
  doi = {http://dx.doi.org/10.1006/csla.2002.0191},
  issn = {0885-2308},
  url = {http://www.sciencedirect.com/science/article/pii/S0885230802901919}
}

@INPROCEEDINGS{Mporas09,
  author = {Mporas, I. and Ganchev, T. and Kostoulas, T. and Kermanidis, K. and
	Fakotakis, N.},
  title = {Automatic Speech Recognition System for Home Appliances Control},
  booktitle = {13th Panhellenic Conference on Informatics},
  year = {2009},
  pages = {114-117}
}

@ARTICLE{Omologo97,
  author = {Omologo, M. and Svaizer, P.},
  title = {Use of the crosspower-spectrum phase in acoustic event location},
  journal = IEEE_J_SAP,
  year = {1997},
  volume = {5},
  pages = {288-292}
}

@INPROCEEDINGS{Ost+91,
  author = {Ostendorf, M. and Kannan, A. and Austin, S. and Kimball, O. and Schwartz,
	R. M. and Rohlicek, J. R.},
  title = {Integration of Diverse Recognition Methodologies Through Reevaluation
	of {N}-{B}est Sentence Hypotheses.},
  booktitle = C_HLT,
  year = {1991},
  pages = {83-87},
  url = {http://acl.ldc.upenn.edu/H/H91/H91-1013.pdf},
  urldate = {2013-09-06}
}

@INPROCEEDINGS{Pri+13,
  author = {Principi, Emanuele and Squartini, Stefano and Piazza, Francesco and
	Fuselli, Danilo and Bonifazi, Maurizio},
  title = {A Distributed System for Recognizing Home Automation Commands and
	Distress Calls in the {I}talian Language},
  booktitle = interspeech,
  year = {2013},
  owner = {nassos},
  timestamp = {2013.10.10}
}

@INPROCEEDINGS{Rav+12,
  author = {Ravanelli, M. and Sosi, A. and Svaizer, P. and Omologo, M.},
  title = {Impulse response estimation for robust speech recognition in a reverberant
	environment},
  booktitle = EURASIP_C_EUSIPCO,
  year = {2012},
  pages = {1668-1672}
}

@INPROCEEDINGS{RSGMP13,
  author = {Rodomagoulakis, I. and Giannoulis, P. and Skordilis, Z.-I. and Maragos,
	P. and Potamianos, G.},
  title = {Experiments on Far-field Multichannel Speech Processing in Smart
	Homes},
  booktitle = {Proc. 18th Int. Conf. Digital Signal Processing},
  year = {2013},
  owner = {nassos},
  timestamp = {2013.11.04}
}

@INPROCEEDINGS{RPM13,
  author = {Rodomagoulakis, I. and Potamianos, G. and Maragos, P.},
  title = {Advances In Large Vocabulary Continuous Speech Recognition In {G}reek:
	{M}odeling And Nonlinear Features},
  booktitle = eusipco,
  year = {2013}
}

@INCOLLECTION{SeKe08,
  author = {Sehr, A. and Kellermann, W.},
  title = {Towards Robust Distant-Talking Automatic Speech Recognition in Reverberant
	Environments},
  booktitle = {Speech and Audio Processing in Adverse Environments},
  publisher = {Springer Berlin Heidelberg},
  year = {2008},
  editor = {H\"{a}nsler, E. and Schmidt, G.},
  pages = {679-728},
  owner = {nassos},
  timestamp = {2013.11.04}
}

@ARTICLE{Smith87,
  author = {Smith, J.O. and Abel, J.S.},
  title = {Closed-form least-squares source location estimation from range-difference
	measurements},
  journal = {Acoustics, Speech and Signal Processing, IEEE Transactions on},
  year = {1987},
  volume = {35},
  pages = {1661-1669},
  number = {12}
}

@INPROCEEDINGS{Vac+13,
  author = {Vacher, M. and Lecouteux, B. and Istrate, D. and Joubert, T. and
	Portet, F. and Sehili, M. and Chahuara, P.},
  title = {Evaluation of a Real-Time Voice Order Recognition System from Multiple
	Audio Channels in a Home},
  booktitle = interspeech,
  year = {2013}
}

@INPROCEEDINGS{VKF05,
  author = {Vovos, A. and Kladis, B. and Fakotakis, N.},
  title = {Speech Operated Smart-Home Control System for Users with Special
	Needs},
  booktitle = interspeech,
  year = {2005}
}



@INPROCEEDINGS{WFIM06,
  author = {W\"{o}lfel, M. and F\"{u}gen, C. and Ikbal, S. and McDonough, J.
	W.},
  title = {Multi-Source Far-Distance Microphone Selection and Combination
	
	for Automatic Transcription of Lectures},
  booktitle = interspeech,
  year = {2006},
  pages = {361-364},
  owner = {nassos},
  timestamp = {2013.11.04}
}

@ARTICLE{Wil+90,
  author = {Wilpon, J. and Rabiner, L. R. and Lee, C.-H. and Goldman, E. R.},
  title = {Automatic recognition of keywords in unconstrained speech using hidden
	{M}arkov models},
  journal = IEEE_J_ASSP,
  year = {1990},
  volume = {38},
  pages = {1870-1878},
  number = {11}
}

@INPROCEEDINGS{WoNa13,
  author = {Wolf, M. and Nadeu, C.},
  title = {Channel Selection Using {N}-{B}est Hypothesis for Multi-Microphone
	{ASR}},
  booktitle = interspeech,
  year = {2013}
}

@INPROCEEDINGS{WoNa10,
  author = {Wolf, M. and Nadeu, C.},
  title = {On the potential of channel selection for
	
	recognition of reverberated speech with multiple microphones},
  booktitle = interspeech,
  year = {2010},
  pages = {80 - 83},
  owner = {nassos},
  timestamp = {2013.11.04}
}


@INPROCEEDINGS{dicit_1,
  author = {Omologo, M.},
  title = {{A prototype of distant-talking interface for control of interactive TV}},
  booktitle = "Proc. of ASILOMAR 2010",
  pages = {1711-1715}
}


@BOOK{dasr,
  title = {Distant Speech Recognition},
  publisher = {Wiley},
  year = {2009},
  author = {W\"{o}lfel, M. and McDonough, J.}
}



@Book{roberto,
  author = "Pieraccini, R.",
  title = "The Voice in the Machine: Building Computers that Understand Speech",
  publisher = "MIT press",
  year = "2012"
}


@Book{mmprocessing,
  author = "Brandstein, D. W. M.",
  title = "Microphone Arrays: Signal Processing Techniques and Applications",
  publisher = "Springer",
  year = "2001"
}

@Book{speh,
  author = "Benesty, J. and Makino, S. and Chen, J.",
  title = "Speech Enhancement",
  publisher = "Springer",
  year = "2005"
}


@Book{roomac,
  author = "Kuttruff, H.",
  title = "Room acoustic-fifth edition",
  publisher = "Spon Press",
  year = "2009"
}







@INPROCEEDINGS{Woo01,
  author = {Woodland, P. C.},
  title = {Speaker adaptation for continuous density {HMM}s: {A} review},
  booktitle = {ISCA Tutorial and Research Workshop on Adaptation Methods for Speech
	Recognition},
  year = {2001}
}




@incollection{vad1,
year={2010},
booktitle={Advanced Techniques in Computing Sciences and Software Engineering},
editor={Elleithy, Khaled},
title={Voiced/Unvoiced Decision for Speech Signals Based on Zero-Crossing Rate and Energy},
publisher={Springer Netherlands},
author={Bachu, R.G. and Kopparthi, S. and Adapa, B. and Barkana, B.D.},
pages={279-282},
}


@BOOK{vad0,
  author = {Meduri, S. and Ananth, S.},
  title = {{A Survey and Evaluation of Voice Activity Detection Algorithms.}},
  publisher = {Lambert Academic Publishing},
  year = {2012}
}



@article{vad2,
	AUTHOR = "Tucker, R.",
	TITLE = "Voice activity detection using a periodicity measure",
	JOURNAL = "IEEE transaction on Speech and Vision",
	VOLUME = {139},
	NUMBER = {4},
	PAGES = {377-380},
	MONTH = "August",
	YEAR = {1992}	
 }
    
 
 @ARTICLE{vad3, 
 author={Sohn, J. Kim, N.S and Sung, W.}, 
 journal={IEEE Signal Processing Letters}, 
 title={A statistical model-based voice activity detection}, 
 year={1999}, 
 month={Jan}, 
 volume={6}, 
 number={1}, 
 pages={1-3}
 }
 
 
 @INPROCEEDINGS{vad4,
  author = {Armani, L. and Matassoni, M and Omologo, M. and Svaizer, P.},
  title = {{Use of a CSP-based voice activity detector for distant-talking ASR}},
  booktitle = {Proc. of EUROSPEECH 2003},
  year = {2003},
  pages={501-504}
}



@incollection{aed1,
booktitle={Computers in the Human Interaction Loop},
title={Acoustic event detection and classification},
publisher={Springer London},
author={Temko, A. and Nadeu, C. and  Macho, D. and Malkin, R. and Zieger, C. and Omologo, M.},
pages={61-73},
year={2009}
}


@article{aed2,
  title={Classification of acoustic events using SVM-based clustering schemes},
  author={Temko, Andrey and Nadeu, Climent},
  journal={Pattern Recognition},
  volume={39},
  number={4},
  pages={682--694},
  year={2006},
  publisher={Elsevier}
}

@inproceedings{aed3,
  author        = "Zieger, C. and Omologo, M.",
  title         = "{Acoustic Event Classification Using a Distributed Microphone Network with a GMM/SVM Combined Algorithm}",
  booktitle     = "Proc. of Interspeech 2008",
  pages={504--5164},
  year          = "2008"
}


@inproceedings{aed4,
  author        = "Gencoglu, O. and  Virtanen, T. and  Huttunen, H.",
  title         = "{Recognition of Acoustic Events Using Deep Neural Networks}",
  booktitle     = "EUSIPCO 2014",
  address = {Lisbon, Portugal},
  year          = "2014"
}

@inproceedings{aed5,
  author        = "Ravanelli, M.  and Elizalde, B. and Ni, K. and  Friedland, G.",
  title         = "{Audio Concept Classification with Hierarchical Deep Neural Networks}",
  booktitle     = "EUSIPCO 2014",
  address = {Lisbon, Portugal},
  year          = "2014"
}


 
@Book{Huang-2004,
  author = 	 {Huang, Y. and Benesty, J.},
  title = 	 {Audio Signal Processing for Next-Generation Multimedia Communication Systems},
  publisher = 	 {Kluwer Academic Publishers},
  year = 	 {2004}
}

@Book{Brandstein-2001,
  author = 	 {Brandstein, M. and Ward, D.},
  title = 	 {Microphone Arrays},
  publisher = 	 {Springer-Verlag},
  year = 	 {2001}
}

@InProceedings{Macho-2005,
  author = 	 {Macho, D. and Padrell, J. and Adad, A. and McDonough, J. and Wolfel, M. and Brutti, A. and Omologo, M. and Potamianos, G. and Chu, S. and Klee, U. and Svaizer, P. and Nadeu, C. and Hernando, J.},
  title = 	 {Automatic Speech Activity Detection, Source Localization and Speech Recognition on the Chil Seminar Corpus},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = {Proc. of IEEE International Conference on Multimedia and Expo},
  OPTpages = 	 {},
  year = 	 {2005}
}

@InProceedings{Chu-2004,
  author = 	 {Chu, W. and Cheng, W. and Wu, J. and Hsu, J.},
  title = 	 {A study of semantic context detection by using {SVM} and {GMM} approache},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = {Proc. of IEEE International Conference on Multimedia and Expo},
  OPTpages = 	 {},
  year = 	 {2004}
}

@Article{Guo-2003,
  author = 	 {Guo, G. and Li, S.},
  title = 	 {Content-based audio classification and retrieval by support vector machines},
  journal = 	 {IEEE Trans. on Neural Networks},
  year = 	 {2003},
  OPTkey = 	 {},
  volume = 	 {14},
  number = 	 {1}
}

@Article{Cai-2006,
  author = 	 {Cai, R and Lu, L. and Hanjalic, A. and Zhang, H. and Cai, L.},
  title = 	 {A flexible framework for key audio effects detection and auditory context inference},
  journal = 	 {IEEE Trans. on Audio, Speech and Language Processing},
  year = 	 {2006},
  OPTkey = 	 {},
  volume = 	 {14},
  number = 	 {3}
}

@Article{Ramirez-2005,
  author = 	 {Ramirez,J. and Segura, J.C. and Benitez, C. and De la Torre, A. and Rubio, A.},
  title = 	 {An effective subband OSF-based VAD with noise reduction for robust speech recognition},
  journal = 	 {IEEE Trans. on Speech and Audio Processing},
  year = 	 {2005},
  OPTkey = 	 {},
  volume = 	 {13},
  number = 	 {6},
  OPTpages = 	 {},
  month = 	 {Nov},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@InProceedings{Vinet-2002,
  author = 	 {Vinet, H. and Herrera, P. and Pachet, F.},
  title = 	 {The cuidado project: New applications based on audio and music content description},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = {Proc. of International Computer Music Conferen},
  OPTpages = 	 {},
  year = 	 {2002},
  OPTeditor = 	 {},
  OPTvolume = 	 {},
  OPTnumber = 	 {},
  OPTseries = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@InProceedings{Trancoso-2009,
  author = 	 {Trancoso, I. and Portelo, J. and Bugalho, M. and da Silva Neto, J. and Serralheiro, A.},
  title = 	 {Training audio events detectors with a sound effects corpus},
  OPTcrossref =  {},
  year = 	 {2009},
  booktitle = {Proc. of Interspeech.},
  OPTpages = 	 {},
  OPTyear = 	 {},
  OPTeditor = 	 {},
  OPTvolume = 	 {},
  OPTnumber = 	 {},
  OPTseries = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@InProceedings{Portelo-2008,
  author = 	 {Portelo, J. and Bugalho, M. and Trancoso, I. and Neto, J. and Abad, A. and Serralheiro, A.},
  title = 	 {Non-speech audio event detection},
  booktitle = 	 {Proc. IEEE International Conference on Acoustics, Speech and Signal Processing},
  year = 	 {2008},
  OPTkey = 	 {},
  OPTvolume = 	 {},
  OPTnumber = 	 {},
  OPTpages = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@Article{Bouquin-1995,
  author = 	 {Bouquin-Jeannes, R.L. and Faucon, G.},
  title = 	 {Study of a voice activity detector and its influence on a noise reduction system},
  journal = 	 {Speech Communication},
  year = 	 {1995},
  OPTkey = 	 {},
  volume = 	 {16},
  OPTnumber = 	 {},
  OPTpages = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@Article{Junqua-1994,
  author = 	 {Junqua, J.C. and Mak, B. and Reaves, B.},
  title = 	 {A robust algorithm for word boundary detection in the presence of noise},
  journal = 	 {IEEE Trans. on Speech and Audio Processing},
  year = 	 {1994},
  OPTkey = 	 {},
  volume = 	 {2},
  number = 	 {3},
  OPTpages = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}


@InProceedings{Dines-2006,
  author = 	 {Dines, J. and Vepa, J. and Hain, T.},
  title = 	 {The segmentation of multichannel meeting recordings for automatic speech recognition},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = { Proc. Int. Conf. on Speech Communication and Technology},
  OPTpages = 	 {},
  year = 	 {2006}
}

@Article{shin-2010,
  author = 	 {Shin, J. W. and  Chang, J.H. and Kim, N. S.},
  title = 	 {Voice activity detection based on statistical models and machine learning approaches},
  journal = 	 {Computer Speech and Language},
  year = 	 {2010},
  OPTkey = 	 {},
  Tvolume = 	 {24},
  Tnumber = 	 {3},
  pages = 	 {515=530},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@Article{Wrigley-2005,
  author = 	 {Wrigley, S.N. and Brown, G.J. and Wan, V. and Renals, S.},
  title = 	 {Speech and crosstalk detection in multichannel audio},
  journal = 	 {IEEE Trans. on Speech and Audio Processing},
  year = 	 {2005},
  OPTkey = 	 {},
  volume = 	 {13},
  number = 	 {1},
  pages = 	 {84-91},
  month = 	 {Jan},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@Article{Zhang-2013,
  author = 	 {Zhang, X.L. and Wu, J.},
  title = 	 {Deep belief networks based voice activity detection},
  journal = 	 {IEEE Trans. on Audio, Speech, and Language Processing},
  year = 	 {2013},
  OPTkey = 	 {},
  volume = 	 {21},
  number = 	 {4},
  pages = 	 {679-710},
  month = 	 {April},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@Article {Deng-2012,
author       = {Li Deng},
journal      = {APSIPA Transactions on Signal and Information Processing},
title        = {Three Classes of Deep Learning Architectures and Their Applications: A Tutorial
                Survey},
opturl          = {http://research.microsoft.com/apps/pubs/default.aspx?id=192937},
year         = {2012},
}

@Article{Cooke-2006,
  author = 	 {Cooke, M. and Barker, J. and Cunningham, S. and Shao, X.},
  title = 	 {An audio-visual corpus for speech perception and automatic speech recognition.},
  journal = 	 {Journal of Acoustical Society of America},
  year = 	 {2006},
  OPTkey = 	 {},
  volume = 	 {120},
  OPTnumber = 	 {},
  OPTpages = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@InProceedings{Brutti-2009,
  author = 	 {Brutti, A. and Omologo, M. and Svaizer, P.},
  title = 	 {A sequential {M}onte {C}arlo approach for tracking of overlapping acoustic sources},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = {EUSIPCO},
  OPTpages = 	 {},
  year = 	 {2009},
  OPTeditor = 	 {},
  OPTvolume = 	 {},
  OPTnumber = 	 {},
  OPTseries = 	 {},
  OPTaddress = 	 {},
  OPTmonth = 	 {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}


@book{woelfel2009,
      author       = "W{\"o}lfel, M. and McDonough, J.",
      title        = "Distant speech recognition",
      publisher    = "Wiley",
      optaddress      = "Chichester",
      year         = "2009",
}
@inproceedings{LREC2014, 
	title={The {DIRHA} simulated corpus}, 
	author={Cristoforetti, L. and Ravanelli, M. and Omologo, M. and Sosi, A. and Abad, A. and Hagmueller, M. and Maragos, P.}, 
	booktitle = "LREC"
}
@inproceedings{Farina_2000, 
	title={Simultaneous Measurement of Impulse Response and Distortion with a Swept-Sine Technique}, 
	author={Farina, A},
	booktitle = "110th AES Convention",
        month={February},
	year={2000}
}
@inproceedings{Ravanelli_2012, 
	title={Impulse Response estimation for robust speech recognition in a reverberant environment}, 
	author={Ravanelli, M. and Sosi, A. and Omologo, M. and Svaizer P.}, 
	booktitle = "Proc. of EUSIPCO 2012"
}
@incollection{omologo2006,
  title={Speaker localization in {CHIL} lectures: Evaluation criteria and results},
  author={Omologo, M. and Svaizer, P. and Brutti, A. and Cristoforetti, L.},
  booktitle={Machine Learning for Multimodal Interaction},
  pages={476--487},
  year={2006},
  publisher={Springer}
}
@inproceedings{Temko2006,
 author = {Temko, A. and Malkin, R. and Zieger, C. and Macho, D. and Nadeu, C. and Omologo, M.},
 title = {CLEAR Evaluation of Acoustic Event Detection and Classification Systems},
 booktitle = {Proceedings of the 1st International Evaluation Conference on Classification of Events, Activities and Relationships},
 series = {CLEAR'06},
 year = {2007},
 optisbn = {978-3-540-69567-7},
 optlocation = {Southampton, UK},
 optpages = {311--322},
 optnumpages = {12},
 opturl = {http://dl.acm.org/citation.cfm?id=1759639.1759676},
 optacmid = {1759676},
 publisher = {Springer-Verlag},
 optaddress = {Berlin, Heidelberg},
} 

@INPROCEEDINGS{Habib-2010,
author={Habib, T. and Romsdorfer, H.},
booktitle={Sensor Array and Multichannel Signal Processing Workshop (SAM), 2010 IEEE},
title={Combining multiband joint position-pitch algorithm and particle filters for speaker localization},
year={2010},
month={Oct},
volume={},
number={},
pages={149 -152},
optkeywords={M-PoPi;multiband joint position-pitch algorithm;multiple concurrent speaker tracking;particle filters;speaker localization;particle filtering (numerical methods);speech processing;},
optdoi={10.1109/SAM.2010.5606723},
optISSN={1551-2282},
}
@Book{DeMori98,
  author = 	 {R. DeMori},
  title = 	 {Spoken Dialogues with Computers},
  publisher = 	 {Academic Press},
  year = 	 {1998},
  address = 	 {London},
  note = 	 {Chapter 2}
}
@article{Brutti_EURASIP,
 author = {Brutti, Alessio and Omologo, Maurizio and Svaizer, Piergiorgio},
 title = {Multiple source localization based on acoustic map de-emphasis},
 journal = {EURASIP J. Audio Speech Music Process.},
  volume = {2010},
optmonth = {January},
 year = {2010},
 pages = {11-17},
}
@INPROCEEDINGS{Armani2003,
author = {Armani, L. and Matassoni, M. and Omologo, M. and Svaizer,P.},
title={Use of a {CSP}-based voice activity detector for distant-talking {ASR}},
booktitle={EUROSPEECH},
year=2003
}

@inproceedings{shallow_fusion,
title	= {A comparison of techniques for language model integration in encoder-decoder speech recognition},
author	= {Shubham Toshniwal and Anjuli Kannan and Chung-Cheng Chiu and Yonghui Wu and Tara Sainath and Karen Livescu},
year	= {2018},
URL	= {https://arxiv.org/pdf/1807.10857.pdf}
}



@article{KnappCarter,
  author = 	 {C. H. Knapp and G. C. Carter},
  title = 	 {The generalized correlation method for estimation of time delay},
  booktitle =    {IEEE Transactions on Acoustics, Speech, and Signal Processing},
  volume =       {24},
  number =	 {4},
  pages =        {320-327},
  year = 	 {1976}
}

@article{wolf2013,
author = {Wolf, M. and Nadeu, C.},
title = {Channel selection measures for multi-microphone speech recognition},
journal = {Speech Communication},
volume = {},
number = {3},
Pages={170-180},
year = {2013},
}

@ARTICLE{sehr2010,
author={Sehr, A. and Maas, R. and Kellermann, W.},
journal={IEEE Trans. on Audio, Speech, and Language Processing},
title={Reverberation Model-Based Decoding in the Logmelspec Domain for
Robust Distant-Talking Speech Recognition},
year={2010},
volume={18},
number={7},
pages={1676-1691},
ISSN={1558-7916},
}
@Article{Maskell-2002,
  author = 	 {M. Arulampalam and S. Maskell},
  title = 	 {A Tutorial on Particle Filters for On-line Nonlinear/Non-Gaussian Bayesian Tracking},
  journal = 	 {IEEE Transactions on Signal Processing},
  year = 	 {2002},
  OPTkey = 	 {},
  volume = 	 {50},
  number = 	 {2},
  optpages = 	 {174-178},
  month = 	 {February},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@InProceedings{Pham-2008,
  author = 	 {Pham, T.V. and Stadtschnitzer, M. and Pernkopf F. and Kubin G.},
  title = 	 {Voice activity detection algorithms using subband power distance feature for noisy environments},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = {Proc. of Interspeech},
  OPTpages = 	 {},
  year = 	 {2008}
}


@InProceedings{Vermaak-2001,
  author = 	 {Vermaak, J and Blake, A.},
  title = 	 {Nonlinear ﬁltering for speaker tracking in noisy and reverberant environments},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = {IEEE Intern. Conf. on Acoustics, Speech and Signal Processing},
  OPTpages = 	 {},
  year = 	 {2001}
}

@Article{Lehman-2007,
  author = 	 {Lehman, E and Johansson, A.},
  title = 	 {Particle filter with integrated voice activity detection for acoustic source tracking},
  journal = 	 { EURASIP Journal on Applied Signal Processing},
  year = 	 {2007}
}


@Article{Lathoud-2007,
  author = 	 {Lathoud, G. and Odobez, J.M.},
  title = 	 {Short-term spatio-temporal clustering applied to multiple moving speakers},
  journal = 	 {IEEE Trans. on Audio, Speech and Language Processing},
  year = 	 {2007},
  OPTkey = 	 {},
  volume = 	 {15},
  number = 	 {5},
  OPTpages = 	 {},
  month = 	 {July},
  OPTnote = 	 {},
  OPTannote = 	 {}
}


 @InProceedings{DiClaudio-2000,
  author = 	 {Di Claudio, E. and Parisi, R. and Orlandi, G.},
  title = 	 {Multi-source localization in reverberant environments by ROOT-MUSIC and clustering},
  OPTcrossref =  {},
  OPTkey = 	 {},
  booktitle = {Proc. of IEEE conference on Acoustics, Speech, and Signal Processing},
  OPTpages = 	 {},
  year = 	 {2000}
}


@INPROCEEDINGS{vtln,
author={Eide, E. and Gish, Herbert},
booktitle={Proc. of ICASSP 96},
title={A parametric approach to vocal tract length normalization},
year={1996},
pages={346-348}
}

@Article{Brutti-2012,
  author = 	 {Brutti, A. and Nesta, F.},
  title = 	 {Tracking of multidimensional TDOA for multiple sources with distributed microphone pairs},
  journal = 	 {Computer Speech And Language},
volume = {27},
 number = {3},
 year = {2013}
}

@INPROCEEDINGS{Fallon-2008,
author={Fallon, M.},
booktitle={Hands-Free Speech Communication and Microphone Arrays, 2008. HSCMA 2008},
title={Multi Target Acoustic Source Tracking with an Unknown and Time Varying Number of Targets},
year={2008},
month={May},
optpages={77-80}
}

@INPROCEEDINGS{Lee-2010,
author={Lee, Y. and Wada, T.S. and Biing-Hwang Juang},
booktitle={ IEEE International Conference on Acoustics Speech and Signal Processing},
title={Multiple acoustic source localization based on multiple hypotheses testing using particle approach},
year={2010},
optmonth={March},
optpages={2722-2725}
}

@InProceedings{Sawada-2003,
  author = 	{H. Sawada, H. and Mukai, R. and Makino, S.},
  title = 	{Direction of Arrival Estimation for Multiple Source Signals using Independent Component Analysis},
  booktitle =	{Proceedings of ISSPA},
  optmonth =	jul,
  year =	{2003},
  optpages =	{411--414},
  optvolume =	{2}
} 

@article{Loesch-2009,
           author = {Loesch, B. and Uhlich, S. and Yang, B.},
            title = {Multidimensional Localization of multiple sound sources using frequency domain {ICA} and an extended state coherence transform},
          journal = {Proceedings of IEEE Workshop on Statistical Signal Processing},
            optmonth = {September},
             year = {2009}
}
@inproceedings{Araki-2009,
 author = {Araki, Shoko and Nakatani, Tomohiro and Sawada, Hiroshi and Makino, Shoji},
 title = {Stereo Source Separation and Source Counting with {MAP} Estimation with {D}irichlet Prior Considering Spatial Aliasing Problem},
 booktitle = {Proc. of the International Conference on Independent Component Analysis and Signal Separation},
 year = {2009},
 optisbn = {978-3-642-00598-5},
 optpages = {742--750},
 optlocation = {Paraty},
 optdoi = {http://dx.doi.org/10.1007/978-3-642-00599-2_93},
 optpublisher = {Springer-Verlag},
 optaddress = {Berlin, Heidelberg}
 }

@ARTICLE{Nesta-2011,
author={Nesta, F. and Omologo, M.},
journal={Audio, Speech, and Language Processing, IEEE Transactions on}, 
title={Generalized {S}tate {C}oherence {T}ransform for multidimensional {TDOA} estimation of multiple sources},
year={2011},
optdoi={10.1109/TASL.2011.2160168},
optISSN={1558-7916}
}


@inproceedings{returnn,
    title = "{RETURNN} as a Generic Flexible Neural Toolkit with Application to Translation and Speech Recognition",
    author = "Zeyer, Albert  and Alkhouli, Tamer  and Ney, Hermann",
    booktitle = "Proc. of ACML",
    year = "2018",
}

@article{speak_or_chat,
  author    = {Sujeong Cha and
               Wangrui Hou and
               Hyun Jung and
               My Phung and
               Michael Picheny and
               Hong{-}Kwang Kuo and
               Samuel Thomas and
               Edmilson da Silva Morais},
  title     = {Speak or Chat with Me: End-to-End Spoken Language Understanding System
               with Flexible Inputs},
  journal   = {CoRR},
  volume    = {abs/2104.05752},
  year      = {2021},
}

@INPROCEEDINGS{gcf,
  author={Omologo, M. and Svaizer, P.},
  booktitle={Proceedings of ICASSP}, 
  title={Acoustic event localization using a crosspower-spectrum phase based technique}, 
  year={1994},
  volume={ii},
  number={},
  pages={II/273-II/276 vol.2},
  doi={10.1109/ICASSP.1994.389667}}
  
@inproceedings{brutti2005oriented,
  title={Oriented global coherence field for the estimation of the head orientation in smart rooms equipped with distributed microphone arrays},
  author={Brutti, A. and Omologo, M. and Svaizer, P.},
  booktitle={Proc. of EUROSPEECH 2005},
   pages = {2337-2340},
  year={2005}
}


@INPROCEEDINGS{spkid,
author={Sidorov, M. and Schmitt, A. and Zablotskiy, S. and Minker, W.},
booktitle={IE 2013},
title={Survey of Automated Speaker Identification Methods},
year={2013},
month={July},
pages={236-239}
}

@INPROCEEDINGS{2011_Stolcke,
  author = {Stolcke, Andreas},
  title = {Making the most from multiple microphones in meeting recognition},
  booktitle = {Proc. of ICASSP 2011},
  year = {2011},
  pages = {4992--4995},
}

@INBOOK{beam,
  author    = {Kellermann, W.},
  title     = {Beamforming for Speech and Audio Signals},
  year      = {2008},
  publisher = {in HandBook of Signal Processing in Acoustics, Springer},
}

@INPROCEEDINGS{beam2,
author={Kajala, M. and Hamalainen, M.},
booktitle={Proc. of ICASSP 2001},
title={Filter-and-sum beamformer with adjustable filter characteristics},
year={2001},
pages={2917-2920}
}

@incollection{beam3,
year={2001},
booktitle={Microphone Arrays},
title={Superdirective Microphone Arrays},
publisher={Springer Berlin Heidelberg},
author={Bitzer, Joerg and Simmer, K.Uwe},
pages={19-38}
}

@article{nadeu,
 author = {Wolf, Martin and Nadeu, Climent},
 title = {Channel Selection Measures for Multi-microphone Speech Recognition},
 journal = {Speech Communication},
 volume = {57},
 month = feb,
 year = {2014},
 pages = {170--180}
} 

@inproceedings{nadeu2,
author="Wolf, M. and Nadeu, C.",
title="On the potential of channel selection for recognition of reverberated speech with multiple microphones",
booktitle="Proc. of Interspeech 2010",
pages="574--577",
year="2010"
}

@inproceedings{nadeu3,
  title={Blind estimation of the coherent-to-diffuse energy ratio from noisy speech signals},
  author={Jeub, M. and Nelke, C. and Beaugeant, C. and Vary, P.},
  booktitle={Proc. of EUSIPCO 2011},
  pages={1347--1351},
  year={2011}
}


@INPROCEEDINGS{nadeu4,
    author = {Wolfel, M Fugen, C. and Ikbal, S. and McDonough, J.},
    title = {Multi-Source Far-Distance Microphone Selection and Combination for Automatic Transcription of Lectures},
    booktitle = {Proc. of Interspeech 2006},
    pages={1121--1125},
    year = {2006}
}






@INPROCEEDINGS{sphinx,
    author = {D. Huggins-Daines and M. Kumar and A. Chan and A. W. Black and M. Ravishankar and A. I. Rudnicky},
    title = {PocketSphinx: A free, real-time continuous speech recognition system for hand-held devices},
    booktitle = {in Proc. of ICASSP},
    year = {2006}
}

@INPROCEEDINGS{julius,
    author = {A. Lee and T. Kawahara and K. Shikano},
    title = {Julius: An open source realtime large vocabulary recognition engine},
    booktitle = {Proc. of EUROSPEECH},
    year = {2001},
}

@inproceedings{pytorch,
 author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
 booktitle = {Proc. of NeurIPS},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
 year = {2019}
}

@inproceedings{tensorflow,
title	= {TensorFlow: A system for large-scale machine learning},
author	= {Martin Abadi and Paul Barham and Jianmin Chen and Zhifeng Chen and Andy Davis and Jeffrey Dean and Matthieu Devin and Sanjay Ghemawat and Geoffrey Irving and Michael Isard and Manjunath Kudlur and Josh Levenberg and Rajat Monga and Sherry Moore and Derek G. Murray and Benoit Steiner and Paul Tucker and Vijay Vasudevan and Pete Warden and Martin Wicke and Yuan Yu and Xiaoqiang Zheng},
year	= {2016},
booktitle	= {Proc. of. USENIX Symposium on Operating Systems Design and Implementation},
}

@misc{fairseq,
   title={fairseq: A Fast, Extensible Toolkit for Sequence Modeling},
   author={Myle Ott and Sergey Edunov and Alexei Baevski and Angela Fan and Sam Gross and Nathan Ng and David Grangier and Michael Auli},
   year={2019},
   eprint={1904.01038},
   archivePrefix={arXiv},
   primaryClass={cs.CL}
}
@misc{deepspeech,
  author = {Hannun, Awni and Case, Carl and Casper, Jared and Catanzaro, Bryan and Diamos, Greg and Elsen, Erich and Prenger, Ryan and Satheesh, Sanjeev and Sengupta, Shubho and Coates, Adam and Ng, Andrew Y.},
  title = {Deep Speech: Scaling up end-to-end speech recognition},
  url = {http://arxiv.org/abs/1412.5567},
  year = 2014
}


@inproceedings{espresso,
  title = {Espresso: A Fast End-to-end Neural Speech Recognition Toolkit},
  author = {Yiming Wang and Tongfei Chen and Hainan Xu 
            and Shuoyang Ding and Hang Lv and Yiwen Shao 
            and Nanyun Peng and Lei Xie and Shinji Watanabe 
            and Sanjeev Khudanpur},
  booktitle = {Proc. of IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
  year = {2019},
}


@inproceedings{espnet,
  author={Shinji Watanabe and Takaaki Hori and Shigeki Karita and Tomoki Hayashi and Jiro Nishitoba and Yuya Unno and Nelson {Enrique Yalta Soplin} and Jahn Heymann and Matthew Wiesner and Nanxin Chen and Adithya Renduchintala and Tsubasa Ochiai},
  title={{ESPnet}: End-to-End Speech Processing Toolkit},
  year={2018},
  booktitle={Proceedings of Interspeech},
  pages={2207--2211},
}

@inproceedings{asteroid,
    title={Asteroid: the {PyTorch}-based audio source separation toolkit for researchers},
    author={Manuel Pariente and Samuele Cornell and Joris Cosentino and Sunit Sivasankaran and
            Efthymios Tzinis and Jens Heitkaemper and Michel Olvera and Fabian-Robert Stöter and
            Mathieu Hu and Juan M. Martín-Doñas and David Ditter and Ariel Frank and Antoine Deleforge
            and Emmanuel Vincent},
    year={2020},
    booktitle={Proc. Interspeech},
}


@inproceedings{pyannote,
  Title = {{pyannote.audio: neural building blocks for speaker diarization}},
  Author = {{Bredin}, Herv{\'e} and {Yin}, Ruiqing and {Coria}, Juan Manuel and {Gelly}, Gregory and {Korshunov}, Pavel and {Lavechin}, Marvin and {Fustes}, Diego and {Titeux}, Hadrien and {Bouaziz}, Wassim and {Gill}, Marie-Philippe},
  Booktitle = {Proc. of ICASSP},
  Year = {2020},
}

@misc{superb,
  title={SUPERB: Speech processing Universal PERformance Benchmark}, 
  author={Shu-wen Yang and Po-Han Chi and Yung-Sung Chuang and Cheng-I Jeff Lai and Kushal Lakhotia and Yist Y. Lin and Andy T. Liu and Jiatong Shi and Xuankai Chang and Guan-Ting Lin and Tzu-Hsien Huang and Wei-Cheng Tseng and Ko-tik Lee and Da-Rong Liu and Zili Huang and Shuyan Dong and Shang-Wen Li and Shinji Watanabe and Abdelrahman Mohamed and Hung-yi Lee},
  year={2021},
  eprint={2105.01051},
  archivePrefix={arXiv},
  primaryClass={cs.CL}
}

@misc{nemo,
  author = {Kuchaiev, Oleksii and Li, Jason and Nguyen, Huyen and Hrinchuk, Oleksii and Leary, Ryan and Ginsburg, Boris and Kriman, Samuel and Beliaev, Stanislav and Lavrukhin, Vitaly and Cook, Jack and Castonguay, Patrice and Popova, Mariya and Huang, Jocelyn and Cohen, Jonathan M.},
  title = {{NeMo: a toolkit for building AI applications using Neural Modules}},
  url = {http://arxiv.org/abs/1909.09577},
  year = 2019
}

@inproceedings{jasper,
  author    = {Jason Li and
               Vitaly Lavrukhin and
               Boris Ginsburg and
               Ryan Leary and
               Oleksii Kuchaiev and
               Jonathan M. Cohen and
               Huyen Nguyen and
               Ravi Teja Gadde},
  editor    = {Gernot Kubin and
               Zdravko Kacic},
  title     = {Jasper: An End-to-End Convolutional Neural Acoustic Model},
  booktitle = {Proc. of Interspeech 2019},
  pages     = {71--75},
  year      = {2019},
}

@inproceedings{quartznet,
  author    = {Samuel Kriman and
               Stanislav Beliaev and
               Boris Ginsburg and
               Jocelyn Huang and
               Oleksii Kuchaiev and
               Vitaly Lavrukhin and
               Ryan Leary and
               Jason Li and
               Yang Zhang},
  title     = {Quartznet: Deep Automatic Speech Recognition with 1D Time-Channel
               Separable Convolutions},
  booktitle = {Proc. of ICASSP},
  pages     = {6124--6128},
  year      = {2020},
}

@misc{citrinet,
      title={Citrinet: Closing the Gap between Non-Autoregressive and Autoregressive End-to-End Models for Automatic Speech Recognition}, 
      author={Somshubra Majumdar and Jagadeesh Balam and Oleksii Hrinchuk and Vitaly Lavrukhin and Vahid Noroozi and Boris Ginsburg},
      year={2021},
      eprint={2104.01721},
      archivePrefix={arXiv},
      primaryClass={eess.AS}
}

@InProceedings {rwth,
author= {Rybach, D. and Hahn, S. and Lehnen, P. and Nolden, D. and Sundermeyer, M. and T{\"u}ske, Z. and Wiesler, S. and Schl{\"u}ter, R. and Ney, H.},
title= {{RASR - The RWTH Aachen University Open Source Speech Recognition Toolkit}},
booktitle= {Proc. of ASRU},
year= 2011,
}

@MISC{dirhaproj,
  title = {{DIRHA}: {D}istant-speech {I}nteraction for {R}obust {H}ome {A}pplications},
  note = {[Online] Available: \url{http://dirha.fbk.eu/}}
}
@ARTICLE{roberto12,
	AUTHOR = "Mic Bowman and Saumya K. Debray and Larry L. Peterson",
	TITLE = "Reasoning About Naming Systems",
	JOURNAL = "ACM Trans. Program. Lang. Syst.",
	VOLUME = {15},
	NUMBER = {5},
	PAGES = {795--825},
	MONTH = "November",
	YEAR = {1993}	}

@ARTICLE{braams:babel,
	AUTHOR = "Johannes Braams",
	TITLE = "Babel, a Multilingual Style-Option System for Use with LaTeX's Standard Document Styles",
	JOURNAL = {TUGboat},
	VOLUME = {12},
	NUMBER = {2},
	PAGES = {291-301},
	MONTH = "June",
	YEAR = {1991}	}

@inproceedings{batching,
  author={Ehsan Variani and Tom Bagby and Erik McDermott and Michiel Bacchiani},
  title={End-to-End Training of Acoustic Models for Large Vocabulary Continuous Speech Recognition with TensorFlow},
  year=2017,
  booktitle={Proc. Interspeech},
  pages={1641--1645},
}

@inproceedings{morishita-etal-2017-empirical,
    title = "An Empirical Study of Mini-Batch Creation Strategies for Neural Machine Translation",
    author = "Morishita, Makoto  and
      Oda, Yusuke  and
      Neubig, Graham  and
      Yoshino, Koichiro  and
      Sudoh, Katsuhito  and
      Nakamura, Satoshi",
    booktitle = "Proc. of the WNMT",
    year = "2017",
}

@INPROCEEDINGS{clark:pct,
	AUTHOR = "Malcolm Clark",
	TITLE = "Post Congress Tristesse",
	BOOKTITLE = "TeX90 Conference Proceedings",
	PAGES = "84-89",
	ORGANIZATION = "TeX Users Group",
	MONTH = "March", 
	YEAR = {1991}	}

@ARTICLE{herlihy:methodology,
	AUTHOR = "Maurice Herlihy",
	TITLE = "A Methodology for Implementing Highly Concurrent
	Data Objects",
	JOURNAL = {ACM Trans. Program. Lang. Syst.},
	VOLUME = {15},
	NUMBER = {5},
	PAGES = {745-770},
	MONTH = "November",
	YEAR = {1993}	}

@BOOK{Lamport:LaTeX,
	AUTHOR = "Leslie Lamport",
	TITLE = "LaTeX User's Guide and Document Reference Manual",
	PUBLISHER = "Addison-Wesley Publishing Company",
	ADDRESS = "Reading, Massachusetts",
	YEAR = "1986"	}

@BOOK{salas:calculus,
	AUTHOR = "S.L. Salas and Einar Hille",
	TITLE = "Calculus: One and Several Variable",
	PUBLISHER = "John Wiley and Sons",
	ADDRESS = "New York",
	YEAR = "1978"	}
    
   @Inproceedings{Peterson,
	author="P. Peterson",
	title="Simulating the response of multiple microphones to a
single acoustic source in a reverberant room",
	booktitle="J. Acoust. Soc. Am",
    volume="80(5)",
    pages="1527--1529",
	year=1986
}

 
  @Inproceedings{Lehmann,
	author="E. Lehmann and A. Johansson",
	title="Prediction of energy decay in room impulse responses simulated with an image-source model",
	booktitle="J. Acoust. Soc. Am",
    volume="124(1)",
    pages="269-277",
	year=2008
}    
    
@incollection{deep_autoencoder_1,
title = {Greedy Layer-Wise Training of Deep Networks},
author = {Bengio, Y. and Pascal L. and D. Popovici and Larochelle, H.},
booktitle = {Proc. of NIPS},
pages = {153--160},
year = {2007},
}
@inproceedings{bagchi2018spectral,
  title={Spectral Feature Mapping with Mimic Loss for Robust Speech Recognition},
  author={Bagchi, Deblin and Plantinga, Peter and Stiff, Adam and Fosler-Lussier, Eric},
  booktitle={Proc. of ICASSP},
  year={2018}
 }
 @article{fu2021metricgan+,
  title={MetricGAN+: An Improved Version of MetricGAN for Speech Enhancement},
  author={Fu, Szu-Wei and Yu, Cheng and Hsieh, Tsun-An and Plantinga, Peter and Ravanelli, Mirco and Lu, Xugang and Tsao, Yu},
  journal={arXiv preprint arXiv:2104.03538},
  year={2021}
}

@article{waibel,
  added-at = {2008-03-11T14:52:34.000+0100},
  author = {Waibel, Alex and Hanazawa, T. and Hinton, Geoffrey E. and Shikano, K. and Lang, K.},
  journal = {IEEE Transactions on Acoustics, Speech, and Signal Processing},
  pages = {328--339},
  title = {Phoneme Recognition Using Time-Delay Neural Networks},
  volume = 37,
  year = 1989
}

@article{defossez2020real,
  title={Real Time Speech Enhancement in the Waveform Domain},
  author={D{\'e}fossez, Alexandre and Synnaeve, Gabriel and Adi, Yossi},
  journal={Proc. Interspeech 2020},
  pages={3291--3295},
  year={2020}
}
@article{valentini2017noisy,
  title={Noisy speech database for training speech enhancement algorithms and {TTS} models},
  author={Valentini-Botinhao, Cassia},
  journal={Edinburgh DataShare},
  year={2017},
  publisher={University of Edinburgh School of Informatics, Centre for Speech Technology.}
}
@article{virtanen2020scipy,
  title={{SciPy} 1.0: fundamental algorithms for scientific computing in {Python}},
  author={Virtanen, Pauli and Gommers, Ralf and Oliphant, Travis E and Haberland, Matt and Reddy, Tyler and Cournapeau, David and Burovski, Evgeni and Peterson, Pearu and Weckesser, Warren and Bright, Jonathan and others},
  journal={Nature methods},
  volume={17},
  number={3},
  pages={261--272},
  year={2020},
  publisher={Nature Publishing Group}
}
@book{gulli2017deep,
  title={Deep learning with {Keras}},
  author={Gulli, Antonio and Pal, Sujit},
  year={2017},
  publisher={Packt Publishing Ltd}
}
@article{falcon2019pytorch,
  title={PyTorch {Lightning}},
  author={William Falcon and others},
  journal={GitHub},
  note={\url{https://github.com/PyTorchLightning/pytorch-lightning}},
  volume={3},
  year={2019}
}
@article{hu2007evaluation,
  title={Evaluation of objective quality measures for speech enhancement},
  author={Hu, Yi and Loizou, Philipos C},
  journal={IEEE Transactions on audio, speech, and language processing},
  volume={16},
  number={1},
  pages={229--238},
  year={2007},
  publisher={IEEE}
}

%Code snippets make it easier to adopt a toolkit:
@inproceedings{10.1145/1167473.1167480,
author = {Fairbanks, George and Garlan, David and Scherlis, William},
title = {Design Fragments Make Using Frameworks Easier},
year = {2006},
isbn = {1595933484},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1167473.1167480},
doi = {10.1145/1167473.1167480},
abstract = {Object oriented frameworks impose additional burdens on programmers that libraries did not, such as requiring the programmer to understand the method callback sequence, respecting behavior constraints within these methods, and devising solutions within a constrained solution space. To overcome these burdens, we express the repeated patterns of engagement with the framework as a design fragment. We analyzed the 20 demo applets provided by Sun and created a representative catalog of design fragments of conventional best practice. By evaluating 36 applets pulled from the internet we show that these design fragments are common, many applets copied the structure of the Sun demos, and that creation of a catalog of design fragments is practical. Design fragments give programmers immediate benefit through tool-based conformance assurance and long-term benefit through expression of design intent.},
booktitle = {Proceedings of the 21st Annual ACM SIGPLAN Conference on Object-Oriented Programming Systems, Languages, and Applications},
pages = {75–88},
numpages = {14},
keywords = {object-oriented programming, patterns, design fragments, frameworks},
location = {Portland, Oregon, USA},
series = {OOPSLA '06}
}

  

@article{fairbanks-2006-design-fragments,
author = {Fairbanks, George and Garlan, David and Scherlis, William},
title = {Design Fragments Make Using Frameworks Easier},
year = {2006},
issue_date = {October 2006},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {41},
number = {10},
issn = {0362-1340},
url = {https://doi.org/10.1145/1167515.1167480},
doi = {10.1145/1167515.1167480},
abstract = {Object oriented frameworks impose additional burdens on programmers that libraries did not, such as requiring the programmer to understand the method callback sequence, respecting behavior constraints within these methods, and devising solutions within a constrained solution space. To overcome these burdens, we express the repeated patterns of engagement with the framework as a design fragment. We analyzed the 20 demo applets provided by Sun and created a representative catalog of design fragments of conventional best practice. By evaluating 36 applets pulled from the internet we show that these design fragments are common, many applets copied the structure of the Sun demos, and that creation of a catalog of design fragments is practical. Design fragments give programmers immediate benefit through tool-based conformance assurance and long-term benefit through expression of design intent.},
journal = {SIGPLAN Not.},
month = oct,
pages = {75–88},
numpages = {14},
keywords = {object-oriented programming, frameworks, design fragments, patterns}
}

@article{schmidt1986multiple,
  title={Multiple emitter location and signal parameter estimation},
  author={Schmidt, Ralph},
  journal={IEEE transactions on antennas and propagation},
  volume={34},
  number={3},
  pages={276--280},
  year={1986},
  publisher={IEEE}
}  

@article{cobos2010modified,
  title={A modified {SRP-PHAT} functional for robust real-time sound source localization with scalable spatial sampling},
  author={Cobos, Maximo and Marti, Amparo and Lopez, Jose J},
  journal={IEEE Signal Processing Letters},
  volume={18},
  number={1},
  pages={71--74},
  year={2010},
  publisher={IEEE}
}

@article{habets2009new,
  title={New insights into the {MVDR} beamformer in room acoustics},
  author={Habets, Emanu{\"e}l Anco Peter and Benesty, Jacob and Cohen, Israel and Gannot, Sharon and Dmochowski, Jacek},
  journal={IEEE Transactions on Audio, Speech, and Language Processing},
  volume={18},
  number={1},
  pages={158--170},
  year={2009},
  publisher={IEEE}
}

@inproceedings{heymann2016neural,
  title={Neural network based spectral mask estimation for acoustic beamforming},
  author={Heymann, Jahn and Drude, Lukas and Haeb-Umbach, Reinhold},
  booktitle={2016 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={196--200},
  year={2016},
  organization={IEEE}
}
